Faith-Shap: The Faithful Shapley Interaction Index

Shapley values, which were originally designed to assign attributions to individual players in coalition games, have become a commonly used approach in explainable machine learning to provide attributions to input features for black-box machine learning models. A key attraction of Shapley values is that they uniquely satisfy a very natural set of axiomatic properties. However, extending the Shapley value to assigning attributions to interactions rather than individual players, an interaction index, is non-trivial: as the natural set of axioms for the original Shapley values, extended to the context of interactions, no longer specify a unique interaction index. Many proposals thus introduce additional less ''natural'' axioms, while sacrificing the key axiom of efficiency, in order to obtain unique interaction indices. In this work, rather than introduce additional conflicting axioms, we adopt the viewpoint of Shapley values as coefficients of the most faithful linear approximation to the pseudo-Boolean coalition game value function. By extending linear to $\ell$-order polynomial approximations, we can then define the general family of faithful interaction indices. We show that by additionally requiring the faithful interaction indices to satisfy interaction-extensions of the standard individual Shapley axioms (dummy, symmetry, linearity, and efficiency), we obtain a unique Faithful Shapley Interaction index, which we denote Faith-Shap, as a natural generalization of the Shapley value to interactions. We then provide some illustrative contrasts of Faith-Shap with previously proposed interaction indices, and further investigate some of its interesting algebraic properties. We further show the computational efficiency of computing Faith-Shap, together with some additional qualitative insights, via some illustrative experiments.

==> proofs.tex <==

\newpage
\section{Proof of Propositions}
\label{sec:proofs_propositions}



In this section, we provide the proof of theorems and propositions in Section \ref{sec:faithful_interaction_indices}. Before going to the main proof, we introduce some new notations.

\subsection{Proof of Proposition \ref{pro:closed_matrix_form_solution}}
\begin{proof} 
Now we transform the problem into a linear regression problem using matrix representations:let the feature matrix 
$$
\mathbf{X} \in \{ 0,1\}^{2^{d} \times d_\ell}
\text{  indexed with  } \mathbf{X}_{S,T} = \mathbbm{1}[(T \subseteq S) \vee (T = \text{\O})], 
\text{ where } S \subseteq [d]
\text{ and } T \in\mathcal{S}_\ell.
$$
We note that the feature matrix $\mathbf{X}$ is indexed with two sets $S$ and $T$, denoting its rows and columns. Each row of $S$ can also be expressed as $\mathbf{X}_S = \expd(S)$, where $\expd(S) \in \mathbb{R}^{d_\ell}$ with $\expd(S)[T] = \mathbbm{1}[(T \subseteq S) \vee (T = \text{\O})]$.


Then we define the weight matrix:
$$
\sqrt{\mathbf{W}} \in \{ 0,1\}^{2^{d} \times 2^{d}}
\text{ is a diagonal matrix with each entry on the diagonal } \sqrt{\mathbf{W}}_{S,S} = \sqrt{\mu(S)},
$$
where $S \subseteq [d]$.
The function values of $\f(\cdot)$ on each subset can be written into a vector:
$$
\mathbf{Y} \in \mathbb{R}^{2^{d}}
\text{  indexed with }
\mathbf{Y}_S = \f(S)
\text{ where } S \subseteq [d].
$$
With the above definitions, Equation \eqref{eqn:weighted_regression_in_proof} can be viewed as
$$
\min \norm{\sqrt{\mathbf{W} }(\mathbf{Y} -\mathbf{X} \Expl(\f,\ell))}_2^2 
= \min \norm{\mathbf{Y_w}-\mathbf{X_w}\Expl(\f,\ell)}_2^2,
$$
where $\mathbf{Y_w} = \sqrt{\mathbf{W} }\mathbf{Y}$ and $\mathbf{X_w} = \sqrt{\mathbf{W} }\mathbf{X}$. This is a linear regression problem with $\mathbf{X_w}$ being design matrix and $\mathbf{Y_w}$ being the response vector. Since it has a unique minimizer by Proposition \ref{pro:unique_minimizer}, we can apply the closed-form solution:
\begin{align*}
\ex(\f,\ell)
& = \left(\mathbf{X_w}^{T} \mathbf{X_w} \right)^{-1}
\mathbf{X_w}^T \mathbf{Y_w}  \\
& = \left(\sum_{S \subseteq [d]} \sqrt{\mu(S)}{\expd}(S)  {\sqrt{\mu(S)}\expd}(S)^T \right)^{-1}\!\!\!\sum_{S \subseteq [d]}  \left(\sqrt{\mu(S)}{\expd}(S) \right) \left(\sqrt{\mu(S)}\f(S) \right), \\
& = \left(\sum_{S \subseteq [d]} \mu(S){\expd}(S) {\expd}(S)^T \right)^{-1}\!\!\!\sum_{S \subseteq [d]} \mu(S) \f(S) {\expd}(S).
\end{align*}

\end{proof}



\subsection{Proof of Proposition \ref{pro:linearity}}
\begin{proof}
By Proposition \ref{pro:unique_minimizer}, Faith-Interaction indices are the unique minimizer for some weighting function $\mu(\cdot)$. In below, we discuss two cases: when $\mu(S)$ is finite for all subsets $S$ and when $\mu(S)$ is infinity for some subsets $S$.

First, when the coalition weighting function is finite such that $\mu(S) < \infty$ for all subsets $S \subseteq [d]$, by Proposition \ref{pro:closed_matrix_form_solution}, $\ex(\f,\ell)$ has a linear relation with respect to the set function $\f(\cdot)$. Therefore, it satisfies the interaction linearity axiom.  

Next, we solve the case when some coalition function $\mu(\cdot)$ has infinity measure on some subsets $S$. Denote $\mathcal{T} = \{T: \mu(T) = \infty, T \subseteq [d] \}$ be the set containing all subsets of $[d]$ with infinity weights. We obtain the unique minimizer by solving this constrained minimization problem with Lagrange multiplier. Specifically, we denote $F(\ex) = \sum_{S:S \subseteq [d], \mu(S) < \infty}  \mu(S) \left( \f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) \right)^2$ as our objective and solve the following $d_\ell + |\mathcal{T}|$ equations:
\begin{equation}
\label{eqn:lagrangian}
\begin{cases}
\frac{\partial F(\ex)}{\partial \ex_A } = \sum_{T: T \subseteq \mathcal{T} \wedge T \supseteq A } \lambda_T 
& \text{ for all } A \in \setlessell.
\\
\f(A) - \sum_{T \subseteq A , |T| \leq \ell}\Expl_T(\f,\ell) = 0 
& \text{ for all } A \subseteq \mathcal{T}.
\end{cases}    
\end{equation}

By Definition \ref{def:Dpq} and Proposition \ref{pro:parital_derivative_general}, the partial derivative of Eqn.\eqref{eqn:weighted_regression} with respect to $\Expl_A(\f, \ell)$ is 
$$
\frac{\partial F(\ex)}{\partial \ex_A } =-2 \sum_{ \substack{S: S \supseteq A, \\ \mu(S) < \infty}} \mu(S) \f(S) + 2\sum_{S \in \setlessell} \bar{\mu}(S \cup A) \Expl_S(\f, \ell).
$$
Combing the above, we solve the following equations:
\begin{align}
\label{eqn:lagrangian2}
(i) \ \  & -2 \sum_{ \substack{S: S \supseteq A, \\ \mu(S) < \infty}} \mu(S) \f(S) + 2\sum_{S \in \setlessell} \bar{\mu}(S \cup A) \Expl_S(\f, \ell) = \sum_{T: (T \subseteq \mathcal{T} )\wedge (T \supseteq A) } \lambda_T 
& ,\text{ for all } A \in \setlessell. \nonumber \\
(ii) \ \  & \f(A) - \sum_{T \subseteq A , |T| \leq \ell}\Expl_T(\f,\ell) = 0 
& ,\text{ for all } A \subseteq \mathcal{T}.
\end{align}
Denote $\lambda = [\lambda_T]_{T \subseteq \mathcal{T}} \subseteq \mathbb{R}^{|\mathcal{T}|}$ as a vector consisting of all multiplier $\lambda_T$.
Let $[\lambda^{(1)}, \Expl(\f_1,\ell)],[\lambda^{(2)},\Expl(\f_2,\ell)] \in \mathbb{R}^{|\mathcal{T}|+ d_\ell}$ be the solution of Eqn.\eqref{eqn:lagrangian2}
( the minimizers of Eqn.\eqref{eqn:constrained_weighted_regresion}) with respect to set functions $\f_1(\cdot)$ and $\f_2(\cdot)$. 

Now we prove that $[\lambda^{(1+2)}, \Expl(\f_{1+2},\ell)] =  [\alpha_1\lambda^{(1)} + \alpha_2 \lambda^{(2)}, \alpha_1\Expl(\f_1,\ell) + \alpha_2 \Expl(\f_2,\ell)]$ is the solution of Eqn.\eqref{eqn:lagrangian2} with respect to the function $\f_{1+2}= \alpha_1 \f_1 + \alpha_2 \f_2$.

First of all, for equation (i), $\lambda$, $\ex(\f,\ell)$ and $\f$ have linear relation. Therefore, we have, for all $A \in \setlessell$, 

\begin{align*}
&-2 \sum_{ \substack{S: S \supseteq A, \\ \mu(S) < \infty}} \mu(S) \f_{1+2}(S) + 2\sum_{S \in \setlessell} \bar{\mu}(S \cup A) \Expl_S(\f_{1+2}, \ell) \\
& = \alpha_1 \left(-2 \sum_{ \substack{S: S \supseteq A, \\ \mu(S) < \infty}} \mu(S) \f_{1}(S) + 2\sum_{S \in \setlessell} \bar{\mu}(S \cup A) \Expl_S(\f_{1}, \ell) \right)  \\
& + \alpha_2 \left(-2 \sum_{ \substack{S: S \supseteq A, \\ \mu(S) < \infty}} \mu(S) \f_{2}(S) + 2\sum_{S \in \setlessell} \bar{\mu}(S \cup A) \Expl_S(\f_{2}, \ell) \right)  \\
& = \alpha_1 \sum_{T: (T \subseteq \mathcal{T} )\wedge (T \supseteq A) } \lambda^{(1)}_T + \alpha_2 \sum_{T:(T \subseteq \mathcal{T} )\wedge (T \supseteq A) } \lambda^{(2)}_T   \\
& = \sum_{T: (T \subseteq \mathcal{T} )\wedge (T \supseteq A) } \lambda^{(1+2)}_T  .
\end{align*}

Secondly, for equation (ii), we also have, for all $A \subseteq \mathcal{T}$,
{ \small
\begin{align*}
& \f_{1+2}(A) - \sum_{T \subseteq A , |T| \leq \ell}\Expl_T(\f_{1+2},\ell) 
& = \alpha_1 \left( \f_1(A) - \sum_{T \subseteq A , |T| \leq \ell}\Expl_T(\f_1,\ell) \right) + \alpha_2 \left( \f_2(A) - \sum_{T \subseteq A , |T| \leq \ell}\Expl_T(\f_2,\ell) \right) 
& = 0.
\end{align*}}

Therefore, $[\lambda^{(1+2)}, \Expl(\f_{1+2},\ell)] =  [\alpha_1\lambda^{(1)} + \alpha_2 \lambda^{(2)}, \  \alpha_1\Expl(\f_1,\ell) + \alpha_2 \Expl(\f_2,\ell)]$ is the solution of Eqn.\eqref{eqn:lagrangian2} with respect to the function $\f_{1+2}= \alpha_1 \f_1 + \alpha_2 \f_2$. Hence, the Faith-Interaction indices satisfy the interaction linearity axiom.
\end{proof}

\subsection{Proof of Proposition \ref{pro:symmetry}}

\subsubsection{Sufficient Condition:}
\begin{proof}
We prove that if the proper weighting functions are permutation invariant, then Faith-Interaction indices $\Expl$ satisfy the interaction symmetry axiom.

Suppose indexes $i$ and $j$ are symmetric with respect to the function $\f$. That is,  $\f(S \cup i) = \f(S \cup j)$ for any set $S \subseteq [d] \backslash \{i,j\}$. Our goal is to prove that indexes $i$ and $j$ in the corresponding explanation are also symmetric, i.e.
$\ex_{S \cup i}(\f,\ell) = \ex_{S \cup j}(\f,\ell)$ for any set $S \subseteq [d] \backslash \{i,j\}$ with $|S| < \ell$. 

By Proposition \ref{pro:unique_minimizer},
Eqn.\eqref{eqn:weighted_regression} has a unique minimizer. The objective function can be written into the following form:

{ \small
\begin{align*}
&  \argmin_{\Expl(\f,\ell) \in \mathbb{R}^{d_\ell}} \sum_{\substack{S \subseteq [d] \\ \mu(S) < \infty}}  \mu(S) \left( \f(S) - \sum_{L \subseteq S , |L| \leq \ell}\Expl_L(\f,\ell) \right)^2  \\
 & = \sum_{\substack{S \subseteq [d] \backslash \{i,j\} \\ \mu(S) < \infty }}  \mu(S) \left( (\f(S) - \sum_{L \subseteq S , |L| \leq \ell}\Expl_L(\f,\ell) \right)^2 + 
 \sum_{\substack{S \subseteq [d] \backslash \{i,j\} \\ \mu(S) < \infty }}  \mu(S \cup i) \left( \f(S \cup i) - \sum_{L \subseteq S \cup i , |L| \leq \ell}\Expl_L(\f,\ell) \right)^2  \\
 & + \sum_{\substack{S \subseteq [d] \backslash \{i,j\}\\ \mu(S) < \infty}}  \mu(S \cup j) \left( \f(S\cup j) - \sum_{L \subseteq S\cup j , |L| \leq \ell}\Expl_L(\f,\ell) \right)^2 \\ 
 & +  \sum_{\substack{S \subseteq [d] \backslash \{i,j\} \\ \mu(S) < \infty}}  \mu(S \cup \{i,j\}) \left( \f(S \cup \{i,j\}) - \sum_{L \subseteq S \cup \{i,j\} , |L| \leq \ell}\Expl_L(\f,\ell) \right)^2 \\
 & \text{ subject to } 
 \f(S) = \sum_{T \subseteq S} \Expl_T(\f,\ell), \ \  \forall \ \  S: \mu(S) = \infty.
\end{align*}}

If $i$ and $j$ in function $\mu(\cdot)$ and $\f(\cdot)$ are interchanged, the above equation becomes

{ \small
\begin{align*}
& \argmin_{\Expl(\f,\ell) \in \mathbb{R}^{d_\ell}} \sum_{S \subseteq [d] \backslash \{i,j\} }  \mu(S) \left( \f(S) - \sum_{L \subseteq S , |L| \leq \ell}\Expl_L(\f,\ell) \right)^2 + 
 \sum_{S \subseteq [d] \backslash \{i,j\} }  \mu(S \cup j) \left( \f(S \cup j) - \sum_{L \subseteq S \cup i , |L| \leq \ell}\Expl_L(\f,\ell) \right)^2  \\
& + \sum_{S \subseteq [d] \backslash \{i,j\} }  \mu(S \cup i) \left( \f(S\cup i) - \sum_{L \subseteq S\cup j , |L| \leq \ell}\Expl_L(\f,\ell) \right)^2 \\
& + 
 \sum_{S \subseteq [d] \backslash \{i,j\} }  \mu(S \cup \{i,j\}) \left( \f(S \cup \{i,j\}) - \sum_{L \subseteq S \cup \{i,j\} , |L| \leq \ell}\Expl_L(\f,\ell) \right)^2 \\
  & \text{ subject to } 
 \f(S) = \sum_{T \subseteq S} \Expl_T(\f,\ell), \ \ \forall \ \  S: \mu(S) = \infty.
\end{align*}}

The equation remains the same since $\mu(S \cup i) = \mu(S \cup j)$  and $\f(S \cup i) = \f(S \cup j)$. Also, the constraints $\f(S) = \sum_{T \subseteq S} \Expl_T(\f,\ell), \ \ \forall \ \  S: \mu(S) = \infty$ remain the same since a proper weighting function is only allowed to have infinity measure on $\mu(\text{\O})$ and $\mu([d])$, which are symmetric to any $i$ and $j$. 

Given that Eqn.\eqref{eqn:weighted_regression} has a unique solution, the above two minimization problems should have the same minimizer. We note that $i$ and $j$ have been interchanged in the set function $\f(\cdot)$ and the weighting function  $\mu$, so $i$ and $j$ should also be symmetric in the minimizer, i.e. $\ex_{S \cup i}(\f,\ell) = \ex_{S \cup j}(\f,\ell)$ for any set $S \subseteq [d] \backslash \{i,j\}$ with $|S| < \ell$. 

\end{proof}

\subsubsection{Necessary Condition}

\begin{proof}
Next, we show that Faith-Interaction indices $\Expl$ satisfy the interaction symmetry axiom only if the proper weighting functions are permutation invariant so that $\mu(S)$ is only a function of $|S|$.

We consider the case when $\ell = d- 1$ and the set function $\f$ is defined as below.
\begin{equation}
\f(S) = \begin{cases}
1  & \text{, if $S = [d]$.} \\
0 & \text{, otherwise.} \\
\end{cases}    
\end{equation}
In this case, $\mathcal{S}_\ell$ consists of all subsets of $[d]$ except for $[d]$. Next, we define a new coalition weighting function $\mu' :2^d \rightarrow \mathbb{R}^{+}$ with 
$$
\mu'(S) =
\begin{cases}
1 & \text{ if } \mu(S) = \infty. \\
\mu(S) & \text{ otherwise.} \\
\end{cases}
$$
We can see that for all $\ex(\f,\ell) \subseteq \mathbb{R}^{d_\ell}$ satisfying  $\f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) =0, \forall S: \mu(S) = \infty, S \subseteq [d]$, the values of objective functions instantiated with $\mu$ and $\mu'$ are the same. That is, 
$$
\sum_{S \subseteq [d]\,:\, \mu(S) < \infty}  \mu(S) \left( \f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) \right)^2
= \sum_{S \subseteq [d]}  \mu'(S) \left( \f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) \right)^2.
$$
Therefore, we can substitute $\mu$ with $\mu'$ and the objective function can be written as 
\begin{align*}
\small
F(\ex) = \sum_{S \subseteq [d]} \mu'(S) \left(\f(S) - \sum_{T \subseteq S, |T| \leq d-1} \Expl_T(\f, \ell)  \right)^2,
\ \text{s.t.} \ & \f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) =0 \;\;,\;\forall S \,:\, \mu(S) = \infty.
\end{align*}
Let $q(S) = \mu'(S) \left(\f(S) - \sum_{T \subseteq S, |T| \leq d-1} \Expl_T(\f, \ell) \right)$ and $p(S) = \sum_{T \supseteq S} q(T)$ for all $S \subseteq [d]$. The partial derivative of $F(\ex)$ with respect to $\ex_L$ is 
$$
\frac{F(\ex)}{\partial \ex_L} 
= -2\sum_{S \supseteq L} \mu'(S) \left(\f(S) - \sum_{T \subseteq S, |T| \leq d-1} \Expl_T(\f, \ell) \right) = -2\sum_{S \supseteq L} q(S) = -2p(L),
$$
where $L \subset [d]$. Before going to the main proof, we first introduce the following claim, which provides a relation between $p(\cdot)$ and $q(\cdot)$.
\begin{claim}
\label{clm:p_q_relation}
For all $S \subseteq [d]$, $q(S) = \sum_{T \supseteq S} (-1)^{|T| - |S|}p(T)$. 
\end{claim}
Also, the following claim states that $p(L)$ for all $L \subseteq [d]$ can not be zero simultaneously. 
\begin{claim}
\label{clm:all_zero}
There is no $\ex(\f,\ell) \in \mathbb{R}^{2^d-1}$ satisfying $p(L) = 0$ for all $L \subseteq [d]$.
\end{claim}
 
With these results in hands, we now prove that 
$q(S_1) = q(S_2)  \neq 0$ for all $S_1, S_2 \subseteq [d]$ with $1 \leq |S_1| = |S_2| \leq d-1$.
Since a proper weighting function is only allowed to have $\mu([d])$ or $\mu(\text{\O})$ to be infinity, we separate the problem into four cases: (1) $\mu(S) < \infty$ for all $S \subseteq [d]$. (2) Only $\mu(\text{\O}) = \infty$. (3) Only $\mu([d]) = \infty$. (4) Only $\mu([d]) = \mu(\text{\O}) = \infty$.

\paragraph{ (1) $\mu(S) < \infty$ for all $S \subseteq [d]$:} 
we solve the minimization problem using partial derivatives:
$$
\frac{F(\ex)}{\partial \ex_S}  = -2p(S) = 0,
\ \text{ for all $S \subset [d]$.}
$$
By Claim \ref{clm:p_q_relation}, for all $S \subset [d]$, we have 
\begin{equation}
\label{eqn:q_p_case1}
q(S) = \sum_{T \supseteq S} (-1)^{|T| - |S|}p(T) = (-1)^{d-|S|}p([d]),
\end{equation}
which implies that $q(S_1) = q(S_2)$ for all $S_1, S_2 \subseteq [d]$ with $1 \leq |S_1| = |S_2| \leq d-1$.

If there exists $q(S) = 0$ for some $S \subset [d]$, then $p([d])$ must also be zero by Eqn.\eqref{eqn:q_p_case1}. Then again by Eqn.\eqref{eqn:q_p_case1}, we have $q(S) = 0$ for all $S \subset [d]$, which is a contradiction by Claim \ref{clm:all_zero}.

\paragraph{ (2) Only $\mu(\text{\O}) = \infty$:} in this case, the only constraint is $q(\text{\O}) = \f(\text{\O}) - \ex_{\text{\O}}(\f,\ell) = 0$, which implies $\ex_{\text{\O}}(\f,\ell) = f(\text{\O})$. Then
we solve the minimization problem using partial derivatives:
$$
\frac{F(\ex)}{\partial \ex_S}  = -2p(S) = 0,
\ \text{ for all $S \subset [d]$ with $ 0 <|S| \leq d-1$.}   
$$
By Claim \ref{clm:p_q_relation}, we have 
\begin{equation}
\label{eqn:q_p_case2}
q(S) = \sum_{T \supseteq S} (-1)^{|T| - |S|}p(T) = (-1)^{d-|S|}p([d]),
\ \text{ for all $S \subset [d]$ with $ 0 <|S| \leq d-1$,}   
\end{equation}
which implies that $q(S_1) = q(S_2)$ for all $S_1, S_2 \subseteq [d]$ with $1 \leq |S_1| = |S_2| \leq d-1$.

If there exists $q(S) = 0$ for some $S \subset [d]$, then $p([d])$ must also be zero by Eqn.\eqref{eqn:q_p_case2}. Then again by Eqn.\eqref{eqn:q_p_case2}, we have $q(S) = 0$ for all $S \subset [d]$ with $ 0 < |S| \leq d-1$. Also, the constraint implies that $q(\text{\O}) = 0$. By Claim \ref{clm:all_zero}, we can not have $q(S) = 0$ for all $S \subseteq [d]$, which is a contradiction.


\paragraph{(3) Only $\mu([d]) = \infty$:} in this case, the only constraint is $q([d]) = \f([d]) - \sum_{T \subseteq [d]} \ex_{T}(\f,\ell) = 0$. Then
we solve the constrained minimization problem using a Lagrange multiplier.
$$
\frac{F(\ex)}{\partial \ex_S}  = -2p(S) = \lambda,
\ \text{ for all $S \subset [d]$ with $ 0 \leq |S| \leq d-1$.}   
$$
By Claim \ref{clm:p_q_relation}, for all $S \subset [d]$ with $ 0 \leq |S| \leq d-1$, we have 
\begin{align}
q(S) & = \sum_{T \supseteq S} (-1)^{|T| - |S|}p(T)  \nonumber \\
& = (-1)^{d-|S|}p([d]) + \sum_{T \supseteq S} (-1)^{|T| - |S|} \frac{-\lambda}{2} \nonumber \\
& = (-1)^{d-|S|}p([d]) -\frac{\lambda}{2} \times \left[(1-1)^{d -|S|} - (-1)^{d-|S|} \right] \nonumber \\
& = (-1)^{d-|S|}p([d]) +\frac{\lambda}{2}  (-1)^{d-|S|} \nonumber \\
& = \frac{\lambda}{2}  (-1)^{d-|S|} 
\ \ \ (p([d]) = q([d]) = 0)
\label{eqn:q_p_case3}
\end{align}
which implies that $q(S_1) = q(S_2)$ for all $S_1, S_2 \subseteq [d]$ with $1 \leq |S_1| = |S_2| \leq d-1$.

If there exists $q(S) = 0$ for some $S \subset [d]$ with $0 \leq |S| \leq d-1$, then we have $\lambda = 0$ by Eqn.\eqref{eqn:q_p_case3}. Then again by Eqn.\eqref{eqn:q_p_case3}, we have $q(S) = 0$ for all $S \subset [d]$ with $ 0 \leq |S| \leq d-1$. Also, the constraint implies that $q([d]) = 0$. By Claim \ref{clm:all_zero}, we can not have $q(S) = 0$ for all $S \subseteq [d]$, which is a contradiction.



\paragraph{(4) Only $\mu(\text{\O}) = \mu([d]) = \infty$:} in this case, the constraints are $q(\text{\O}) = \f(\text{\O}) - \ex_{\text{\O}} = 0$ and $q([d]) = \f([d]) - \sum_{T \subseteq [d]} \ex_{T}(\f,\ell) = 0$. Then
we solve the constrained minimization problem using a Lagrange multiplier.
$$
\frac{F(\ex)}{\partial \ex_S}  = -2p(S) = \lambda,
\ \text{ for all $S \subset [d]$ with $ 1 \leq |S| \leq d-1$.}   
$$
By Claim \ref{clm:p_q_relation}, for all $S \subset [d]$ with $ 1 \leq |S| \leq d-1$, we have 
\begin{align}
q(S) & = \sum_{T \supseteq S} (-1)^{|T| - |S|}p(T)  \nonumber \\
& = (-1)^{d-|S|}p([d]) + \sum_{T \supseteq S} (-1)^{|T| - |S|} \frac{-\lambda}{2} \nonumber \\
& = (-1)^{d-|S|}p([d]) -\frac{\lambda}{2} \times \left[(1-1)^{d -|S|} - (-1)^{d-|S|} \right] \nonumber \\
& = (-1)^{d-|S|}p([d]) +\frac{\lambda}{2}  (-1)^{d-|S|} \nonumber \\
& = \frac{\lambda}{2}  (-1)^{d-|S|} 
\ \ \ (p([d]) = q([d]) = 0)
\label{eqn:q_p_case4}
\end{align}
which implies that $q(S_1) = q(S_2)$ for all $S_1, S_2 \subseteq [d]$ with $1 \leq |S_1| = |S_2| \leq d-1$.

If there exists $q(S) = 0$ for some $S \subset [d]$ with $1 \leq |S| \leq d-1$, then we have $\lambda = 0$ by Eqn.\eqref{eqn:q_p_case4}. Then again by Eqn.\eqref{eqn:q_p_case4}, we have $q(S) = 0$ for all $S \subset [d]$ with $ 1 \leq  |S| \leq d-1$. Also, the constraint implies that $q(\text{\O}) = q([d]) = 0$. By Claim \ref{clm:all_zero}, we can not have $q(S) = 0$ for all $S \subseteq [d]$, which is a contradiction.

By summarizing (1)$\sim$(4), we conclude that $q(S_1) = q(S_2)  \neq 0$ for all $S_1, S_2 \subseteq [d]$ with $1 \leq |S_1| = |S_2| \leq d-1$. That is,
$$
\mu'(S_1) 
\underbrace{\left(\f(S_1) - \sum_{T_1 \subseteq S_1, |T_1| \leq d-1} \Expl_{T_1}(\f, \ell) \right)}_{(i)}
= \mu'(S_2) 
\underbrace{\left(\f(S_2) - \sum_{T_2 \subseteq S_2, |T_2| \leq d-1} \Expl_{T_2}(\f, \ell) \right)}_{(ii)}.
$$
Since $\f(\cdot)$ is symmetric by definition ( only depends on its input size) and the minimizer $\Expl(\f, \ell) $ satisfies the interaction symmetry axiom, we get that 
the mimimizer $\Expl_{T_1}(\f, \ell) = \Expl_{T_2}(\f, \ell) $ for all $|T_1| = |T_2|$.  Therefore, each term in $(i)$ and $(ii)$ have one-to-one correspondence. We have $(i)=(ii)$ and we can simplify the above equation: 
$$
\left(\mu'(S_1) - \mu'(S_2) \right) \times \left(\f(S_1) - \sum_{T_1 \subseteq S_1, |T_1| \leq d-1} \Expl_{T_1}(\f, \ell)  \right) 
= 0,
$$
Since the value in the second bracket is nonzero ($q(S_1) \neq 0$), we can conclude that $\mu'(S_1) = \mu'(S_2)$ for all $S_1, S_2 \subseteq [d]$ with $1 \leq |S_1| = |S_2| \leq d-1$. Also, by definition of $\mu'()$, we have $\mu(S) = \mu'(S)$ for all $S \subseteq [d]$ with $1 \leq |S| \leq d-1$. Therefore, we conclude the weighting function $\mu(\cdot)$ is also symmetric.

\end{proof}

\subsection{Proof of Proposition \ref{pro:dummy}}
\begin{proof}


The minimization problem can be written as follows:
\begin{equation*}
\small
\ex(\f,\ell) = \min_{\Expl \in \mathbb{R}^{d_\ell}} F_\ell(\f,\ex) = \min \sum_{S \subseteq [d]} \mu(S) \left(
\f(S) - \sum_{T \subseteq S, |T| \leq \ell} \Expl_T(\f, \ell)  \right)^2,
\end{equation*}
Without loss of generality, let $\mu(S) = \prod_{j \in S} p_j \prod_{k \not \in S} (1-p_k)$ for some $0 < p_j < 1$.

Now, we prove the minimizer of the above equation satisfies interaction dummy axiom.  More generally, we prove that the minimization problem with a dummy feature can be reduced to another problem with only $d-1$ features and the interaction terms containing the dummy feature is zero.
Formally, we have the following lemma:
\begin{lemma}
\label{lm:dummt_reduce}
Assume that $i^{\text{th}}$ feature of the set function $\f(\cdot)$ is a dummy feature such that $\f(S) = \f(S \cup i)$ for all $S \subseteq [d] \backslash \{i\}$.
Let $\f':2^{d-1} \mapsto \mathbb{R}$ with $\f'(S) = \f(S)$ for all $S \subseteq [d-1]$. Then we have 
\begin{equation}
\label{eqn:dummy_solution}
\begin{cases}
\Expl_{S}(\f,\ell) = \Expl_{S}(\f',\ell), 
& \text{ for all }  \ \ S \subseteq [d] \backslash \{ i\}, 0 \leq |S| \leq \ell. \\
\Expl_{S \cup \{i\}}(\f,\ell) = 0, & \text{ for all }  \ \ S \subseteq [d] \backslash \{ i\}, 0 \leq |S| \leq \ell - 1. 
\end{cases}
\end{equation}
where $\Expl_{S}(\f',\ell)$ is the minimizer of the following problem:
$$
\min \sum_{S \subseteq [d]\backslash i} \mu'(S) \left(
\f'(S) - \sum_{T \subseteq S, |T| \leq \ell} \Expl'_T(\f, \ell)  \right)^2,
\text{ with }
\mu'(S) = \prod_{j \in S} p_j \prod_{k \in [d-1] \backslash S} (1-p_k).
$$
\end{lemma}

\begin{proof}
Without loss of generality, we assume that $d^{th}$ feature is a dummy feature, such that $\f(S \cup d) = \f(S)$ for all $S \subseteq [d-1]$.
Now, we solve the minimization problem  by partial derivatives. 
\begin{equation}
\frac{\partial \ F_\ell(\f,\ex)}{\partial \Expl_S } = 0  \text{  for all  } S \subseteq [d-1], |S| \leq \ell.
\end{equation}
We note that the partial derivative can be calculated as below:
$$
\frac{\partial \ F_\ell(\f,\ex)}{\partial \Expl_S } 
= -2\sum_{T \supseteq S} \mu(T) \left(\f(T) - \sum_{L \subseteq T, |L| \leq \ell} \ex_L(\f,\ell) 
\right)
= 0
\text{  for all  } S \subseteq [d-1], |S| \leq \ell.
$$
Now, for convenience, we denote 
$q(T) = \f(T) - \sum_{L \subseteq T, |L| \leq \ell} \ex_L(\f,\ell)$ for all $T \subseteq [d]$. Then $\ex(\f,\ell)$ satisfies the following equalities:
\begin{equation}
\label{eqn:partial_derivative_dummy}
\sum_{T \supseteq S} \mu(T)q(T) = 0,
\text{  for all  } S \subseteq [d-1], |S| \leq \ell.    
\end{equation}

Similarly, the minimizer $\ex(\f',\ell)$ of $F_\ell(\f',\ex)$ satisfies 
\begin{equation}
\label{eqn:partial_derivative_dummy_prime}\sum_{T: S \subseteq T \subseteq [d-1]} \mu'(T)q'(T) = 0,
\text{  for all  } S \subseteq [d-1], |S| \leq \ell,
\end{equation}
where $q':2^{d-1} \mapsto \mathbb{R}$ with $q'(T) = \f'(T) - \sum_{L \subseteq T, |L| \leq \ell} \ex_L(\f',\ell)$ for all $T \subseteq [d-1]$.

By the definitions of weighting function $\mu(\cdot)$ and $\mu'(\cdot)$, we have 
\begin{equation}
\label{eqn:mu_dummy_property}
\mu(S) = (1-p_d)\mu'(S),
\text{ and }
\mu(S \cup d) = p_d\mu'(S), 
\text{ for all }
S \subseteq [d-1].
\end{equation}
Also, since we have $\ex_L(\f,\ell) = 0$ for all $L$ containing $\{d\}$ and $ \f(T) = \f(T \cup \{ d\})$ ( Eqn.\eqref{eqn:dummy_solution}), for all $T \subseteq [d-1]$, we have 
\begin{equation}
\label{eqn:q_dummy_property1}
q(T \cup \{ d\}) 
= \f(T \cup \{ d\}) - \sum_{L \subseteq T \cup \{ d\}, |L| \leq \ell} \ex_L(\f,\ell) 
= \f(T) - \sum_{L \subseteq T, |L| \leq \ell} \ex_L(\f,\ell) 
= q(T),    
\end{equation}
and
\begin{equation}
\label{eqn:q_dummy_property2}
q'(T) 
= \f'(T) - \sum_{L \subseteq T, |L| \leq \ell} \ex_L(\f',\ell) 
= \f(T) - \sum_{L \subseteq T, |L| \leq \ell} \ex_L(\f,\ell) 
= q(T) = q(T \cup \{ d\}). 
\end{equation}
Now, we prove that $\ex(\f,\ell)$ defined in Eqn.\eqref{eqn:dummy_solution} satisfies the system of linear equations in Eqn.\eqref{eqn:partial_derivative_dummy}.

(1) For all $S \subseteq [d-1]$ with $0 \leq |S| \leq \ell$, we have

\begin{align*}
\sum_{T: S \subseteq T \subseteq [d]} \mu(T) q(T) 
& =  \sum_{T: S \subseteq T \subseteq [d-1]} \mu(T) q(T)
+ \sum_{T: S \subseteq T \subseteq [d-1]} \mu(T \cup \{ d\}) q(T\cup \{ d\}) \\
& = \sum_{T: S \subseteq T \subseteq [d-1]} \left(\mu(T) +\mu(T \cup \{ d\}) \right) q(T) \ \ \text{( Using Eqn.\eqref{eqn:q_dummy_property1} )} \\
& =  \sum_{T: S \subseteq T \subseteq [d-1]} \mu'(T) q(T) \ \
\text{( Using Eqn.\eqref{eqn:mu_dummy_property} )} \\
& = \sum_{T: S \subseteq T \subseteq [d-1]} \mu'(T) q'(T) \ \ 
\text{(Using Eqn.\eqref{eqn:q_dummy_property2} )} \\
&  = 0  \ \ 
(\text{Eqn.\eqref{eqn:partial_derivative_dummy_prime}}).
\end{align*} 

(2) For all $S \subseteq [d]$ containing $\{ d\}$ with $ 1 \leq |S| \leq \ell$, we have 
\begin{align*}
\sum_{T: S \subseteq T \subseteq [d]} \mu(T) q(T)
& = \sum_{T: (S\backslash \{d\}) \subseteq T \subseteq [d-1]} \mu(T \cup \{d\} ) q(T \cup \{d\}) \\
& = \sum_{T: (S\backslash \{d\}) \subseteq T \subseteq [d-1]} p_d \mu'(T) q'(T) \ \ \text{(Using Eqn.\eqref{eqn:mu_dummy_property} and Eqn.\eqref{eqn:q_dummy_property2})} \\
& = p_d \sum_{T: (S\backslash \{d\}) \subseteq T \subseteq [d-1]} \mu'(T) q'(T)  \\
& = 0 
\ \ \text{ (By Eqn.\eqref{eqn:partial_derivative_dummy_prime})} \\
\end{align*}
Therefore, combining (1) and (2), we have 
$$
\sum_{T: S \subseteq T \subseteq [d]} \mu(T) q(T) = 0 \text{  for all  }
S \subseteq [d], \text{ with } |S| \leq \ell.
$$
That is, Eqn.\eqref{eqn:dummy_solution} is the minimizer of the minimization problem. Consequently, the minimizer satisfies interaction dummy axiom for all $1 \leq \ell \leq d$.
\end{proof}

\end{proof}


\subsection{Proof of Proposition \ref{pro:efficiency}}
\begin{proof}

\textbf{Sufficient condition:} first of all, we prove that if the proper weighting functions have $\mu(\text{\O}) = \mu([d]) = \infty$, the Faith-Interaction indices satisfy the interaction efficiency axiom. 

By Proposition \ref{pro:unique_minimizer}, the constrained minimization problem has a unique minimizer. Also, the constraints ensures that $\f([d]) = \sum_{T \subseteq [d], |T| \leq \ell} \ex_T(\f,\ell)$ and $\f(\text{\O}) = \ex_{\text{\O}}(\f,\ell)$. Therefore, the minimizer (or the Faith-Interaction indices) satisfies the interaction efficiency axiom.

\textbf{Necessary condition:} we prove that if the Faith-Interaction indices satisfy the interaction efficiency axiom, the corresponding weighting function must satisfy $\mu(\text{\O}) = \mu([d]) = \infty$.

We consider the case when $\ell = d-1$ and the set function $\f$ is defined as below.
\begin{equation}
\f(S) = \begin{cases}
1  & \text{, if $S = [d]$.} \\
0 & \text{, otherwise.} \\
\end{cases}    
\end{equation}
In this case, $\mathcal{S}_\ell$ consists of all subsets of $[d]$ except for $[d]$. We will prove that $\ex(\f,d-1)$ satisfies the interaction efficiency axiom only if $\mu(\text{\O}) = \mu([d]) = \infty$.

First, we define a new coalition weighting function $\mu' :2^d \rightarrow \mathbb{R}^{+}$ with 
$$
\mu'(S) =
\begin{cases}
1 & \text{ if } \mu(S) = \infty. \\
\mu(S) & \text{ otherwise.} \\
\end{cases}
$$
We can see that for all $\ex(\f,\ell) \subseteq \mathbb{R}^{d_\ell}$ satisfying  $\f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) =0, \forall S: \mu(S) = \infty, S \subseteq [d]$, the values of objective functions instantiated with $\mu$ and $\mu'$ are the same. That is, 
$$
\sum_{S \subseteq [d]\,:\, \mu(S) < \infty}  \mu(S) \left( \f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) \right)^2
= \sum_{S \subseteq [d]}  \mu'(S) \left( \f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) \right)^2.
$$
Therefore, we can substitute $\mu$ with $\mu'$ and the objective function can be written as 
\begin{align*}
F(\ex) = \sum_{S \subseteq [d]} \mu'(S) \left(\f(S) - \sum_{T \subseteq S, |T| \leq d-1} \Expl_T(\f, \ell)  \right)^2,
\ \text{s.t.} \ & \f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) =0 \;\;,\;\forall S \,:\, \mu(S) = \infty.
\end{align*}

Let $q(S) = \mu'(S) \left(\f(S) - \sum_{T \subseteq S, |T| \leq d-1} \Expl_T(\f, \ell) \right)$ and $p(S) = \sum_{T \supseteq S} q(T)$ for all $S \subseteq [d]$. The partial derivative of $F(\ex)$ with respect to $\ex_L$ is 
$$
\frac{F(\ex)}{\partial \ex_L} 
= -2\sum_{S \supseteq L} \mu'(S) \left(\f(S) - \sum_{T \subseteq S, |T| \leq d-1} \Expl_T(\f, \ell) \right) = -2\sum_{S \supseteq L} q(S) = -2p(L),
$$
where $L \subset [d]$. Recall that Claim \ref{clm:p_q_relation} in the proof of Proposition \ref{pro:symmetry} states that 
\begin{equation}
\label{eqn:p_q_relation}
q(S) = \sum_{T \supseteq S} (-1)^{|T| - |S|}p(T), \text{ for all $S \subseteq [d]$ }.
\end{equation}

Also, Claim \ref{clm:all_zero} ensures that $p(L)$ for all $L \subseteq [d]$ can not be zero simultaneously:
\begin{equation}
\label{eqn:all_zero}
\text{ There is no $\ex(\f,\ell) \in \mathbb{R}^{2^d-1}$ satisfying $p(L) = 0$ for all $L \subseteq [d]$.}
\end{equation}
 
With these results in hands, we now prove that 
we must have $\mu(\text{\O}) = \mu([d]) = \infty$. Otherwise, we will have $q([d]) \neq 0$ or $q(\text{\O}) \neq 0$.
Since a proper weighting function is only allowed to have $\mu([d])$ or $\mu(\text{\O})$ to be infinity, we only need to discuss three cases: (1) $\mu(S) < \infty$ for all $S \subseteq [d]$. (2) Only $\mu(\text{\O}) = \infty$. (3) Only $\mu([d]) = \infty$. 

\paragraph{ (1) $\mu(S) < \infty$ for all $S \subseteq [d]$:} 
we solve the minimization problem using partial derivatives:
$$
\frac{F(\ex)}{\partial \ex_S}  = -2p(S) = 0,
\ \text{ for all $S \subset [d]$ with $ 0 \leq |S| \leq d-1$.}   
$$
By Claim \ref{clm:p_q_relation}, for all $S \subset [d]$, we have 
\begin{equation}
\label{eqn:q_p_case1_eff}
q(S) = \sum_{T \supseteq S} (-1)^{|T| - |S|}p(T) = (-1)^{d-|S|}p([d]),
\ \text{ for all $S \subset [d]$ with $ 0 \leq |S| \leq d-1$.}   
\end{equation}

If $q(\text{\O}) = 0$, then $p([d])$ must also be zero by Eqn.\eqref{eqn:q_p_case1_eff}. Then again by Eqn.\eqref{eqn:q_p_case1_eff}, we have $q(S) = 0$ for all $S \subset [d]$, which is a contradiction by Claim \ref{clm:all_zero}.

\paragraph{ (2) Only $\mu(\text{\O}) = \infty$:} in this case, the only constraint is $q(\text{\O}) = \f(\text{\O}) - \ex_{\text{\O}}(\f,\ell) = 0$, which implies $\ex_{\text{\O}}(\f,\ell) = f(\text{\O})$. Then
we solve the minimization problem using partial derivatives:
$$
\frac{F(\ex)}{\partial \ex_S}  = -2p(S) = 0,
\ \text{ for all $S \subset [d]$ with $ 0 <|S| \leq d-1$.}   
$$
By Claim \ref{clm:p_q_relation}, we have 
\begin{equation}
\label{eqn:q_p_case2_eff}
q(S) = \sum_{T \supseteq S} (-1)^{|T| - |S|}p(T) = (-1)^{d-|S|}p([d]),
\ \text{ for all $S \subset [d]$ with $ 0 <|S| \leq d-1$.}   
\end{equation}

If $q([d]) = 0$, then by Eqn.\eqref{eqn:q_p_case2_eff}, we have $q(S) = 0$ for all $S \subset [d]$ with $ 0 < |S| \leq d-1$. Also, the constraint implies that $q(\text{\O}) = 0$. By Claim \ref{clm:all_zero}, we can not have $q(S) = 0$ for all $S \subseteq [d]$, which is a contradiction.


\paragraph{(3) Only $\mu([d]) = \infty$:} in this case, the only constraint is $q([d]) = \f([d]) - \sum_{T \subseteq [d]} \ex_{T}(\f,\ell) = 0$. Then
we solve the constrained minimization problem using a Lagrange multiplier.
$$
\frac{F(\ex)}{\partial \ex_S}  = -2p(S) = \lambda,
\ \text{ for all $S \subset [d]$ with $ 0 \leq |S| \leq d-1$.}   
$$
By Claim \ref{clm:p_q_relation}, for all $S \subset [d]$ with $ 0 \leq |S| \leq d-1$, we have 
\begin{align}
q(S) & = \sum_{T \supseteq S} (-1)^{|T| - |S|}p(T)  \nonumber \\
& = (-1)^{d-|S|}p([d]) + \sum_{T \supseteq S} (-1)^{|T| - |S|} \frac{-\lambda}{2} \nonumber \\
& = (-1)^{d-|S|}p([d]) -\frac{\lambda}{2} \times \left[(1-1)^{d -|S|} - (-1)^{d-|S|} \right] \nonumber \\
& = (-1)^{d-|S|}p([d]) +\frac{\lambda}{2}  (-1)^{d-|S|} \nonumber \\
& = \frac{\lambda}{2}  (-1)^{d-|S|} 
\ \ \ (\text{ By } p([d]) = q([d]) = 0).
\label{eqn:q_p_case3_eff}
\end{align}

If $q(\text{\O}) = 0$, then we have $\lambda = 0$ by Eqn.\eqref{eqn:q_p_case3_eff}. Then again by Eqn.\eqref{eqn:q_p_case3_eff}, we have $q(S) = 0$ for all $S \subset [d]$ with $ 0 \leq |S| \leq d-1$. Also, the constraint implies that $q([d]) = 0$. By Claim \ref{clm:all_zero}, we can not have $q(S) = 0$ for all $S \subseteq [d]$, which is a contradiction.


Let come back to the main proof of Proposition \ref{pro:efficiency}. By summarizing (1)$\sim$(3), we do not have $q(\text{\O}) = q([d])= 0$ and $\ex(\f,d-1)$ does not satisfy the interaction efficiency axiom in these cases. Therefore, the proper weighting function must have $\mu(\text{\O}) = \mu([d]) = \infty$.

\end{proof}


\subsection{Proof of Proposition \ref{pro:faith_shap_cardinal_prob}}

\begin{proof}
By Theorem \ref{thm:faith_shap}, for all $S \subseteq [d]$ with $|S| = \ell$, we have 
$$
\ex^{\text{F-Shap}}_{S}(\f,\ell) 
= \frac{(2\ell -1)!}{((\ell-1)!)^2} \sum_{T \subseteq [d] \backslash S} \frac{(\ell+|T|-1)!(d-|T|-1)!}{ (d+\ell-1)!} \Delta_S(\f(T))
= \sum_{T \subseteq [d] \backslash S} p^\ell_{|T|} \Delta_S(\f(T)).
$$
We next show that $\sum_{t=0}^{d-\ell} {d-\ell \choose t} p^\ell_t = 1$. The following derivation is based on the following property of beta functions:
$$
B(\alpha,\beta) = \int_{x=0}^1 x^{\alpha-1}(1-x)^{\beta-1} dx = \frac{(\alpha-1)!(\beta-1)!}{(\alpha+\beta-1)!}
\text{ for all } \alpha, \beta \in \mathbb{N}.
$$
Then we have
\begin{align*}
\sum_{t=0}^{d-\ell} {d-\ell \choose t} p^\ell_t 
& = \sum_{t=0}^{d-\ell} {d-\ell \choose t}\frac{(2\ell -1)!(\ell+t-1)!(d-t-1)!}{((\ell-1)!)^2 (d+\ell-1)!} \\
& = \frac{(2\ell -1)!}{((\ell-1)!)^2} \sum_{t=0}^{d-\ell} {d-\ell \choose t} \int_{x=0}^1 x^{\ell+t-1}(1-x)^{d-t-1} dx  \\
& \ \ (\text{ Using the definition of Beta function } B(\ell+t,d-t) ) \\
& = \frac{(2\ell -1)!}{((\ell-1)!)^2} \int_{x=0}^1  x^{\ell-1}(1-x)^{\ell-1}\sum_{t=0}^{d-\ell} {d-\ell \choose t}  x^{t}(1-x)^{d-\ell-t} dx  \\
& = \frac{(2\ell -1)!}{((\ell-1)!)^2} \int_{x=0}^1  x^{\ell-1}(1-x)^{\ell-1}\left(x + (1 -x)\right)^{d-\ell} dx  \\
& = \frac{(2\ell -1)!}{((\ell-1)!)^2} \int_{x=0}^1  x^{\ell-1}(1-x)^{\ell-1} dx  \\
& = \frac{(2\ell -1)!}{((\ell-1)!)^2} B(\ell,\ell) \\
& = 1.
\end{align*}
\end{proof}


\subsection{Proof of Proposition \ref{pro:faith_shap_path_integral}}

Again, we use the following property of beta functions.
$$
B(\alpha,\beta) = \int_{x=0}^1 x^{\alpha-1}(1-x)^{\beta-1} dx = \frac{(\alpha-1)!(\beta-1)!}{(\alpha+\beta-1)!}
\text{ for all } \alpha, \beta \in \mathbb{N}.
$$
Also, we have the following equalities \citet{hammer2012boolean}.
$$
g(x) = \sum_{T \subseteq [d]} a(\f,T) \prod_{i \in T} x_i,
\text{ and }
\Delta_S g(x) = \sum_{T \supseteq S} a(\f,T) \prod_{i \in T\backslash S} x_i,
$$
where $a(\f,\cdot)$ is the Mobius transform of $\f$.

Then for all $S \in \setlessell$ with $|S| = \ell$, we have
\begin{align*}
\int_{x=0}^1 \Delta_S g(x,\cdots,x) dI_x(\ell,\ell)
& = \frac{1}{B(\ell,\ell)} \int_{x=0}^1 x^{\ell-1}(1-x)^{\ell-1} \Delta_S g(x,\cdots,x) dx \\
& = \frac{1}{B(\ell,\ell)} \int_{x=0}^1 x^{\ell-1}(1-x)^{\ell-1} \sum_{W \supseteq S} \left(
a(\f,W) \prod_{i \in W \backslash S }x \right) dx \\
& = \frac{1}{B(\ell,\ell)} \int_{x=0}^1 x^{\ell-1}(1-x)^{\ell-1} \sum_{U \subseteq [d] \backslash S} \left(
a(\f,U \cup S) x^{|U|} \right) dx  \\
& \,\, (\text{ by setting } U = W \backslash S) \\
& = \frac{1}{B(\ell,\ell)} \sum_{U \subseteq [d] \backslash S} a(\f,U \cup S) \int_{x=0}^1 x^{\ell+|U|-1}(1-x)^{\ell-1}  dx \\
& = \frac{1}{B(\ell,\ell)} \sum_{U \subseteq [d] \backslash S}  \frac{(\ell+|U|-1)!(\ell-1)!}{(2\ell+|U|-1)!} a(\f,U \cup S)\\
& = \frac{1}{B(\ell,\ell)} \sum_{T \supseteq  S} \frac{(|T|-1)!(\ell-1)!}{(|T|+\ell-1)!}  a(\f,T)\\
& = 
a(\f,S) + (-1)^{\ell - |S| }\frac{|S|}{\ell + |S|} {\ell \choose |S| } \sum_{T \supset S, |T| > \ell} \frac{ {|T| - 1 \choose \ell }}{ { |T| + \ell -1 \choose \ell + |S|}} a(\f,T) \\
& = \ex^{\text{F-Shap}}_S(\f,\ell)
\ \ (\text{ by Eqn.\eqref{eqn:faith_shapley}}).
\end{align*}


\subsection{Proof of Proposition \ref{pro:ab_condition}}
In this proof, we use the notation of cumulative weighting function introduced in Definition \ref{def:cumulative_weighting} and the notation of $D^p_q$ in Definition \ref{def:Dpq}. 

Also, we utilize the results in the proof of Claim \ref{clm:mubar_closeform} in Section \ref{sec:clm_d_linear_relation}, where we show that there exists constants $ c^{(1)}_q , c^{(2)}_q,  c^{(3)}_q \in \mathbb{R}$ for $1 \leq q \leq d$ such that 
$$ \frac{D^{p}_{q}}{D^{p}_{q+1}} = c^{(1)}_q p +  c^{(2)}_q \text{ and } \frac{D^{p+1}_{q}}{D^{p}_{q+1}} =  c^{(1)}_q  p +  c^{(3)}_q
\ \text{ for } \ 0 \leq p \leq d-q-1.$$ 

Moreover, the relation between constants can be obtained recursively on $q$:
\begin{equation}
\label{eqn:ABC0}
c^{(1)}_0 = \frac{b-a^2}{(1-a)(a-b)} 
\ \ , c^{(2)}_0 = \frac{a-b}{(1-a)(a-b)}
\ \ , c^{(3)}_0= \frac{a(a-b)}{(1-a)(a-b)} ,
\end{equation}
and 
\begin{equation}
\label{eqn:abc_q_relation}
c^{(1)}_{q+1} = \frac{c^{(1)}_q}{c^{(1)}_q + c^{(2)}_q - c^{(3)}_q},
\ \ c^{(2)}_{q+1} = \frac{c^{(1)}_q + c^{(2)}_q}{c^{(1)}_q + c^{(2)}_q - c^{(3)}_q},
\ \ c^{(3)}_{q+1}=  \frac{c^{(3)}_q}{c^{(1)}_q + c^{(2)}_q - c^{(3)}_q}.
\end{equation}

Now we come back to the proof of Proposition \ref{pro:ab_condition}.
We first show that $c^{(1)}_q \geq 0 ,c^{(2)}_q >0$ and $c^{(3)}_q > 0$ for $q=0,1,2...,d$.
From Eqn. \eqref{eqn:ABC0}, by using the condition $1 > a > b \geq a^2 > 0$, we have 
$$
c^{(1)}_0 = \frac{b-a^2}{(1-a)(a-b)} \geq 0, 
\ \ c^{(2)}_0 = \frac{a-b}{(1-a)(a-b)} > 0, 
\ \ c^{(3)}_0= \frac{a(a-b)}{(1-a)(a-b)} > 0.
$$
Then, since $c^{(2)}_0 - c^{(3)}_0 = 1$ and $c^{(2)}_{q+1} - c^{(3)}_{q+1} = \frac{c^{(1)}_q + c^{(2)}_q - c^{(3)}_q}{c^{(1)}_q+c^{(2)}_q-c^{(3)}_q} = 1$ from Eqn.\eqref{eqn:abc_q_relation}, we get that the denominators of $c^{(1)}_{q+1},c^{(2)}_{q+1}$ and  $c^{(3)}_{q+1}$ are positive.
Then we get that $c^{(1)}_q \geq 0 ,c^{(2)}_q >0$ and $c^{(3)}_q > 0$ for $q=0,2...,d$. Since the ratio $D^{p}_q / D^p_{q+1} >0$ is positive and $D^p_0 = \mubar{p} > 0$ by Lemma \ref{clm:mubar_closeform}, we  conclude that $D^p_q > 0$ for all $p,q$ with $0 \leq p+q \leq d$.

Lastly, we note that $\mu_p = \sum_{j=p}^{d} (-1)^{j-p}{d-p \choose j-p } \mubar{j} =  D^p_{d-p} > 0$ for $0 \leq p \leq d$ by Claim \ref{clm:mubar_mu_relation}. Therefore, we get that $\mu(S) > 0$ for all $S \subseteq [d]$.


\newpage

\subsection{Proof of Proposition \ref{pro:guideline_ab} }
We first transform the ratios into the form of cumulative weighting functions as in Definition \ref{def:cumulative_weighting}.
$$
\frac{\mubar{d}}{\mubar{d-1}}
= \frac{\mu_d}{\mu_d + \mu_{d-1}}
= \frac{r_1}{r_1+1}
\ \ \text{ and }\ \ 
\frac{\mubar{d-1}}{\mubar{d-2}}
= \frac{\mu_d + \mu_{d-1}}{\mu_d + 2\mu_{d-1} + \mu_{d-2}}
= \frac{r_1r_2 + r_2}{1+2r_2+r_1r_2} 
$$
By Claim \ref{clm:mubar_closeform}, we have 
$$
\frac{\mubar{d}}{\mubar{d-1}} 
= \frac{a(a-b)+(d-1)(b-a^2)}{(a-b)+(d-1)(b-a^2)} 
= \frac{A + d-1}{B+d-1}
\ \ \text{ and }\ \ 
\frac{\mubar{d-1}}{\mubar{d-2}}
= \frac{a(a-b)+(d-2)(b-a^2)}{(a-b)+(d-2)(b-a^2)} 
= \frac{A + d-2}{B+d-2},
$$
where we let $A = \frac{a^2-ab}{b-a^2}$ and $B = \frac{a-b}{b-a^2}$. Next, by combining the above equations, we can solve $A$ and $B$ in terms of $r_1$ and $r_2$.

\begin{align*}
1 & = (A+d-1) - (A+d-2) = \frac{\mubar{d}}{\mubar{d-1}} (B+d-1)
- \frac{\mubar{d-1}}{\mubar{d-2}} (B+d-2)
\end{align*}
$$ \Rightarrow 
B = -(d-1) + \frac{1 - \frac{\mubar{d-1}}{\mubar{d-2}}}
{\frac{\mubar{d}}{\mubar{d-1}} - \frac{\mubar{d-1}}{\mubar{d-2}}}
= -(d-1) + \frac{(r_1+1)(r_2+1)}{r_1 - r_2}
$$
Similarly, we get
$$ 
A = -(d-1) + \frac{1 - \frac{\mubar{d-1}}{\mubar{d-2}}}
{1 - \frac{\mubar{d-1}}{\mubar{d}} \times \frac{\mubar{d-1}}{\mubar{d-2}}}
= -(d-1) + \frac{r_1(r_2+1)}{r_1 - r_2}.
$$
Next, by solving $A$ and $B$ in terms of $a$ and $b$, we get
$$
a  =  \frac{A}{B} 
\ \ \text{ and } \ \ 
b = \frac{A}{B} \times \frac{A+1}{B+1}.
$$
By plugging $A$ and $B$ into the above equation, we get the form of $a$ and $b$ in terms of $r_1$ and $r_2$:
$$
a = \frac{ r_1(r_2+1) -(d-1)(r_1-r_2) }
{(r_1+1)(r_2+1) - (d-1)(r_1-r_2)  } 
\ \text{ and } \ 
b = \frac{ r_1(r_2+1)  -(d-2)(r_1-r_2) }
{(r_1+1)(r_2+1) - (d-2)(r_1-r_2) } a.
$$
We next prove that given $1 > r_1 > r_2 > \frac{(d-2)r_1}{r_1 + d -1} > 0$, we have 
$1 > a > b \geq a^2 > 0$. First, we prove that $B > A > 0 $:
\begin{align*}
B-A 
& = \frac{(r_1+1)(r_2+1)}{r_1 - r_2}
- \frac{r_1(r_2+1) }{r_1 - r_2} \\
& = \frac{r_2+1}{r_1 - r_2} > 0 \\
\end{align*}
Also,
\begin{align*}
A > 0
& \Leftrightarrow  \frac{r_1(r_2+1)}{r_1 - r_2} > d-1 \\
& \Leftrightarrow 
 r_1(r_2+1)> (d-1)r_1 - (d-1)r_2 \\
& \Leftrightarrow 
(d-1 +r_1)r_2 > (d-2)r_1  \\
& \Leftrightarrow 
r_2 > \frac{(d-2)r_1 }{d-1 + r_1} \\
\end{align*}
Therefore, we have  $B > A > 0 $. Then we have
\begin{align*}
B > A > 0 
& \Rightarrow 1 > \frac{A}{B} >  \frac{A(A+1)}{B(B+1)}  \geq  \frac{A^2}{B^2} > 0\\
& \Rightarrow 1 > a > b \geq a^2 > 0.
\end{align*}

\subsection{Proof of Proposition \ref{pro:strictly_convex}}
\begin{proof}
First, we deal with the case when the coalition weighting function $\mu(\cdot)$ is finite such that $\mu(S) \in \mathbb{R}^+$ for all $S \subseteq [d]$. 
Recall that the objective is defined as following:
\begin{equation}
\label{eqn:weighted_regression_in_proof}
\sum_{S \subseteq [d]}  \mu(S) \left( \f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) \right)^2.
\end{equation}
Obviously, this is a convex function since $\mu(S) > 0$ for all $S \subseteq [d]$. Now we show that it is additionally a strictly convex function:

We first rewrite Eqn.\eqref{eqn:weighted_regression_in_proof} into a matrix form. Let the feature matrix 
$$
\mathbf{X} \in \{ 0,1\}^{2^{d} \times d_\ell}
\text{  indexed with  } \mathbf{X}_{S,T} = \mathbbm{1}[(T \subseteq S) \vee (T = \text{\O})], 
\text{ where } S \subseteq [d]
\text{ and } T \in\mathcal{S}_\ell.
$$
We note that the feature matrix $\mathbf{X}$ is indexed with two sets $S$ and $T$, denoting its rows and columns. Each row of $S$ can also be expressed as $\mathbf{X}_S = \expd(S)$, where $\expd(S) \in \mathbb{R}^{d_\ell}$ with $\expd(S)[T] = \mathbbm{1}[(T \subseteq S) \vee (T = \text{\O})]$.


Then we define the weight matrix:
$$
\sqrt{\mathbf{W}} \in \{ 0,1\}^{2^{d} \times 2^{d}}
\text{ is a diagonal matrix with each entry on the diagonal } \sqrt{\mathbf{W}}_{S,S} = \sqrt{\mu(S)},
$$
where $S \subseteq [d]$.
The function values of $\f(\cdot)$ on each subset can be written into a vector:
$$
\mathbf{Y} \in \mathbb{R}^{2^{d}}
\text{  indexed with }
\mathbf{Y}_S = \f(S)
\text{ where } S \subseteq [d].
$$
With the above definitions, Equation \eqref{eqn:weighted_regression_in_proof} can be viewed as
\begin{equation}
\label{eqn:weighted_regression_matrix_form}
\norm{\sqrt{\mathbf{W} }(\mathbf{Y} -\mathbf{X} \Expl(\f,\ell))}_2^2 = \norm{\mathbf{Y_w}-\mathbf{X_w}\Expl(\f,\ell)}_2^2,
\end{equation}
where $\mathbf{Y_w} = \sqrt{\mathbf{W} }\mathbf{Y}$ and $\mathbf{X_w} = \sqrt{\mathbf{W} }\mathbf{X}$. The Hessian matrix can be expressed as $2\mathbf{X_w}^T \mathbf{X_w}$.

We now prove that the Hessian matrix is positive definite. 
Let $\mathbf{b}$ be any vector in  $\mathbb{R}^{d_\ell}$. 
$$
\mathbf{b}^T \left(2\mathbf{X_w}^T\mathbf{X_w} \right) \mathbf{b}
= 2\norm{\mathbf{X_w} \mathbf{b}}_2^2  
= 2\norm{\sqrt{\mathbf{W}}\mathbf{X} \mathbf{b}}_2^2 
\geq 0.
$$
We get that $\mathbf{b}^T \mathbf{X_w}^T\mathbf{X_w} \mathbf{b} = 0$ if and only if $\norm{\sqrt{\mathbf{W}}\mathbf{X} \mathbf{b}}_2 = 0$. Since $\sqrt{\mathbf{W}}$ is a diagonal matrix with each entry is a positive number, we get
$$
\norm{\sqrt{\mathbf{W}}\mathbf{X} \mathbf{b}}_2 = 0 
\Leftrightarrow
\mathbf{X} \mathbf{b} = \mathbf{0}
\Leftrightarrow
\expd(S) \mathbf{b} = 0, \ \ \forall \ S \subseteq [d].
$$

We prove that this also implies that $\mathbf{b}_L = 0$ for all $L \in \setlessell$ by using induction on the size of $T$.
\begin{enumerate}
    \item If we plug in $S = \text{\O}$, we get $\mathbf{b}_{\text{\O}} = 0$.
    \item Assume $\mathbf{b}_L = 0$ for all $L \subseteq [d]$ with $|L| \leq k$.
    \item For all subsets $L$ with size $k+1 \leq \ell$, we have 
    $$
    \sum_{T \subseteq L} \mathbf{b}_T 
    = \mathbf{b}_L +  \sum_{T \subseteq L, |T| \leq k} \mathbf{b}_T 
    =0.
    $$
    Therefore, we have $\mathbf{b}_L =0$.
\end{enumerate}
We obtain that $\mathbf{b}^T \mathbf{X_w}^T\mathbf{X_w} \mathbf{b} = 0$ if and only if $\mathbf{b} = \mathbf{0}$. Therefore, the Hessian matrix is positive definite and Eqn.\eqref{eqn:weighted_regression_in_proof} is strictly convex.

\end{proof}

\subsection{Proof of Proposition \ref{pro:unique_minimizer}}

\begin{proof}
If the coalition weighting function $\mu$ is finite, Proposition \ref{pro:strictly_convex} has shown that the objective is strictly convex and therefore has a unique minimizer. Now we deal with the case when $\mu(\text{\O})$ and $\mu([d])$ are allowed to be infinite.

We first define a new coalition weighting function $\mu' :2^d \rightarrow \mathbb{R}^{+}$ with 
$$
\mu'(S) =
\begin{cases}
1 & \text{ if } \mu(S) = \infty. \\
\mu(S) & \text{ otherwise.} \\
\end{cases}
$$
We can see that for all $\ex(\f,\ell) \subseteq \mathbb{R}^{d_\ell}$ satisfying  $\f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) =0, \forall S: \mu(S) = \infty, S \subseteq [d]$, the values of objective functions instantiated with $\mu$ and $\mu'$ are the same. That is, 
$$
\sum_{S \subseteq [d]\,:\, \mu(S) < \infty}  \mu(S) \left( \f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) \right)^2
= \sum_{S \subseteq [d]}  \mu'(S) \left( \f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) \right)^2.
$$
Therefore, we can substitute $\mu$ with $\mu'$ and use the fact that  $\sum_{S \subseteq [d]}  \mu'(S) \left( \f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) \right)^2$ is a strictly convex function by Propostion \ref{pro:strictly_convex}.

Then, since there exists at least a solution $\ex(\f,\ell) \subseteq \mathbb{R}^{d_\ell}$ for the set of linear equations $\f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) =0, \forall S: \mu(S) = \infty, S \subseteq [d]$, we have at least one minimizer of Eqn.\eqref{eqn:constrained_weighted_regresion}. Suppose that there exist two minimizers $\ex_1(\f,\ell)$ and $\ex_2(\f,\ell)$. Since $\ex_1(\f,\ell)$ and $\ex_2(\f,\ell)$ both satisfy the set of linear equations $\f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) =0, \forall S: \mu(S) = \infty, S \subseteq [d]$, $(\ex_1(\f,\ell) + \ex_2(\f,\ell)) / 2$ also satisfy it. However, since we have a strictly convex objective,
$$
F(\ex) = \sum_{S \subseteq [d]}  \mu'(S) \left( \f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) \right)^2,
$$
we have $F(\ex_1) + F(\ex_2) > \frac{F((\ex_1+\ex_2)/2)}{2}$, which is a contradiction. Therefore, we have a unique minimizer for Eqn.\eqref{eqn:constrained_weighted_regresion}.

\end{proof}


\subsection{Proof of Proposition \ref{pro:ell_equals_d}}

\begin{proof}
First, by Proposition \ref{pro:unique_minimizer}, Eqn.\eqref{eqn:constrained_weighted_regresion} has a unique minimizer. Next, we prove that $\ex_S(\f,d) = a(\f,S)$ is the only minimzer. Specifically, \citet{grabisch2000equivalent} has shown that $\ex_S(\f,d) = a(\f,S)$ satisfies
$$
\f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) 
= \f(S) - \sum_{T \subseteq S , |T| \leq \ell} a(\f,T) 
= 0 
\text{, for all }
S \subseteq [d].
$$
This implies that Eqn.\eqref{eqn:constrained_weighted_regresion} is zero. However, since Eqn.\eqref{eqn:constrained_weighted_regresion} is always non-negative,
$\ex_S(\f,d) = a(\f,S)$ is the only minimizer.
\end{proof}


\subsection{Proof of Proposition \ref{pro:parital_derivative_general}}
\begin{proof}

The objective can be expressed as a quadratic function of $\Expl_A(\f, \ell)$:
\begin{equation}
\label{eqn:quadratic_objective}
\sum_{S \subseteq [d], \mu(S) < \infty}  \mu(S) \left( \f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) \right)^2 = 
a_A \Expl_A(\f, \ell)^2 + b_A\Expl_A(\f, \ell) + c_A.
\end{equation}

We now solve the coefficients $a_A, b_A, c_A$. First, the leading coefficient is
$$
a_A = \sum_{\substack{S:S \supseteq A, \\ \mu(S) < \infty }} \mu(S).
$$
Secondly, for any subset $B \in \setlessell, B \neq A$,  we note that $\Expl_A(\f_R, \ell)$ and $\Expl_B(\f_R, \ell)$ appear in the same bracket for all subsets $S \supseteq (A \cup B)$ in Eqn.\eqref{eqn:quadratic_objective}. Hence, the coefficient of the first order term is 
\begin{align*}
b_A
& = \left[\sum_{\substack{B:B \in \setlessell, \\ B \neq A}}  \sum_{\substack{S:S \supseteq A \cup B, \\ 
\mu(S) < \infty}} 2\mu(S)\Expl_B(\f, \ell) \right] - 2 \sum_{\substack{S:S \supseteq{A}, \\ \mu(S) < \infty}} \mu(S) \f(S) \\
& =2 \left[\sum_{\substack{B:B \in \setlessell, \\ B \neq A}} \Expl_B(\f, \ell) \sum_{\substack{S:S \supseteq A \cup B, \\ 
\mu(S) < \infty}} \mu(S) \right] - 2 \sum_{\substack{S:S \supseteq{A}, \\ \mu(S) < \infty}} \mu(S) \f(S). \\
\end{align*}

Combining the above, the partial derivative is
\begin{align*}
2a_A \Expl_A(\f, \ell)+ b_A =  
-2 \sum_{ \substack{S: S \supseteq A, \\ \mu(S) < \infty}} \mu(S) \f(S) + 2\sum_{S \in \setlessell} \Expl_S(\f, \ell) \sum_{\substack{L: L \supseteq S \cup T, \\ \mu(L) < \infty}} \mu(L).
\end{align*}

\end{proof}

\subsection{Proof of Proposition \ref{pro:constrained_closed_matrix_form_solution}}

\begin{proof}
We solve the constrained minimization problem via Lagrangian multiplier. Denote the objective $F(\ex) = \sum_{S \subseteq [d], 1 \leq |S| \leq d-1}  \mu(S) \left( \f(S) - \sum_{T \subseteq S , |T| \leq \ell}\Expl_T(\f,\ell) \right)^2$. Then we have the following equalities.
$$
\begin{cases}
\frac{\partial F(\ex)}{\partial \ex_A} 
= \lambda_{[d]} \cdot \frac{\partial }{\partial \ex_A} \left( -\f([d]) + \sum_{T \subseteq [d], |T| \leq \ell} \ex_T(\f,\ell) \right) = \lambda_{[d]}
& \text{ for all } A \in \setlessell \backslash \{\text{\O} \}. \\
\frac{\partial F(\ex)}{\partial \ex_{\text{\O}}} 
= \lambda_{\text{\O}} + \lambda_{[d]} \frac{\partial }{\partial \ex_{\text{\O}}} \left( -\f([d]) + \sum_{T \subseteq [d], |T| \leq \ell} \ex_T(\f,\ell) \right) =
\lambda_{\text{\O}} +\lambda_{[d]} \\
\sum_{T \subseteq [d], |T| \leq \ell} \ex_T = \f([d]) \\
\ex_{\text{\O}}(\f,\ell) = \f(\text{\O}).
\end{cases}
$$
By Proposition \ref{pro:parital_derivative_general}, we have 
\begin{align*}
\frac{\partial F(\ex)}{\partial \ex_A} 
& = -2 \sum_{ \substack{S: S \supseteq A, \\ \mu(S) < \infty}} \mu(S) \f(S) + 2\sum_{S \in \setlessell} \Expl_S(\f, \ell) \sum_{\substack{L: L \supseteq S \cup A, \\ \mu(L) < \infty}} \mu(L) \\
& = -2 \bar{\f}(A) + 2 \sum_{S \in \setlessell} \bar{\mu}(S \cup A)\Expl_S(\f, \ell). \\
\end{align*}
Combining the above two equations, we then have
$$
\begin{cases}
- \frac{1}{2}\lambda_{[d]} + \sum_{S \in \setlessell} \bar{\mu}(S \cup A)\Expl_S(\f, \ell) 
 =  \bar{\f}(A)
& \text{ for all } A \in \setlessell \backslash \{\text{\O} \}. \\
- \frac{1}{2}\lambda_{\text{\O}} - \frac{1}{2}\lambda_{[d]} + \sum_{S \in \setlessell} \bar{\mu}(S)\Expl_S(\f, \ell)
 =  \bar{\f}(\text{\O}) \\
\ex_{\text{\O}}(\f,\ell) = \f(\text{\O}).\\
\sum_{T \subseteq [d], |T| \leq \ell} \ex_T = \f([d]). \\
\end{cases}
$$
Now we write the system of linear equations into the matrix form.
$$
\mathbf{M} \begin{bmatrix}
\lambda_{\text{\O}} \\
\lambda_{[d]} \\
\ex_{\text{\O}}(\f,\ell) \\
\cdots \\
\ex_{S}(\f,\ell) \\
\ex_{T}(\f,\ell) \\
\cdots \\
\end{bmatrix}
= \mathbf{y}.
$$
By Proposition \ref{pro:unique_minimizer}, we know the system of linear equations has a unique solution, we have that the matrix $\mathbf{M}$ is invertible and therefore the solution can be expressed as $\mathbf{M}^{-1}\mathbf{y}$.

\end{proof}



\newpage


\section{Proof of Theorems}
\label{sec:proofs_theorems}
In this section, we provide the proof for Theorem \ref{thm:thmdummysymm} and \ref{thm:faith_shap}.

\subsection{Extra Notations}
\label{sec:extra_notations}

First, we introduce the cumulative weighting function. This function appears naturally in the partial derivatives of  Eqn.\eqref{eqn:weighted_regression} and Eqn.\eqref{eqn:constrained_weighted_regresion} with respect to each variable $\ex_S(\f,\ell)$ (we will show it in the later proof).  

\begin{definition}
\label{def:cumulative_weighting}
The cumulative weighting  function $\bar{\mu}:2^d \rightarrow \mathbb{R}^+$ such that $\bar{\mu}(S) = \sum_{\substack{T:T \supseteq S, \mu(T) < \infty}} \mu(T)$ for all subset $S \subseteq [d]$.
\end{definition}

When the function $\mu(S)$ only depends on the size of the input $|S|$, we simplify the notations by $\mu_{|S|} = \mu(S)$ and  $\bar{\mu}(S)
= \mubar{|S|} 
= \sum_{T \supseteq S, \mu(T) < \infty} \mu_{|T|} = \sum_{i: |S| \leq i \leq d, \mu_i < \infty}{d-|S| \choose i-|S|}\mu_{i}$ for all subsets $S \subseteq [d]$ to simplify the notation. Also, we introduce the notation of $D^{p}_q$ which will be used when solving first-order conditions of weighted regression problems.


\begin{definition}
\label{def:Dpq}
When the weighting function $\mu(\cdot)$ only depends on its input size, we define
$D^{p}_q = \sum_{j=0}^{q}{q \choose j} (-1)^{j}\mubar{p+j}$ for all $p,q \in \{0,1,2,...,d\}$ with $0 \leq p+q \leq d$. 
\end{definition}

In the proof in this section, the binomial coefficient ${ n \choose k}$ has a more general definition: for integers $n$ and $k$,
\begin{equation}
{ n \choose k}
= \begin{cases}
\frac{n!}{k!(n-k)!} & \text{  , if  } \ \ n \geq k \geq 0 \\
0 & \text{ , otherwise. }
\end{cases}
\end{equation}


\subsection{Proof of Theorem \ref{thm:thmdummysymm}}
\label{sec:proof_theorem_dummysymm}

We separate the proof of Theorem \ref{thm:thmdummysymm} into two parts: the sufficient condition and the necessary condition.

\subsubsection{Sufficient Condition}
\label{sec:suf_condition}

\begin{proof}
First of all, we prove the sufficient condition: suppose that the weighting function is in the following form:
\begin{align*}
\mu(S) & \propto \sum_{i=|S|}^{d} {d- |S| \choose i-|S|}(-1)^{i-|S|} g(a,b,i), \  \text{ where }
g(a,b,i) = 
\begin{cases}
1 & \text{ , if } \ i = 0. \\
\prod_{j=0}^{j=i-1} \frac{a(a-b) + j(b-a^2)}{a-b + j(b-a^2)}
& \text{ , if } \   1 \leq i \leq d. \\
\end{cases}
\end{align*} 
for some $a,b \in \R^{+}$ with $a>b$ such that $\mu(S) > 0$ for all $S \subseteq [d]$. Then we prove that the minimizer of Eqn.\eqref{eqn:weighted_regression} given the above weighting function satisfies interaction linearity, symmetry and dummy axioms. 

Since the $\mu(\cdot)$ defined in Eqn.\eqref{eqn:thmdummysymm} only depends on the size of the input set, to simplify the notations, we use $\mu_{|S|} = \mu(S)$ and  $\bar{\mu}(S) = \mubar{|S|} =  \sum_{i=|S|}^{d}{d-|S| \choose i-|S|}\mu_{i}$ to denote the weighting function and the cumulative weighting function (Definition \ref{def:cumulative_weighting}) for all subsets $S \subseteq [d]$. Also, since multiplying a scalar to $\mu$ does not change the minimizer of Eqn.\eqref{eqn:weighted_regression}, without loss of generality, we assume that $\mu(S) = \sum_{i=|S|}^{d} {d- |S| \choose i-|S|}(-1)^{i-|S|} g(a,b,i)$.

Then, we derive some properties of the weighting function $\mu(\cdot)$ the cumulative weighting function $\bar{\mu}(\cdot)$ and the operator $D_{i}^{t}$. We delay the proof of Claim \ref{clm:mubar_mu_relation}-\ref{clm:d_ri_positive} to Section \ref{sec:proofs_claims}.

\begin{claim}
\label{clm:mubar_mu_relation}
For all weighting function $\mu:\{0,1\}^d \rightarrow \mathbb{R}^+$, we have
$$\mu(S) = \sum_{T \supseteq S} (-1)^{|T| - |S|} \bar{\mu}(T) \text{  , for all $S \subseteq [d]$.  } 
$$
\end{claim}


Then the cumulative weighting function $\mubar{t}$ can be computed as following:

\begin{claim}
\label{clm:mubar_closeform}
When $\mu(S) = \sum_{i=|S|}^{d} {d- |S| \choose i-|S|}(-1)^{i-|S|} g(a,b,i)$, the cumulative weighting function is 
$$
\mubar{t} = 
\begin{cases}
\prod_{j=0}^{t-1} \frac{a(a-b) + j(b-a^2)}{a -b + j(b-a^2)} & \text{ , if } 1 \leq t \leq d. \\
1 & \text{ , if } t=0.\\
\end{cases}
$$
\end{claim}

Also, the following claim states that the operator $D^t_i$ is positive for all $t,i \in \{0,1,2,...,d\}$ with $0 \leq t+i \leq d$. 
\begin{claim}
\label{clm:d_ri_positive}
When $\mu(\cdot)$ is finite and permutation-invariant, we have $D^{p}_q > 0$ for all $p,q \in \{0,1,2,...,d\}$ with $0 \leq p+q \leq d$. 
\end{claim}

By Proposition \ref{pro:linearity}, the Faith-Interaction index satisfies interaction linearity axiom. 
In addition, by Proposition \ref{pro:symmetry},  since the weighting $\mu(S)$ only depends on $|S|$, the Faith-Interaction index also satisfies the interaction symmetry axiom. Consequently, we only need to prove that the Faith-Interaction index satisfies the interaction dummy axiom.

Next, we introduce the basis function.
\begin{definition}
\label{def:basis_function}
For any subset $R \subseteq [d]$ with $|R| = r$, the basis function with respect to $R$ is defined below:
$$
\f_R(S) = \begin{cases}
1, & \text{if  } \ S \supseteq R. \\
0, & \text{otherwise.}
\end{cases}
$$
\end{definition}

This is known as \textit{unanimity game} in game theory community. We note that only elements inside $R$ actually contribute to the function value. That is, elements belong to $[d] \backslash R$ are dummy elements. Formally, we have $\f(S \cup i) = \f(S)$ for any $i \in [d] \backslash R$ and $S \subseteq [d]\backslash \{i\}$.

An important property of the basis functions is that any function $\f:\{0,1\}^d \rightarrow \mathbb{R}$ can be expressed as a linear combination of the $2^d$ basis functions. 
Then by the interaction linearity axiom, the minimizer of Eqn.\eqref{eqn:weighted_regression} with respect to $\f(\cdot)$ can be represented as the same linear combination of minimizer of these basis functions. 
In the following lemma, we show that if the minimizers of Eqn.\eqref{eqn:weighted_regression} with respect to these $2^d$ basis functions satisfy the interaction dummy axiom, then all functions satisfy dummy axiom. Therefore, it is sufficient to prove that these minimizers satisfy the interaction dummy axiom for these $2^d$ basis functions.
\begin{lemma}
\label{lm:f_decomposable}
Let $\ex(\f,\ell)$ be a Faith-Interaction indice with respect to a proper weighting function $\mu:2^d \mapsto \mathbb{R}^+ \cup \{\infty \}$.
If $\ex_S(\f_R,\ell) = 0$ for all $\ell \in [d]$ and for all $S \in \setlessell, R \subseteq [d]$ with $S \cap ([d] \backslash R) \neq \text{\O}$, then the Faith-Interaction indices with respect to the weighting function $\mu(\cdot)$ satisfy interaction dummy axiom. 
\end{lemma}
\begin{proof}
By Lemma 3 in \citet{shapley1953value}, any function $\f:\{0,1\}^d \rightarrow \mathbb{R}$ can be expressed as a linear combination of these $2^d$ basis functions, such that
$$
\f = \sum_{R \subseteq [d]} c_R \f_R 
\ \  \text{  with  }  \ \ 
c_R = \sum_{T \subseteq R} (-1)^{|R| - |T|} \f(T).
$$
$c_R$ here is the Möbius coefficient.
By Proposition \ref{pro:linearity}, the Faith-Interaction indice $\ex$ satisfies the interaction linearity axiom, which implies that $\Expl(\f,\ell)$ can be expressed as the following form:
$$
\Expl(\f,\ell) = \sum_{R \subseteq [d]} c_R \Expl(\f_R,\ell).
$$
Suppose that we have some dummy feature $i \in [d]$ such that $\f(T \cup i) = \f(T)$ for any $ T \subseteq [d] \backslash \{ i\}$, then for any $R \supseteq \{ i\}$, we have 
$$
c_R 
= \sum_{T \subseteq R} (-1)^{|R| - |T|} \f(T)
= \sum_{T \subseteq R \backslash \{ i\}} (-1)^{|R| - |T|} ( \f(T) - \f(T \cup i)) = 0.
$$
Therefore, the function $\f$ is the linear combinations of $\f_R(\cdot)$ for some $R$ not containing $i$. However, for these subsets, by the definition of the basis function, we have $\f_R(S) = \f_R(S \cup i)$ for any $S \subseteq [d] \backslash \{i\}$. Since we have $\ex_S(\f_R, \ell) = 0$ for all $S \in \setlessell$ with $S \cap ([d] \backslash R) \neq \text{\O}$, we get $\ex_T(\f_R, \ell) = 0$ for any $T$ containing the dummy feature $i$.
Consequently, we have 
$$
\Expl_T(\f,\ell) = \sum_{R \subseteq [d]} c_R \Expl_T(\f_R,\ell) = \sum_{R \subseteq [d]\backslash \{i\}} c_R \Expl_T(\f_R,\ell) = 0.
$$
We note that the above proof holds for any $\ell \in [d]$. Therefore, the Faith-Interaction indices with respect to $\mu(\cdot)$ satisfy interaction dummy axiom.
\end{proof}

Now we come back to the proof of Theorem \ref{thm:thmdummysymm}. By Lemma \ref{lm:f_decomposable}, we only need to prove that for any $R \subseteq [d]$, the minimizer of Eqn.\eqref{eqn:weighted_regression} with respect to the basis function $\f_R$, $\ex(\f_R,\ell)$, satisfies $\ex_S(\f_R,\ell) = 0$ if $S$ containing any dummy element in $[d] \backslash R$. 

The objective function of the weighted least square problem with respect to the basis function $\f_R$ can be written as follows:

\begin{align}
\label{eqn:weighted_ls}
F_R(\ex) & = \sum_{S \subseteq [d]} \mu_{|S|} \left[\sum_{T \subseteq S, |T| \leq \ell} \Expl_T(\f_R, \ell) - \f_R(S) \right]^2
\\
\label{eqn:weighted_ls_2}
& = \sum_{S \supseteq R, S \subseteq [d]} \mu_{|S|} \left[ \sum_{T \subseteq S, |T| \leq \ell} \Expl_T(\f_R, \ell) - 1 \right]^2 + \sum_{S \not\supseteq R, S \subseteq [d]} \mu_{|S|} \left[ \sum_{T \subseteq S, |T| \leq \ell} \Expl_T(\f_R, \ell)  \right]^2.
\end{align}
Note that the weighting function $\mu$ is defined in Eqn.\eqref{eqn:thmdummysymm}. Let $r = |R|$ denote the size of the set $R$. Now, we separate the problem into three cases: (1) $d \geq \ell \geq  r \geq 0$. (2) $d \geq \ell + r $ and $r > \ell$. (3) $\ell + r > d \geq r > \ell \geq 1$.


\paragraph{(1)  $d \geq \ell \geq  r \geq 0$:} 

\begin{lemma}
If $\f_R$ is a basis function with $|R| = r \leq \ell$, the unique minimizer of Eqn.\eqref{eqn:weighted_ls} is
\begin{equation}
\Expl_T(\f_R, \ell)
= \begin{cases}
1 & \text{, if } \ \ T = R. \\
0 & \text{, otherwise.}
\end{cases}
\end{equation}
\end{lemma}

\begin{proof}
By Proposition \ref{pro:unique_minimizer}, Eqn.\eqref{eqn:weighted_ls} has a unique minimizer. 
If we plug in the above definition of  $\Expl_T(\f_R, \ell)$ to Eqn.\eqref{eqn:weighted_ls_2}, we get that 
$$
\sum_{T \subseteq S, |T| \leq \ell} \Expl_T(\f_R, \ell) - \f_R(S) = 0 
\ \ \text{ for all } \ \
S \subseteq [d].
$$
This implies that $F_R(\ex) = 0$. Since the objective is always non-negative, this is the unique minimizer of Eqn.\eqref{eqn:weighted_ls}.
\end{proof}

\paragraph{(2) $d \geq \ell + r$ and $r > \ell$:} 
Next, we solve Eqn.\eqref{eqn:weighted_ls_2} by using partial derivatives. By Proposition \ref{pro:parital_derivative_general}, for all $A \in \setlessell$, we have 
\begin{align}
\frac{\partial \ F(\ex)}{\partial \Expl_A}
& = -2 \sum_{ \substack{S: S \supseteq A, \\ \mu(S) < \infty}} \mu(S) \f_R(S) + 2\sum_{S \in \setlessell} \Expl_S(\f, \ell) \sum_{\substack{L: L \supseteq S \cup A, \\ \mu(L) < \infty}} \mu(L)
\nonumber \\
& = -2\mubar{|A \cup R|} + 2\sum_{S \in \setlessell} \mubar{|S \cup A|} \Expl_S(\f_R, \ell).
\label{eqn:partial_derivative}
\end{align}

Now we utilize the symmetric structure in the basis function $\f_R(\cdot)$ and weighting function $\mu(\cdot)$.
In the basis functions, there are only two kinds of input elements, which are elements in $R$ and not in $R$. Therefore, for $i^{th}$ order interactions terms $\Expl_{T}(\f_R,\ell)$ where $|T| = i$, there are at most $i+1$ distinct values. Each value corresponds to the set with $j$ elements in $R$ for $j=0,1,...i$. That is, by the interaction symmetry axiom, there are only $i+1$ different importance value for $i^{th}$ order interactions terms (since if $|T_1| = |T_2|$ and $|T_1 \cap R| = |T_2 \cap R|$ then $T_1$ and $T_2$ are symmetric and $\Expl_{T_1}(\f_R,\ell) = \Expl_{T_2}(\f_R,\ell)$), so there are $ 1 + 2 +... + (\ell + 1)= \frac{(\ell + 2)(\ell + 1)}{2}$ kinds of values in the minimizer $\Expl(\f_R,\ell)$. We then introduce a new notation system that utilizes the symmetric structure. First, we use a vector $\bfb$
to represent these $\frac{(\ell + 2)(\ell + 1)}{2}$ values.

\begin{definition}
\label{def:bij}
The vector
$ \bfb \in \mathbb{R}^{\frac{(\ell +1)(\ell + 2)}{2}} \text{ is indexed with  }
\bfb_{i,j} = \Expl_S(\f_R,\ell) \text{  with  } |S| = i \text{ and } |S \backslash R| = j,$
where $i, j$ are integers with $ 0 \leq i \leq \ell$ and $0 \leq j \leq i$.
\end{definition}

The term $\bfb_{i,j}$ means the importance score of an $i^{th}$ order interaction (of size $i$) term with $i-j$ elements lying in $R$ and $j$ element lying in $[d] \backslash R$. Note that in this definition, $\bfb_{0,0} = \ex_{\text{\O}(\f_R,\ell)}$ means the bias term in the weighted linear regression. Now we can apply this new notation to rewrite Eqn. \eqref{eqn:partial_derivative}.


\begin{lemma}
\label{lm:bij_parital_derivative}
The partial derivative of $F_R(\ex)$ with respect to $\bfb_{i,j} $ is 
$$
\frac{\partial F_R(\ex)}{\partial \bfb_{i,j}} 
= -2\mubar{r+j}  
+ 2 \sum_{p=0}^{\ell} \sum_{q=0}^{p} \left( \sum_{\rho=0}^{i-j} \sum_{\sigma=0}^{j} { i-j \choose \rho} { r-(i-j) \choose p-q-\rho} { j \choose \sigma}{ d-r-j \choose q-\sigma} \mubar{i+p-\rho-\sigma} \bfb_{p,q} \right), 
$$
where $r = |R|$.
%where $\mubar{k} = \sum_{i=k}^{d} { d - k \choose i -k} \mu_i$.
\end{lemma}

\begin{proof}
Let $\Expl_A(\f_R, \ell) = \bfb_{i,j} $, where $i = |A|$ and $ j = |A \backslash R| $. Then the first term in Eqn. \eqref{eqn:partial_derivative} is $-2\mubar{|A \cup R|} = -2\mubar{r+j}.$ We know that for any 

\begin{equation}
\label{eqn:mapping_S_to_b}
\mubar{|S \cup A|}\Expl_S(\f_R, \ell)
= \mubar{ \{ |S| + |A| - |S \cap  A| \}} \bfb_{ \{|S|,|S \backslash R| \}} =  \mubar{ \{ |S| + |A| - |S \cap R \cap A | - |(S \cap A \backslash R  | \} } \bfb_{ \{|S|,|S \backslash R| \}}
\end{equation}

for all $S \in \setlessell$. The equation depends on the four sets, which are $A \cap R, A \backslash R, S \cap R$ and $S \backslash R$. 
Therefore, in the following proof of this lemma, we split set $S$ to $S \cap R$ and $S \backslash R$ and consider them in different cases.

We now let $\Expl_S(\f_R, \ell) = \bfb_{p,q}$, so that $p(S) = |S|$ and $q(S) = |S \backslash R|$. Assume $\rho(S) = |S \cap R \cap A |$ and $\sigma(S) = |S  \cap A \backslash R |$. 
Eqn. \eqref{eqn:mapping_S_to_b} can be written as
$$
\mubar{|S \cup A|}\Expl_S(\f_R, \ell) = \mubar{p(S) + i - \rho(S) - \sigma(S)} \bfb_{p,q}.
$$

%Each of $p, q, \rho, \sigma$ are constraints on the relation of sets $S$, $A$ and $R$, since $R$ and $A$ are known, 
We can calculate the number of sets $S$ that satisfies the constraints $p(S) = p_0, q(S) = q_0, \rho(S) = \rho_0, \sigma(S) = \sigma_0$.
%Since $S = (S \cap R) + (S \backslash R)$, we must select $p-q$ elements from $R$ and  $q$ elements from $[d] \backslash R$. Therefore, t
Since $S = (S \cap R) + (S \backslash R)$, the number of $S$ (satisfies the constraints) equals to the number set $ (S \cap R)$ (satisfies the constraints) times the number of set $ (S \backslash R)$ (satisfies the constraints), since $S$ is determined given $S\cap R$ and $ (S \backslash R)$. We calculate the number of set $(S \cap R)$ and set $ (S \backslash R)$ (that satisfies the constraints) respectively.

\begin{enumerate}
    \item First, we observe that the number of $S \cap R$ (that satisfies the constraints) is equal to the number of ways to choose $|S \cap R|$ elements from $R$ (that satisfies the constraints), and $|S \cap R| = p(S) - q(S) = p_0 - q_0.$ Choosing $p_0 - q_0$ elements from $R$ can be further viewed as choosing $|(S \cap R) \cap A|$ elements from $R\cap A$ and $|(S \cap R) \backslash A|$ elements from $R\backslash A$. We note that $|(S \cap R) \cap A| = \rho_0$ and $|(S \cap R) \backslash A| = |(S \cap R)| - |(S \cap R) \cap A| = p_0 - q_0 - \rho_0$.
    %we want to select $p-q$ elements from $R$. There should be $\rho = |(S \cap R) \cap (A \cap R)|$ elements from $R \cap A$ and $|S \cap R| - \rho = p-q-\rho$ elements from $R \backslash A$. Therefore,  
    Therefore, there are ${|R \cap A| \choose \rho_0 }{ |R  \backslash A | \choose p_0-q_0-\rho_0} = {i-j \choose \rho}{r -(i-j) \choose (p-q)-\rho}$ ways to select $|S \cap R|$ elements from $R$.
    
    \item  Secondly, we observe that the number of $S \backslash R$ (that satisfies the constraints) is equal to the number of ways to choose $|S \backslash R|$ elements from $[d] \backslash R$ (that satisfies the constraints), and $|S \backslash R| = q(S) =  q_0.$ Choosing $q_0$ elements from $[d] \backslash R$ can be further viewed as choosing $|S  \cap A \backslash R|$ elements from $A \backslash R$ and $|S \backslash R \backslash A|$ elements from $[d] \backslash R \backslash A$.
    We note that $|S  \cap A \backslash R| = \sigma_0 $ and $|S \backslash R \backslash A| = q_0- \sigma_0$.
    Therefore, there are ${| A \backslash R| \choose  p_0-q_0 -\sigma_0 }{ |[d]\backslash R \backslash A| \choose q_0 -\sigma_0} = {j \choose \sigma}{d-r-j \choose q -\sigma}$ ways to select $|S \cap R|$ elements from $R$.
    
    For elements in $S \backslash R$, there should be $\sigma =  |(S \backslash R) \cap ( A \backslash R )|$ elements 
    from $ A \backslash R = ([d]\backslash R) \cap A$ and $q - \sigma$ elements  from $ ([d]\backslash R) \backslash A$ to satisfy the constraint $\sigma$. Therefore,  
    there are ${ |([d]\backslash R) \cap A| \choose \sigma }{| ([d]\backslash R) \backslash A| \choose q- \sigma}  = {j \choose \sigma}{d-r-j \choose q-\sigma}$  ways to select 
    elements of $S \backslash R$ from $[d]\backslash R$.
    
\end{enumerate}

Note that we have $\rho \leq |A \cap R| = i-j$ and $\sigma \leq |A \backslash R| = j $. Since every $S$ can map to some constraints $p,q,\rho, \sigma$, by summation over all possible $p,q, \rho, \sigma$, we can get the partial derivative of the objective with respect to $\bfb_{i,j}$.

Also, if there are not enough elements to be selected, i.e. $|R \backslash A| < p_0-q_0-\rho_0$, ${|R \backslash A| \choose p_0-q_0-\rho_0} = 0$, so the number of ways for selection is zero. 


\end{proof}

Now, since the minimizer of Eqn.\eqref{eqn:weighted_regression} must satisfy $\frac{\partial F_R(\ex)}{\partial \bfb_{i,j}} $ for all $0 \leq i \leq \ell$ and $0 \leq j \leq i$ , we can write the system of $\frac{(\ell+2)(\ell+1)}{2}$ equations into a matrix form, $\mathbf{M}\bfb= \mathbf{Y}$, with definitions below.


\begin{definition}
The coefficient matrix $\mathbf{M} \in \mathbb{R}^{\frac{(\ell +1)(\ell + 2)}{2} \times \frac{(\ell +1 ) (\ell + 2)}{2}}$, whose rows and columns are indexed with 2 iterators respectively. The value of each entry is 
$$
\mathbf{M}_{\{i,j\}, \{p,q\}} = \sum_{\rho=0}^{i-j} \sum_{\sigma=0}^{j} { i-j \choose \rho } { r-(i-j) \choose p-q-\rho} { j \choose \sigma}{ d-r-j \choose q-\sigma} \mubar{i+p-\rho-\sigma}, $$
where $ 0 \leq i \leq \ell$, $0 \leq j \leq i$,  $ 0 \leq p \leq \ell$ and $0 \leq q \leq p$.
\end{definition}

\begin{definition}
 $\mathbf{Y} \in \mathbb{R}^{\frac{(\ell + 1) (\ell+2)}{2}}$ is a column vector with each entry $\mathbf{Y}_{j} = \mubar{r+j}$.
\end{definition}

Now we prove the interaction dummy axiom holds for the basis function $\f_R$. That is,
$\bfb_{i,j} = 0$ if $j > 0$ for all $i^{th}$ order interaction, $0 \leq i \leq \ell$ since $j > 0$ means there are some elements lying in $[d] \backslash R$.

\begin{lemma}
\label{lm:simplified_matrix}
Assume we have a system of $\upsilon$ linear equations with $\upsilon$ unknowns, $\mathbb{A} \mathbf{v} = \mathbb{C}$, where $\mathbb{A} \in \mathbb{R}^{\upsilon \times \upsilon}$ is the coefficient matrix, $\mathbf{v} \in \mathbb{R}^{\upsilon}$ is a vector of unknowns, and $\mathbb{C} \in \mathbb{R}^{\upsilon}$ is a vector of real numbers. Define $P \subseteq{\{1,2,...,\upsilon \}}$ as a set of indexes, and denote $\mathbb{A}_{P} \in \mathbb{R}^{\upsilon \times |P|}$ as a submatrix of $\mathbb{A}$ by only taking columns in $\mathbb{A}$ whose indexes are in $P$.
%$x_{P} \in \mathbb{R}^{|P|}$ by taking values in $x$  whose indexes is in $P$.  
If $\mathbb{A}\mathbf{v}  = \mathbb{C}$ has a unique solution $\mathbf{v} $ and $rank([\mathbb{A}_P, \mathbb{C}]) = |P|$, then the solution $\mathbf{v}_i = 0$ if $i \notin P$. 
\end{lemma}

\begin{proof}
Since $\mathbb{A}\mathbf{v} = \mathbb{C}$ has a unique solution, by Rouché–Capelli theorem, we have $rank(\mathbb{A}) = rank([\mathbb{A},\mathbb{C}]) = \upsilon$, which equals to the number of columns in $\mathbb{A}$. Hence, the columns of $\mathbb{A}$ are linear independent. The column spaces of $\mathbb{A}_P$ consists of $|P|$ columns from $\mathbb{A}$, so we have $rank(\mathbb{A}_P) = |P|$.

Let $\mathbf{v} _P \in \mathbb{R}^{|P|}$ consist of values in $x$ whose indexes are in $P$.
By Rouché–Capelli theorem, $rank(\mathbb{A}_P)= rank([\mathbb{A}_P,\mathbb{C}]) = |P|$ implies the system of linear equations, $\mathbb{A}_P\mathbf{v}_P=\mathbb{C}$, has a unique solution $\mathbf{v}_P$. 
Now we construct the solution of $\mathbb{A}\mathbf{v}  = \mathbb{C}$ by $\mathbf{v}_P$: let
$$
\mathbf{v} _i = \begin{cases}
\mathbf{v} _{Pj} \text{ if } i \in P, \text{ where $i$ the $j^{th}$ element of $P$} \\
0 \text{ , otherwise, } \\
\end{cases}
$$
where $\mathbf{v}_{Pj}$ denote the $j^{th}$ element of $\mathbf{v}_P$. We can easily verify that $\mathbf{v}$ is the unique solution of $\mathbb{A}\mathbf{v} = \mathbb{C}$. 

\end{proof}

Lemma \ref{lm:simplified_matrix} tells us that if we aim to prove that some unknown variables are zero in a system of linear equations, we can alternatively prove that the rank of a simplified augmented matrix $[\mathbb{A}_P,\mathbb{C}]$ equals $|P|$. 

Then, if the interaction dummy axiom holds, the terms $\bfb_{i,j}$ with $i \geq j > 0$ should be zero since these interaction terms contain at least one dummy element ( that is outside $R$). Therefore, by Lemma \ref{lm:simplified_matrix},
we now consider columns corresponding to $\bfb_{0,0}, \bfb_{1,0},..., \bfb_{\ell,0}$. These columns correspond to interaction terms that only contain elements in $R$. 
We simplify the matrix $\mathbf{M}$ in the following way:

Put
$$
\mathbf{M'} \in \mathbb{R}^{\frac{(\ell+1)(\ell+2)}{2} \times (\ell+1)} \text{, whose columns correspond to } \bfb_{i,0} \text{ of } \mathbf{M} \text{ for } 0 \leq i \leq \ell
$$
\begin{equation}
\label{eqn:m_definition}
\small
\text{ with each entry } \mathbf{M'}_{\{i,j\},\{p, 0\} } = \sum_{\rho=0}^{i-j} { i-j \choose \rho} { r-(i-j) \choose p- \rho} \mubar{i+p-\rho}  \text{ for } 0 \leq i \leq \ell,  0 \leq p \leq \ell  \text{ and }  0 \leq j \leq i.
\end{equation}


The entry $\mathbf{M'}_{\{i,j\},\{p, 0\}}$ can be interpreted as the coefficient of $\bfb_{p,0}$ in the equation $\frac{\partial F_R(\ex)}{ \partial \bfb_{i,j}} = 0$.
Since we have already known that the system of linear equations, $\mathbf{M}b=\mathbf{Y}$, has a unique solution by Proposition \ref{pro:unique_minimizer}, if we can prove that the rank of the matrix $\mathbf{Q} = [\mathbf{M'}, \mathbf{Y}]$ equals to $\ell + 1$, we can conclude that $\bfb_{i,j} = 0 $ for all $i \geq j > 0$ by Lemma \ref{lm:simplified_matrix}. It implies the interaction dummy axiom holds for the basis function $\f_R$. To calculate the rank of matrix $\mathbf{Q}$, we first define some notations.

\begin{definition}
\label{def:row_combination}
We define a function  $\Re_{i,j}^k(\cdot): \mathbb{R}^{\frac{(\ell+1)(\ell+2)}{2}  \times (\ell+1) } \rightarrow  \mathbb{R}^{ \ell+1} $, which takes a matrix as input and outputs a weighted summation of rows. Formally, for any matrix $\mathbf{B} \in \mathbb{R}^{\frac{(\ell+1)(\ell+2)}{2}  \times (\ell+1)}$, let
$$
\Re_{i,j}^k(\mathbf{B}) = \sum_{\sigma=0}^{\sigma=k} {k \choose \sigma} (-1)^{\sigma} \mathbf{B}_{\{i,j+\sigma \}}
$$
be a combination of rows of $\mathbf{B}$
for any $0 \leq i \leq \ell $, $0 \leq j \leq i$ and $0 \leq k \leq i-j$, where $\mathbf{B}_{\{i,j+\rho\}}$ is denoted as the $\{i, j+\rho\}$th row of the matrix $\mathbf{B}$.
\end{definition}
$\Re_{i,j}^k (\mathbf{Q})$ can be interpreted as some row operations during the Gaussian elimination process along the rows corresponding to the interaction terms of size $i$, $\bfb_{i,\rho}$ for some $0 \leq \rho \leq i$, in the matrix $\mathbf{Q}$.
We note that $\Re_{i,j}^0(\mathbf{B}) = \mathbf{B}_{\{i,j\}}$ if $k = 0$.
Then we prove the following lemma. 

\begin{definition}
\label{def:Pst}
Define
$$
\mathbf{P}_{s,t} = 
\begin{bmatrix}
\Re_{s,s}^{0}(\mathbf{Q}) \\
\Re_{s+1,s}^{1}(\mathbf{Q}) \\
...\\
\Re_{s+t, s }^{t}(\mathbf{Q}) \\
\end{bmatrix}, 
\text{ and } 
\mathbf{P'}_{s,t} = 
\begin{bmatrix}
\mathbf{P}_{s,t} \\
\Re_{s+t-1, s }^{t-1}(\mathbf{Q}) - \Re_{s+t, s}^{t-1}(\mathbf{Q}) \\
\end{bmatrix}, 
$$
where $\mathbf{P}_{s,t} \in \mathbb{R}^{(t+1) \times (\ell + 2)}$ and $\mathbf{P'}_{s,t} \in \mathbb{R}^{(t+2) \times (\ell + 2)}$ for 
$0 \leq s \leq \ell-1 $ and $1 \leq t \leq \ell - s$.

\end{definition}

\begin{lemma}
\label{lm:Pst_value}
Following Definition \ref{def:Dpq} and \ref{def:Pst} ,  
\begin{equation}
\small
\mathbf{P'}_{s,t} =
\begin{bmatrix}
D_{0}^{s}, & {r \choose 1 }D_{0}^{s+1}, & ...&
{r \choose t-1 }D_{0}^{s+t-1}, & {r \choose t }D_{0}^{s+t}, &...  & { r \choose \ell  }D_{0}^{s+\ell},  & D_{0}^{r+s} \\
0, & {r-1 \choose 0 }D_{1}^{s+1}, & ...& 
{r-1 \choose t-2 }D_{1}^{s+t-1}, & 
{r-1 \choose t-1 }D_{1}^{s+t}, & ... & { r-1 \choose \ell -1 } D_{1}^{s+\ell}, & D_{1}^{r+s} \\
0, & 0, & ...&  
{r-2 \choose t-3 }D_{2}^{s+t-1}, & 
{r-2 \choose t-2 }D_{2}^{s+t}, & ... & { r-2 \choose \ell-2 } D_{2}^{s+\ell}, & D_{2}^{r+s} \\
., & ., & ... &., &., & ... & .,& . \\
0, & 0,& ...& 0 , & 
{r-t \choose 0 }  D_{t}^{s+t}, & ... 
 & { r-t \choose \ell-t } D_{t}^{s+\ell}, & D_{t}^{r+s}  \\
0,& 0,& ...& {r-t+1 \choose 0} D_{t}^{s+t-1}, & 
[{r-t+1 \choose 1}- {r-t \choose 0 } ] D_{t}^{s+t}, &... & [{r-t+1 \choose \ell-t+1}- {r-t \choose \ell-t } ] D_{t}^{s+\ell}, & 0  \\
\end{bmatrix}.
\end{equation}
Formally, for all $0 \leq t' \leq t+1$ and $0 \leq p \leq \ell+1$, the $(p+1)^{th}$ element of  $(t'+1)^{\ th}$ row of $\mathbf{P'}_{s,t}$ is 
\begin{equation}
\begin{cases}
0 & \text{ if } 0 \leq t' \leq t \text{ and } p < t' \\
{r-t' \choose p-t'} D_{t'}^{s+p} 
& \text{ if } 0 \leq t' \leq t  \text{ and }  t' \leq p \leq \ell\\
D_{t'}^{r+s} & \text{ if } 0 \leq t' \leq t \text{ and } p = \ell+1 \\
0 & \text{ if }    t'=t+1 \text{ and } p < t-1  \\
{r-t+1 \choose 0} D_{t}^{s+t-1}  & \text{ if } t'=t+1 \text{ and } p = t-1\\
[{r-t+1 \choose p-t+1}- {r-t \choose p-t } ] D_{t}^{s+p} & \text{ if }    t'=t+1 \text{ and } t \leq  p \leq \ell  \\
0 & \text{ if }    t'=t+1 \text{ and } p =\ell + 1 \\
\end{cases}.
\end{equation}
\end{lemma}

\begin{proof}
We first introduce two claims.
\begin{claim}
\label{clm:row_operation}
For $0 \leq s' \leq \ell -1$, $0 \leq t' \leq \ell-s'$ and $0 \leq p'\leq \ell$, 
\begin{equation}
\sum_{\sigma=0}^{\sigma=t'} {t' \choose \sigma} (-1)^{\sigma} \mathbf{M'}_{\{s'+t', s'+\sigma \},\{p',0\}} 
= \begin{cases}
0 & \text{ if } p' < t' \\
{r-t' \choose p-t'} D_{t'}^{s'+p'}
  & \text{ if }  t' \leq p' \leq \ell
\end{cases}
\end{equation}

\end{claim}

\begin{claim}
\label{clm:row_decomp}
For any matrix $\mathbf{B} \in \mathbb{R}^{\frac{(\ell+1)(\ell+2)}{2}  \times (\ell+1)}$, $\Re_{s+t,s}^{t-1}(\mathbf{B}) = \Re_{s+t,s}^{t}(\mathbf{B}) + \Re_{s+t,s+1}^{t-1}(\mathbf{B})$.
\end{claim}
We leave the proof of Claim \ref{clm:row_operation} and \ref{clm:row_decomp} to Section \ref{sec:proofs_claims}.
We now compute value of each entry of $\mathbf{P'}_{s,t}$ by cases.
\begin{enumerate}
    \item If $0 \leq t' \leq t$ and $p < t'$, by plugging in $s'=s$, $t'=t'$ and $p'=p$ to Claim \ref{clm:row_operation}, the value of $(p+1)^{th}$ element of $(t'+1)^{th}$ row of $\mathbf{P'}_{s,t}$ is
    $$
    \sum_{\sigma=0}^{\sigma=t'} {t' \choose \sigma} (-1)^{\sigma} \mathbf{M'}_{\{s+t', s+\sigma \},\{p,0\}} 
    = 0 
    $$
    
    \item If $0 \leq t' \leq t$ and $t' \leq p \leq \ell$, by plugging in $s'=s$, $t'=t'$ and $p'=p$ to Claim \ref{clm:row_operation}, the value of $(p+1)^{th}$ element of $(t'+1)^{th}$ row of $\mathbf{P'}_{s,t}$ is
    $$
    \sum_{\sigma=0}^{\sigma=t'} {t' \choose \sigma} (-1)^{\sigma} \mathbf{M'}_{\{s+t', s+\sigma \},\{p,0\}} 
    = {r-t' \choose p-t'} D_{t'}^{s+p}
    $$
    \item If $0 \leq t' \leq t$ and $p=\ell + 1$, the value of $(\ell+2)^{th}$ element of $(t'+1)^{th}$ row of $\mathbf{P'}_{s,t}$ is 
    $$
    \sum_{\sigma=0}^{\sigma=t'} {t' \choose \sigma} (-1)^{\sigma} \mathbf{Y}_{s+t', s+\sigma } 
    = \sum_{\sigma=0}^{\sigma=t'} {t' \choose \sigma} (-1)^{\sigma} \mubar{r+s+\sigma } 
    = D_{t'}^{r+s}
    $$
    
    \item If $t'=t+1$ and $p < \ell+1$, by Claim \ref{clm:row_decomp}, the  $(t+2)^{th}$ row of $\mathbf{P'}_{s,t}$ becomes $ \Re_{s+t-1,s}^{t-1} - \Re_{s+t,s+1}^{t-1} - \Re_{s+t,s}^{t} $.
    The value of $p^{th}$ element this row is
    \begin{align*}
    & \sum_{\sigma=0}^{t-1} {t-1 \choose \sigma} (-1)^{\sigma} ( \mathbf{M'}_{\{s+t-1, s+\sigma \},\{p,0\}} -   \mathbf{M'}_{\{s+t, s+\sigma+1 \},\{p,0\}} ) 
    - \sum_{\sigma=0}^{t} {t \choose \sigma} (-1)^{\sigma} \mathbf{M'}_{\{s+t, s+\sigma \},\{p,0\}} \\
    & =  
    \begin{cases}
    0 & \text{ if } p < t-1 \\
    {r-t+1 \choose p-t+1} D_{t-1}^{s+p} 
    - {r-t+1 \choose p-t+1} D_{t-1}^{s+p+1}
    & \text{ if }  p = t-1  \\
    {r-t+1 \choose p-t+1} D_{t-1}^{s+p} 
    - {r-t+1 \choose p-t+1} D_{t-1}^{s+p+1}
    - {r-t \choose p-t } D_{t}^{s+p}
    & \text{ if }  t \leq p \leq \ell   \\
    \end{cases}
    \ \ \ (\text{Claim \ref{clm:row_operation}}) \\
    & =  
    \begin{cases}
    0 & \text{ if } p < t-1 \\
    {r-t+1 \choose p-t+1} D_{t}^{s+p} 
    & \text{ if }  p = t-1  \\
    [{r-t+1 \choose p-t+1}- {r-t \choose p-t } ] D_{t}^{s+p} & \text{ if }  t \leq p \leq \ell   \\
    \end{cases}
    \end{align*}
    
    \item If $t'=t+1$ and $p=\ell + 1$, the value of $(\ell+2)^{th}$ element of $(t+2)^{th}$ row of $\mathbf{P'}_{s,t}$ is 
    \begin{align*}
    & \sum_{\sigma=0}^{t-1} {t-1 \choose \sigma} (-1)^{\sigma} \mathbf{Y}_{s+t-1, s+\sigma } 
    - \sum_{\sigma=0}^{t-1} {t-1 \choose \sigma} (-1)^{\sigma} \mathbf{Y}_{s+t, s+\sigma }  \\
    & = \sum_{\sigma=0}^{t-1} {t-1 \choose \sigma} (-1)^{\sigma} \mubar{r+s+\sigma } 
    - \sum_{\sigma=0}^{t-1} {t-1 \choose \sigma} (-1)^{\sigma} \mubar{r+s+\sigma }  \\
    & = 0 \\
    \end{align*}

\end{enumerate}



\end{proof}

\begin{lemma}
\label{lm:submatrix_rank}
The rank of matrices $\mathbf{P}_{s,t}$ and $\mathbf{P'}_{s,t}$ are $t+1$ and therefore the vector $\Re_{s+t, s }^{t-1}(\mathbf{Q})$ lies in the span of $\{ \Re_{s,s}^{0}(\mathbf{Q}),
\Re_{s+1,s}^{1}(\mathbf{Q}),
...,
\Re_{s+t, s }^{t}(\mathbf{Q}) \}$.
\end{lemma}
\begin{proof}

By lemma \ref{lm:Pst_value}, we know value of each entry of $\mathbf{P}_{s,t}$ and $\mathbf{P'}_{s,t}$. The first $t+1$ columns of $\mathbf{P}_{s,t}$ is

\begin{equation}
\mathbf{P}_{s,t}^{(sub)} =
\begin{bmatrix}
D_{0}^{s}, & {r \choose 1 }D_{0}^{s+1}, & ...&
{r \choose t-1 }D_{0}^{s+t-1}, & {r \choose t }D_{0}^{s+t}\\
0, & {r-1 \choose 0 }D_{1}^{s+1}, & ...& 
{r-1 \choose t-2 }D_{1}^{s+t-1}, & 
{r-1 \choose t-1 }D_{1}^{s+t} \\
0, & 0, & ...&  
{r-2 \choose t-3 }D_{2}^{s+t-1}, & 
{r-2 \choose t-2 }D_{2}^{s+t} \\
., & ., & ... &., &. \\
0, & 0,& ...& 0 , & 
{r-t \choose 0 }  D_{t}^{s+t}  \\
\end{bmatrix}.
\end{equation}

This is an upper triangular matrix. Also, the value on the diagonal is positive since ${r-i \choose 0} = 1$ and $D_{t}^{s+t} > 0$ ( by Claim \ref{clm:d_ri_positive} )
for all $0 \leq i \leq t \leq \ell$ and $r > \ell$. Therefore, the submatrix $\mathbf{P}_{s,t}^{1(sub)}$ is full rank, so that $rank(\mathbf{P}_{s,t}^{(sub)}) = t+1$. It also implies that the rank of $\mathbf{P}_{s,t}$ is $t+1$ since the rank of $\mathbf{P}_{s,t}$ is larger or equal to the rank of column spaces of $\mathbf{P}_{s,t}^{1(sub)}$ and less or equal to the number of rows in $\mathbf{P}_{s,t}$, which are both $t+1$.

Next, we calculate the rank of the matrix $\mathbf{P'}_{s,t}$. We first show that every $(t+2) \times (t+2)$ submatrix of $\mathbf{P'}_{s,t}$ below has rank $t+1$.
The submatrix $\mathbf{P}_{s,t}^{'(sub,i)}$ consists of the first $t$ columns, the $i^{th}$ column and the last column for any $i$ with  $t+1 \leq i \leq \ell$. This matrix can be written as following:  

\begin{equation}
\mathbf{P}_{s,t}^{'(sub,i)} =
\begin{bmatrix}
D_{0}^{s}, & {r \choose 1 }D_{0}^{s+1}, & ...&
{r \choose t-1 }D_{0}^{s+t-1}, & {r \choose i }D_{0}^{s+i}, & D_0^{r+s}\\
0, & {r-1 \choose 0 }D_{1}^{s+1}, & ...& 
{r-1 \choose t-2 }D_{1}^{s+t-1}, & 
{r-1 \choose i-1 }D_{1}^{s+i}, & D_1^{r+s} \\
0, & 0, & ...&  
{r-2 \choose t-3 }D_{2}^{s+t-1}, & 
{r-2 \choose i-2 }D_{2}^{s+i}, & D_2^{r+s} \\
., & ., & ... &., &.,& . \\
0, & 0,& ...&  {r-t+1 \choose 0 }  D_{t-1}^{s+t-1}, & 
{r-t+1 \choose i-t+1 }  D_{t-1}^{s+i}, & D_{t-1}^{r+s}  \\
0, & 0,& ...& 0 , & 
{r-t \choose i-t }  D_{t}^{s+i}, & D_t^{r+s}  \\
0,& 0,& ...& {r-t+1 \choose 0} D_{t}^{s+t-1}, &
[{r-t+1 \choose i-t+1}- {r-t \choose i-t } ] D_{t}^{s+i},&  0  \\
\end{bmatrix}.
\end{equation}
The determinant of $\mathbf{P}_{s,t}^{(sub,i)}$ is 
\begin{align*}
|\mathbf{P}_{s,t}^{(sub,i)}| 
& = \left( \prod_{j=0}^{t-2} {r-j \choose 0} D_{j}^{s+j} \right) \times |\mathbf{P}_{s,t}^{(3 \times 3,i)}|,
\end{align*}
where $\mathbf{P}_{s,t}^{(3 \times 3,i)} \in \mathbb{R}^{3 \times 3}$ is defined below:
$$
\mathbf{P}_{s,t}^{(3 \times 3,i)} 
= 
\begin{bmatrix}
 {r-t+1 \choose 0 }  D_{t-1}^{s+t-1}, & 
{r-t+1 \choose i-t+1 }  D_{t-1}^{s+i}, & D_{t-1}^{r+s}  \\
0 , & 
{r-t \choose i-t }  D_{t}^{s+i}, & D_{t}^{r+s}  \\
{r-t+1 \choose 0} D_{t}^{s+t-1}, &
[{r-t+1 \choose i-t+1}- {r-t \choose i-t } ] D_{t}^{s+i},&  0  \\
\end{bmatrix}
= \begin{bmatrix}
  D_{t-1}^{s+t-1}, & 
{r-t+1 \choose i-t+1 }  D_{t-1}^{s+i}, & D_{t-1}^{r+s}  \\
0 , & 
{r-t \choose i-t }  D_{t}^{s+i}, & D_{t}^{r+s}  \\
D_{t}^{s+t-1}, &
[{r-t+1 \choose i-t+1}- {r-t \choose i-t } ] D_{t}^{s+i},&  0  \\
\end{bmatrix}.
$$
$\mathbf{P}_{s,t}^{(3 \times 3,i)} $ is the right bottom $3 \times 3$ submatrix of $\mathbf{P}_{s,t}^{(sub,i)}$. 
Before we show that the determinant of $\mathbf{P}_{s,t}^{(3 \times 3,i)}$ is zero, we introduce a property of $D^{t}_i$.
\begin{claim}
\label{clm:d_linear_relation}
When $\mu(\cdot)$ is defined in Eqn.\eqref{eqn:thmdummysymm}, for all $p,q \in \{0,1,2,...,d-1\}$ with $0 \leq p+q \leq d-1$, the ratios of $D^{p}_{q}$ and $D^{p}_{q+1}$ can be written as an affine function of $p$, which is equivalent to
$\frac{D^{p}_{q}}{D^{p}_{q+1}} = c^{(1)}_q p +  c^{(2)}_q $ for some constants $ c^{(1)}_q , c^{(2)}_q \in \mathbb{R}$ depending on $q$.
\end{claim}
The proof of Claim \ref{clm:d_linear_relation} is deferred to Section \ref{sec:proofs_claims}.

The determinant of $\mathbf{P}_{s,t}^{(3 \times 3,i)}$ is
\begin{align*}
|\mathbf{P}_{s,t}^{(3 \times 3,i)}| 
& = && - D_{t-1}^{s+t-1} D_{t}^{r+s}\left[{r-t+1 \choose i-t+1}- {r-t \choose i-t } \right] D_{t}^{s+i}\\
& && + D_{t}^{s+t-1} \left[  
{r-t+1 \choose i-t+1 }  D_{t-1}^{s+i}  D_{t}^{r+s} - D_{t-1}^{r+s} {r-t \choose i-t } D_{t}^{s+i}
\right] \ \ \ (\text{Expand with the first column}) \\ \\
& = && D_{t}^{s+t-1}D_{t}^{r+s}D_{t}^{s+i} \Bigg[
\left[-{r-t+1 \choose i-t+1}+{r-t \choose i-t } \right][c^{(1)}_{t-1}(s+t-1)+c^{(2)}_{t-1}] \\
& && + {r-t+1 \choose i-t+1 }[(c^{(1)}_{t-1}(s+i)+ c^{(2)}_{t-1}] -  {r-t \choose i-t }[c^{(1)}_{t-1}(r+s) + c^{(2)}_{t-1}]
\Bigg]
\ \ \ (\text{Claim \ref{clm:d_linear_relation}}) \\
& = && D_{t}^{s+t-1}D_{t}^{r+s}D_{t}^{s+i}
\left[ {r-t+1 \choose i-t+1}(i-t+1) 
- {r-t \choose i-t }(r-t+1)
\right]c^{(1)}_{t-1} \\
& = && 0.
\end{align*}
It implies that the submatrix $\mathbf{P}_{s,t}^{(sub,i)}$ is not full rank. 
Now if we take away the bottom row and the second last column of $\mathbf{P}_{s,t}^{(sub,i)}$, the submatrix becomes 
$$
\begin{bmatrix}
D_{0}^{s}, & {r \choose 1 }D_{0}^{s+1}, & ...&
{r \choose t-1 }D_{0}^{s+t-1}, &  D_0^{r+s}\\
0, & {r-1 \choose 0 }D_{1}^{s+1}, & ...& 
{r-1 \choose t-2 }D_{1}^{s+t-1}, & D_1^{r+s} \\
0, & 0, & ...&  
{r-2 \choose t-3 }D_{2}^{s+t-1},  & D_2^{r+s} \\
., & ., & ... &., & . \\
0, & 0,& ...&  {r-t+1 \choose 0 }  D_{t-1}^{s+t-1}, & 
 D_{t-1}^{r+s}  \\
0, & 0,& ...& 0 , 
& D_t^{r+s}  \\
\end{bmatrix}.
$$
This is again a full rank upper triangular matrix since its diagonal entries are all positive. Therefore, the second last (or the $(t+1)^{th}$) column of $\mathbf{P}_{s,t}^{1(sub,i)}$ lies in the span of the other $t+1$ columns. That is, the $i^{th}$ column of matrix $\mathbf{P'}_{s,t}$ can be expressed as the first $t$ columns and the last column of the matrix $\mathbf{P'}_{s,t}$ for all $i$ with $t+1 \leq i \leq \ell$.
Therefore, the rank of $\mathbf{P'}_{s,t}$ is $t+1$.

Finally, we note that matrices $\mathbf{P}_{s,t}$ and $\mathbf{P'}_{s,t}$ only differ in the last row, but their rank is the same. Consequently, the last row, $\Re_{s+t, s }^{t-1}(\mathbf{Q})$, lies in the span of the first $t+1$ rows, which are $\{ \Re_{s,s}^{0} (\mathbf{Q}),
\Re_{s+1,s}^{1} (\mathbf{Q}),
...,
\Re_{s+t, s }^{t} (\mathbf{Q}) \}$.



\end{proof}


\begin{lemma}
\label{lm:overall_rank}
Given the results in Lemma \ref{lm:submatrix_rank} and following Definition \ref{def:row_combination}, then 
$$
\calA = \{
\Re_{0,0}^{0}(\mathbf{Q}) ,
\Re_{1,0}^{1}(\mathbf{Q}),
...,
\Re_{\ell,0}^{\ell}(\mathbf{Q}) \}
$$
forms the basis of row space of matrix $\mathbf{Q}$ and therefore implies that $rank(\mathbf{Q}) = \ell + 1$.
\end{lemma}
\begin{proof}

We prove a stronger version of this lemma: $\Re_{i,j}^k(\mathbf{Q})$ lies in the span of $\calA$ for all $0 \leq i \leq \ell $, $0 \leq k \leq i$, and $0 \leq j \leq i-k$. This result immediately implies that the row $\mathbf{Q}_{\{i,j\}} = \Re_{i,j}^0$ in matrix $\mathbf{Q}$ also lies in the span of $\mathcal{A}$.

We prove it by induction on two indices, which are $i$ and $k$. 
\begin{enumerate}
    \item When $i=0$, $k$ and $j$ can only be zero. We have $\Re_{0,0}^0(\mathbf{Q}) \in \spann(\calA)$. 
    \item When $i=i'$, suppose that $\Re_{i,j}^k(\mathbf{Q}) \in \spann(\calA)$ holds for $0 \leq i \leq i'$, $0 \leq k \leq i$ and $0 \leq j \leq i-k$.
    \item When $i=i'+1$, we prove that $\Re_{i'+1,j}^k(\mathbf{Q})$  lies in the span of $\calA$ for all $0 \leq k \leq i'+1$, and $0 \leq j \leq i-k$ by using another induction on $k$. In this induction process, $k$ is taking value from $i'+1$ to $0$.

\begin{enumerate}
    \item When $k=i'+1$, we know $\Re_{i'+1,i'+1}^{i'} \in \spann(\calA)$ by plugging  $s=0$ and $t=i'+1$ in Lemma \ref{lm:submatrix_rank} . 
    
    \item Suppose $\Re_{i'+1, j}^{k'}(\mathbf{Q}) \in \spann(\calA)$ for $k=k'+1,.., i'+1$ and $0\leq j \leq i'+1 - k$ for some $0 \leq k' \leq i'$
    \item When $k=k'$,
    by Lemma \ref{lm:submatrix_rank}, we know 
    $$
    \Re_{i'+1,i'-k'}^{k'}(\mathbf{Q}) \in \spann(\Re_{i'-k',i'-k'}^{0}(\mathbf{Q}),...,\Re_{i',i'-k'}^{k'}(\mathbf{Q}),\Re_{i'+1,i'-k'}^{k'+1}(\mathbf{Q})) 
    $$ 
    by plugging in $s=i'-k'$ and $t=k'+1$. Since we have 
    $$
    \spann(\Re_{i'-k',i'-k'}^{0}(\mathbf{Q}),...,\Re_{i',i'-k'}^{k'}(\mathbf{Q})) \subseteq \spann(\calA)
    $$ 
    by induction hypothesis on $i$ and $\Re_{i'+1,i'-k'}^{k'+1}(\mathbf{Q}) \in \spann(\calA)$ by the induction hypothesis on $k$, we have 
    \begin{equation}
    \label{eqn:row_i_k_lie_A}
    \Re_{i'+1,i'-k'}^{k'}(\mathbf{Q}) \in \spann(\Re_{i'-k',i'-k'}^{0}(\mathbf{Q}),...,\Re_{i',i'-k'}^{k'}(\mathbf{Q}),\Re_{i'+1,i'-k'}^{k'+1}(\mathbf{Q})) \subseteq \spann(\calA).
    \end{equation}
    
    Then we observe that 
    \begin{equation}
    \label{eqn:row_relation}
    \Re_{i'+1,j}^k(\mathbf{Q}) = 
    \begin{cases}
    \Re_{i'+1,i'-k}^k(\mathbf{Q})  + \sum_{\rho=j}^{i'-k-1} \Re_{i'+1,\rho}^{k+1}(\mathbf{Q}) & \text{ if   } 0 \leq j < i'-k. \\
    \Re_{i'+1,i'-k}^k(\mathbf{Q}) & \text{ if   } j = i'-k \\
    \Re_{i'+1,i'-k}^k(\mathbf{Q}) - \Re_{i'+1,i'-k}^{k+1}(\mathbf{Q})  & \text{ if   } j = i'-k+1.\\
    \end{cases}    
    \end{equation}
    The Eqn. \eqref{eqn:row_relation} follows from 
    \begin{align*}
    \Re_{i'+1, \rho}^{k+1}(\mathbf{Q})
    & = \sum_{\sigma=0}^{k+1} {k+1 \choose \sigma} (-1)^{\sigma} \mathbf{Q}_{\{i'+1,\rho+\sigma \}} \\
    & = \sum_{\sigma=0}^{k} {k \choose \sigma} (-1)^{\sigma} \mathbf{Q}_{\{i'+1,\rho+\sigma \}}
    + \sum_{\sigma=1}^{k+1} {k \choose \sigma-1} (-1)^{\sigma} \mathbf{Q}_{\{i'+1,\rho+\sigma \}} \\
    & = \sum_{\sigma=0}^{k} {k \choose \sigma} (-1)^{\sigma} \mathbf{Q}_{\{i'+1,\rho+\sigma \}}
    - \sum_{\sigma=0}^{k} {k \choose \sigma} (-1)^{\sigma} \mathbf{Q}_{\{i'+1,\rho+\sigma +1\}} \\
    & = \Re_{i'+1, \rho}^{k}(\mathbf{Q}) - \Re_{i'+1, \rho+1}^{k}(\mathbf{Q}),
    \end{align*}
    Then Eqn. \eqref{eqn:row_relation} can be attained by summing over the above equation from $\rho =j$ to $\rho=i'-k-1$.
    
    By Eqn. \eqref{eqn:row_relation}, we know that the vector $\Re_{i'+1,j}^{k'}(\mathbf{Q})$ can be expressed as the combination of some terms in the form of $\Re_{i'+1,\rho}^{k'+1}(\mathbf{Q})$ and $\Re_{i'+1,i'-k' }^{k'}(\mathbf{Q})$. Both terms lie in the span of $A$ by the induction hypothesis on $k$ and Eqn. \eqref{eqn:row_i_k_lie_A}.
    
    Therefore, we can conclude that $\Re_{i'+1,j}^{k'}(\mathbf{Q})$ also lies in the span of $\calA$ for all $0 \leq j \leq i'+1-k'$. It implies that it also holds when $k=k'$ and we establish the induction step on $k$.
\end{enumerate}
After completing mathematical induction proof on $k$, we know that $\Re_{i'+1,j}^k(\mathbf{Q})$ lies in the span of $\calA$ for all $0 \leq k \leq i'+1$ and $0 \leq j \leq i'+1-k$. Consequently, we also finish the induction step on $i$ (when $i= i'+1$).

\end{enumerate}

Finally, we can deduce that $\Re_{i,j}^k(\mathbf{Q})$ lies in the span of $\calA$ for any $0 \leq i \leq \ell $, $0 \leq j \leq i$ and $0 \leq k \leq i-j$. Then we know every row $\mathbf{Q}_{\{i,j\}} = \Re_{i,j}^0(\mathbf{Q})$ in matrix $\mathbf{Q}$ also lies in the span of $\mathcal{A}$. It immediately implies $rank(\mathbf{Q}) = \ell +1$.


\end{proof}

By Lemma \ref{lm:overall_rank}, the rank of the matrix $ \mathbf{Q} = [\mathbf{M'}, \mathbf{Y}]$ equals to $\ell + 1$. This in turn implies that $\bfb_{i,j} = 0 $ for all $i \geq j > 0$ by Lemma \ref{lm:simplified_matrix}. Therefore, the corresponding Faith-Interaction indices satisfy the interaction dummy axiom when $d \geq \ell + r$ and $r > \ell$.

\paragraph{(3) $ r + \ell > d \geq \ell + r$ and $r > \ell$:} Now, we generalize the results in the second case to the last case. We recall that $\bfb_{i,j}$ denotes the interaction indices with $j$ elements in $R$ and $j$ elements in $[d] \backslash R$ (Definition \ref{def:bij}). However, 
when $r + \ell > d$, there are some $\bfb_{i,j}$ that do not exist since there are not enough elements outside $R$.
For example, $\bfb_{\ell,\ell}$ does not exist since there are only $d-r < \ell$ elements outside $R$. 

In this case, we can still compute the matrix of linear equations,  $\mathbf{Q'} = [ \mathbf{M'}, \mathbf{Y}]$, but some rows do not exist. Particularly, all rows corresponding to $\bfb_{i,j}$ with $d-r < j \leq i$ do not exist.
Nevertheless, removing rows do not
increases the rank of the matrix $\mathbf{Q}$. Therefore, by Lemma \ref{lm:overall_rank}, the rank of $\text{rank}(\mathbf{Q'}) \leq \text{rank}(\mathbf{Q}) = \ell + 1 $. Also, we note that the columns in the coefficient matrix $\mathbf{M}$ are linearly independent (since it has a unique solution by Proposition \ref{pro:unique_minimizer}). This implies that the columns in the reduced coefficient matrix $\mathbf{M'}$ are also linearly independent (since $\mathbf{M'}$ is a submatrix of $\mathbf{M}$). Therefore, the rank of the reduced coefficient matrix $\mathbf{M'}$ equals to the number of columns in $\mathbf{M'}$, which is $\ell+1$. 

Overall, we have $ \ell + 1 \geq \text{rank}(\mathbf{Q'}) \geq \text{rank}(\mathbf{M'}) = \ell +1 $. That is, $\text{rank}(\mathbf{Q'}) = \ell +1$, which in turn implies that $\bfb_{i,j} = 0 $ for all $i \geq j > 0$ by Lemma \ref{lm:simplified_matrix}. Therefore, the corresponding Faith-Interaction indices satisfy the interaction dummy axiom when $ r + \ell > d \geq \ell + r$ and $r > \ell$.


Therefore, by summarizing (1)-(3),
we conclude that the interaction dummy axiom holds for all basis function $\f_R$. This result can be generalized to any function $\f(\cdot)$ by applying Lemma \ref{lm:f_decomposable}.

In conclusion, 
the Faith-Interaction indices with respect to the weighting function defined in Eqn.\eqref{eqn:thmdummysymm} satisfy the interaction linearity, symmetry and dummy axioms for all set functions $\f(\cdot):2^d \mapsto \mathbb{R}$ and all maximum interaction order $1 \leq \ell \leq d$.
\end{proof}

\subsubsection{Proof of Necessary Condition of Theorem \ref{thm:thmdummysymm}}
\label{sec:necessity_theorem_dummysymm}

Now we prove the necessary condition of Theorem \ref{thm:thmdummysymm}. That is, Faith-Interaction indices $\Expl$ with a finite weighting function 
satisfy interaction linearity, symmetry, and dummy axioms only if the weighting function $\mu$ has the form in Eqn.\eqref{eqn:thmdummysymm}.

From Proposition \ref{pro:symmetry}, the Faithful-Interaction indices satisfy interaction symmetry axiom if and only if $\mu(S)$ only depends on the size of the input set $|S|$. Therefore, the weighting function must be symmetric. The following lemma show that the weighting function must be in the form in Eqn.\eqref{eqn:thmdummysymm} if the corresponding Faith-Interaction indices satisfy interaction dummy axiom.

\begin{lemma}
\label{lm:necessity_dummy}
Faith-Interaction indices $\Expl$ with a finite and permutation-invariant weighting function 
satisfy the interaction dummy axiom only if the weighting function $\mu$ has the following form: 
\begin{align*}
\mu(S) & \propto \sum_{i=|S|}^{d} {d- |S| \choose i-|S|}(-1)^{i-|S|} g(a,b,i), \  \text{ where }
g(a,b,i) = 
\begin{cases}
1 & \text{ , if } \ i = 0. \\
\prod_{j=0}^{j=i-1} \frac{a(a-b) + j(b-a^2)}{a-b + j(b-a^2)}
& \text{ , if } \   1 \leq i \leq d. \\
\end{cases}
\end{align*} 
for some $a,b \in \R^{+}$ with $a>b$ such that $\mu(S) > 0$ for all $S \subseteq [d]$.
\end{lemma}

\begin{proof}

We now solve the case when the function $\f = \f_R$ is a basis function. Recall that the definition of basis functions is :
$$
\f_R(S) = \begin{cases}
1, & \text{if}\ S \supseteq R \\
0, & \text{otherwise}. \\
\end{cases}
$$ 
Since the weighting function $\mu(\cdot)$ if finite and only depends on the size of the input set, we use the definitions in Section \ref{sec:extra_notations}: $\mu_{|S|} = \mu(S)$ and  $\mubar{|S|} = \sum_{T \supseteq S} \mu(T) = \sum_{i=|S|}^d { d-|S| \choose i-|S|} \mu_i$ for all $S \subseteq [d]$. Since  Faithful-Interaction indices should hold for all maximum interaction orders $1 \leq \ell \leq d$, we restrict the maximum interaction order to $\ell=1$.

Now we use the following proposition from \citet{ding2008formulas} to prove the necessary condition.

\begin{proposition}
\label{pro:closed_form_finite_mu}
(\citet{ding2008formulas}, equation (8)) When the maximum interaction order $\ell = 1$ (no interaction terms) and the set function $\f = \f_R$ is a basis function for some $R \subseteq [d]$ with $|R| = r$, and the weighting function $\mu(S)$ is permutation-invariant and is normalized so that $\mubar{0} = \sum_{S \subseteq [d]} \mu(S) = 1$, then the minimizer of Eqn.\eqref{eqn:weighted_regression}, $\Expl(\f_R, \ell) \in \mathbb{R}^{d+1}$, has the following form:
$$
\Expl_S(\f_R, \ell) = 
\begin{cases}
-\frac{\mubar{1} + (d-1)\mubar{2}}{\varrho}\mubar{r} + \frac{\mubar{1}}{\varrho} \left(r\mubar{r} + (d-r)\mubar{r+1} \right) & \text{, if $S = \phi$} \\
\frac{1}{\varrho(\mubar{1} - \mubar{2})} \left( (\mubar{1}^2 - \mubar{1}\mubar{2})\mubar{r} + \varrho \mubar{r} - (\mubar{1}^2 - \mubar{2})(r\mubar{r} + (d-r)\mubar{r+1} ) \right) & \text{, if $S = \{ i\}$ for $ i \in R$} \\
\frac{1}{\varrho(\mubar{1} - \mubar{2})} \left( (\mubar{1}^2 - \mubar{1}\mubar{2})\mubar{r} + \varrho \mubar{r+1} - (\mubar{1}^2 - \mubar{2})(r\mubar{r} + (d-r)\mubar{r+1} ) \right) & \text{, if $S = \{ i\}$ for $ i \notin R$} \\
\end{cases}
$$
where $\varrho = d\mubar{1}^2 - (d-1)\mubar{2} - \mubar{1}$. 
\end{proposition}
Note that the basis function satisfies $\f_R(S \cup i) = \f_R(S)$ for $i \notin R$ and $S \subseteq [d] \backslash i$. Since the minimizer satisfies the interaction dummy axiom,
we have $\Expl_{\{i\}}(\f_R, \ell) =  0$ for all $i \notin R$, which implies
\begin{equation*}
 (\mubar{1}^2 - \mubar{1}\mubar{2})\mubar{r} + \varrho \mubar{r+1} - (\mubar{1}^2 - \mubar{2})(r\mubar{r} + (d-r)\mubar{r+1} ) = 0.
\end{equation*}

Let $\mubar{1} = a$ and $\mubar{2} = b$. By plugging in $\varrho = d\mubar{1}^2 - (d-1)\mubar{2} - \mubar{1}$, we have 
$$
(a^2 - ab)\mubar{r} + (da^2 - (d-1)b - a) \mubar{r+1} - ra^2\mubar{r} - (d-r)\mubar{r+1}a^2 + rb\mubar{r} + b(d-r)\mubar{r+1} = 0.
$$
By rearranging, we have
\begin{equation}
\label{eqn:mubar_recursive}
\frac{\mubar{r+1}}{\mubar{r}} = \frac{a(a-b) + r(b-a^2)}{(a-b) + r(b-a^2)}.
\end{equation}

Without loss of generality, we assume that $\bar{\mu}_0 = \sum_{S \subseteq [d]} \mu(S) = 1$, so we have $\mubar{0} =1, \mubar{1} = a$ and $\mubar{2} =b$. Since Eqn. \eqref{eqn:mubar_recursive} holds for all $1 \leq r \leq d$, then we can solve $\mubar{k}$ for $3 \leq k \leq d$ by rewinding the above recursive equation.
\begin{equation}
\label{eqn:mubar_closed_form}
\mubar{k} = \prod_{j=0}^{k-1} \frac{a(a-b) + j(b-a^2)}{(a-b) + j(b-a^2)}.
\end{equation}
Then by applying Lemma \ref{clm:mubar_mu_relation}, we can have 
\begin{align*}
\mu(S) = \mu_{|S|} 
& =  \sum_{i=|S|}^{d} {d- |S| \choose i-|S|}(-1)^{i-|S|} \mubar{i} \\
& = \sum_{i=|S|}^{d} {d- |S| \choose i-|S|}(-1)^{i-|S|} \prod_{j=0}^{j=i-1} \frac{a(a-b) + j(b-a^2)}{a-b + j(b-a^2)}, \\
\end{align*}
for some $a,b \in \R^{+}$ with $a>b$ such that $\mu(S) > 0$ for all $S \subseteq [d]$.
 
\end{proof}

\newpage

\subsection{Proof of Theorem \ref{thm:faith-banzhaf}}

\begin{proof}

\textbf{Sufficiency:} Below we show that the Faith-Banzhaf index satisfies interaction linearity, symmetry, dummy, and generalized 2-efficiency axiom.

By Proposition \ref{pro:linearity}, the Faith-Banzhaf index satisfies interaction linearity axiom. By Proposition \ref{pro:symmetry}, the Faith-Banzhaf index satisfies the interaction symmetry axiom. By Proposition \ref{pro:dummy}, when specifying $p_i = \frac{1}{2}$ for all $1 \leq i \leq d$, $\mu(S)=\prod_{i \in S} p_i \prod_{j \not \in S} (1-p_j) = \frac{1}{2^d}$ is the same as the weighting function used in this theorem. Therefore, the Faith-Banzhaf index satisfies the interaction dummy axiom. 

Note that the closed-form expression in Eqn.\eqref{eqn:faith_banzhaf2} is from Proposition 7.1 of \citep{grabisch2000equivalent}. Also, for all $S$ with size $\ell$, \citep{grabisch2000equivalent} has shown that these values coincide with the Banzhaf interaction indices, which has the following form:
$$
\Expl_S^{\text{F-Bzf}}(\f,\ell) = 
\sum_{T \subseteq [d] \backslash S}\frac{1}{2^{d-|S|}} \Delta_S(\f(T))
\ \ \text{ for all } S \in \setlessell 
\text{ with } |S| = \ell.
$$
Also, recall that the generalized 2-efficiency axiom is only defined on the highest-order interaction, where the Faith-Banzhaf and the Banzhaf interaction indices overlap. Therefore, Faith-Banzhaf indices also satisfy the generalized 2-efficiency axiom.

\textbf{Necessity:} Below we show that the Faith-Banzhaf index is the only index that satisfies interaction linearity, symmetry, dummy, and generalized 2-efficiency axiom.

First, when $\ell = d$, 
by Proposition \ref{pro:ell_equals_d}, we have 
$\ex_{[d]}(\f,d) = a(\f,[d])$ for all $d \in \mathbb{N}$. We then apply the following  results for the Banzhaf interaction index.

\begin{claim}
\label{clm:generalized_2eff}
\citep[Theorem~4]{grabisch1999axiomatic}
If an interaction index that satisfies the interaction linearity, symmetry, dummy, generalized 2-efficiency axioms and $\ex_{[d]}(\f,d) = a(\f,[d])$ for all $d \in \mathbb{N}$, then its highest order terms must have the following form:
$$
\ex_S(\f,\ell) = \sum_{T \subseteq [d] \backslash S}\frac{1}{2^{d-|S|}} \Delta_S(\f(T)),
\forall S \in \setlessell \text{ with } |S| = \ell. 
$$
\end{claim}
Therefore, by the above claim, the highest order terms (with $|S| = \ell$) must coincide with the Banzhaf interaction indices. Then we prove that the weighting function should be a constant, i.e. $\mu(S) = c$ for some constant $c>0$ for all $S \subseteq [d]$. 

Now, we consider the case when the maximum interaction order $\ell = 1$ and $\f = \f_R$ is a basis function, where $\f_R(S) = 1$ for all $S \supseteq R$ and $0$ otherwise.
Since the Faithful-Interaction indices that satisfy the interaction symmetry axiom, the corresponding weighting function is symmetric by Proposition \ref{pro:symmetry}. Then, we let $\mubar{|S|} = \sum_{T \supseteq S} \mu(T) = \sum_{i=|S|}^d { d-|S| \choose i-|S|} \mu_i$ for all $S \subseteq [d]$. 

By Proposition \ref{pro:closed_form_finite_mu}, the minimizer of Eqn.\eqref{eqn:weighted_regression} is
$$
\Expl_S(\f_R, \ell) = 
\begin{cases}
-\frac{\mubar{1} + (d-1)\mubar{2}}{\varrho}\mubar{r} + \frac{\mubar{1}}{\varrho} \left(r\mubar{r} + (d-r)\mubar{r+1} \right) & \text{, if $S = \phi$} \\
\frac{1}{\varrho(\mubar{1} - \mubar{2})} \left( (\mubar{1}^2 - \mubar{1}\mubar{2})\mubar{r} + \varrho \mubar{r} - (\mubar{1}^2 - \mubar{2})(r\mubar{r} + (d-r)\mubar{r+1} ) \right) & \text{, if $S = \{ i\}$ for $ i \in R$} \\
\frac{1}{\varrho(\mubar{1} - \mubar{2})} \left( (\mubar{1}^2 - \mubar{1}\mubar{2})\mubar{r} + \varrho \mubar{r+1} - (\mubar{1}^2 - \mubar{2})(r\mubar{r} + (d-r)\mubar{r+1} ) \right) & \text{, if $S = \{ i\}$ for $ i \notin R$} \\
\end{cases},
$$
where  $\varrho = d\mubar{1}^2 - (d-1)\mubar{2} - \mubar{1}$.

Since we have known that the $\ex_{i}(\f_R,\ell)$ must coincide with the Banzhaf interaction indices 
by Claim \ref{clm:generalized_2eff}, we have $\Expl_{\{i\}}(\f_R, \ell) = 0$ for $i \not \in R$ and $\Expl_{\{i\}}(\f_R, \ell) = \frac{1}{2^{|R|-1}}$ for $i \in R$. Equivalently, we have
\begin{equation}
\label{eqn:basis_function_banzhaf}
\begin{cases}
\frac{1}{\varrho(\mubar{1} - \mubar{2})} \left( (\mubar{1}^2 - \mubar{1}\mubar{2})\mubar{r} + \varrho \mubar{r} - (\mubar{1}^2 - \mubar{2})(r\mubar{r} + (d-r)\mubar{r+1} ) \right) = \frac{1}{2^{r-1}}. \\
\frac{1}{\varrho(\mubar{1} - \mubar{2})} \left( (\mubar{1}^2 - \mubar{1}\mubar{2})\mubar{r} + \varrho \mubar{r+1} - (\mubar{1}^2 - \mubar{2})(r\mubar{r} + (d-r)\mubar{r+1} ) \right) = 0.
\end{cases}.
\end{equation}

Subtracting the first equality with the second one, we have  
\begin{equation}
\label{eqn:mubar_recursive2}
\frac{1}{\varrho(\mubar{1} - \mubar{2})} \cdot  \varrho (\mubar{r} -\mubar{r+1} )  = \frac{1}{2^{r-1}}
\Rightarrow 
\frac{\mubar{r} - \mubar{r+1}}{\mubar{1} - \mubar{2}}
= \frac{1}{2^{r-1}}
\Rightarrow \frac{\mubar{r+1} - \mubar{r+2}}{\mubar{r} - \mubar{r+1}} = \frac{1}{2}.
\end{equation}
Note that it holds for all $1 \leq r \leq d-2$. 

Next, by solving $\Expl_{\{i\}}(\f_R, \ell) = 0$ for $i \not \in R$ and for all $1 \leq r \leq d-1$, we have the following result from Eqn.\eqref{eqn:mubar_recursive}:
$$
\mubar{k} = \prod_{j=0}^{k-1} \frac{a(a-b) + j(b-a^2)}{(a-b) + j(b-a^2)}, 
\text{ for some $1 > a = \mubar{1} > b = \mubar{2} > 0$.}
$$

Then by plugging in the above expression to Eqn.\eqref{eqn:mubar_recursive2}, we have
\begin{align*}
0 
& = \mubar{r} - 3 \mubar{r+1} + 2\mubar{r+2} \\
& =  \mubar{r} \left( 
1 - 3 \cdot \frac{a(a-b) + r(b-a^2)}{(a-b) + r(b-a^2)} 
+ 2 \cdot \frac{a(a-b) + r(b-a^2)}{(a-b) + r(b-a^2)} \cdot \frac{a(a-b) + (r+1)(b-a^2)}{(a-b) + (r+1)(b-a^2)} 
\right) \\
& = \mubar{r} \left( 
\left(1 - \frac{a(a-b) + r(b-a^2)}{(a-b) + r(b-a^2)} 
\right)
- 2  \frac{a(a-b) + r(b-a^2)}{(a-b) + r(b-a^2)}  \left( 1-   \frac{a(a-b) + (r+1)(b-a^2)}{(a-b) + (r+1)(b-a^2)} \right)
\right) \\
& = \mubar{r} \left( \frac{(1-a)(a-b)}{(a-b) + r(b-a^2)} - 2  \frac{a(a-b) + r(b-a^2)}{(a-b) + r(b-a^2)} \cdot \frac{(1-a)(a-b)}{(a-b) + (r+1)(b-a^2)} 
\right) \\
& = \frac{\mubar{r}(1-a)(a-b)}{(a-b) + r(b-a^2)} \left(1  - 2  \frac{a(a-b) + r(b-a^2)}{(a-b) + (r+1)(b-a^2)}  \right) \\
& = \frac{\mubar{r}(1-a)(a-b)}{(a-b) + r(b-a^2)} \left( \frac{(a-b) + (r+1)(b-a^2) - 2a(a-b) - 2r(b-a^2)}{(a-b) + (r+1)(b-a^2)}  \right) \\
& = \frac{\mubar{r}(1-a)(a-b)}{(a-b) + r(b-a^2)} \cdot \frac{a - rb +(r-3)a^2 +2ab}{(a-b) + (r+1)(b-a^2)}   \\
& = \frac{\mubar{r}(1-a)(a-b)}{\left[(a-b) + r(b-a^2) \right]\left[(a-b) + (r+1)(b-a^2) \right]} 
\cdot \left[a(1-3a+2b) -r(b-a^2) \right].
\end{align*}
Since we have $1 > a = \mubar{1} > b = \mubar{2} > 0$ and $\mubar{r} > 0$,  we have $a(1-3a+2b) -r(b-a^2) = 0$ for all $1 \leq r \leq d-2$. Then for all $d \geq 4$, we have 
\begin{equation}
\label{eqn:ab_relation}
a(1-3a+2b) -(b-a^2) = a(1-3a+2b) -2(b-a^2) = 0.    
\end{equation}

It implies $b=a^2$ and $a(1-3a+2b)  = 0$. That is, $a = \frac{1}{2}$ and $b = \frac{1}{4}$. By substituting these into Eqn.\eqref{eqn:mubar_recursive}, we have $\mubar{k} = \frac{1}{2^k}$. Then by applying Lemma \ref{clm:mubar_mu_relation}, we get 
\begin{align*}
\mu(S) = \mu_{|S|} 
& =  \sum_{i=|S|}^{d} {d- |S| \choose i-|S|}(-1)^{i-|S|} \mubar{i} = \frac{1}{2^d}, \ \  \forall S \subseteq [d].
\end{align*}

Finally, for $d=3$, from Eqn.\eqref{eqn:ab_relation}, we have 
$$
a(1-3a+2b) -(b-a^2) = 0
\Rightarrow (2a-1)(b-a) = 0
\Rightarrow a = \frac{1}{2}.
$$
Next, we plug in $r=d$ into the first equality in Eqn.\eqref{eqn:basis_function_banzhaf}, we have 
\begin{align}
\frac{1}{2^{d-1}}
& = \frac{(\mubar{1}^2 - \mubar{1}\mubar{2})\mubar{d} + \varrho \mubar{d} - (\mubar{1}^2 - \mubar{2})(d\mubar{d})}{(d\mubar{1}^2 - (d-1)\mubar{2} - \mubar{1})(\mubar{1} - \mubar{2})}  \nonumber \\
& =\mubar{d} \frac{(\mubar{1}^2 - \mubar{1}\mubar{2}) + (d\mubar{1}^2 - (d-1)\mubar{2} - \mubar{1}) - d(\mubar{1}^2 - \mubar{2})}{(d\mubar{1}^2 - (d-1)\mubar{2} - \mubar{1})(\mubar{1} - \mubar{2})}  \nonumber \\
& =\mubar{d} \frac{(\mubar{1}^2 - \mubar{1}\mubar{2}) + \mubar{2}- \mubar{1}}{(d\mubar{1}^2 - (d-1)\mubar{2} - \mubar{1})(\mubar{1} - \mubar{2})}  \nonumber \\
& = \mubar{d} \frac{\mubar{1}-1}{d\mubar{1}^2 - (d-1)\mubar{2} - \mubar{1}}  \nonumber \\
& =  \frac{\mubar{d}( a-1 )}{da^2 - (d-1)b - a} , \ \ (\text{By definition, we have } a=\mubar{1} \text{ and } b=\mubar{2}) 
\label{eqn:r=d}
\end{align}
By plugging in $d=3$, $a=\frac{1}{2}$ and $\mubar{3} = \frac{ab(a-b) + 2b(b-a^2)}{(a-b) + j(b-a^2)}
$ from Eqn.\eqref{eqn:mubar_recursive}, we have 
\begin{align*}
\frac{1}{4} 
& =  \frac{\mubar{d}( a-1 )}{da^2 - (d-1)b - a}  \\
& = \frac{ab(a-b) + 2b(b-a^2)}{(a-b) + 2(b-a^2)} \times \frac{a-1}{3a^2 - 2b - a} \ \ \ \text{By plugging in } d=3  \\
& = \frac{b(-a^2-ab+2b)}{a+b-2a^2} \times \frac{a-1}{3a^2 - 2b - a}  \\
& = \left(-\frac{1}{4}+\frac{3b}{2} \right) \times \frac{-\frac{1}{2}}{\frac{1}{4} - 2b }
\ \ \ \text{By plugging in } a = \frac{1}{2}.
\end{align*}
Therefore, we have $b=\frac{1}{4}$, which implies that $\mu(S) = \frac{1}{2^d}$ using the same argument.

We note that for $d=2$, any weighting function satisfies $\mu_1= c$ and $\mu_0 = \mu_2 = \frac{1}{2} -c $ for some constant $c > 0$ leads to Banzhaf interaction values for $\ell=1,2$.



\end{proof}


\newpage

\subsection{Proof of Theorem \ref{thm:faith_shap}}
In this section, we present
proof for the sufficient condition, the closed-form expressions of Faithful Shapley index, and the necessary condition of Theorem \ref{thm:faith_shap}. For the sufficient condition, we provide two proof. The first one is in Section \ref{sec:faithshap_sufficiency} and is simpler. The second one is in Section \ref{sec:alternative_faithshap_sufficiency} and is similar to the proof of Theorem \ref{thm:thmdummysymm}. 
Next, we derive the closed-form expression of Faithful Shapley  Interaction indices in Section \ref{sec:closed_form_solution_faith_shap}. Finally, we provide the proof of the necessary condition in Section \ref{sec:faithshap_necessity}. 

\subsubsection{Proof of Sufficient Condition of Theorem \ref{thm:faith_shap}}
\label{sec:faithshap_sufficiency}

In the following, we prove that under the weighting function defined in Eqn. \eqref{eqn:faithshap_weight}, the minimizers of Eqn.\eqref{eqn:constrained_weighted_regresion} satisfy interaction linearity, symmetry, efficiency, and dummy axioms.

\textbf{Interaction linearity, symmetry, efficiency axiom:} The minimizers of Eqn.\eqref{eqn:constrained_weighted_regresion} satisfy interaction linearity, symmetry, and efficiency axioms by Proposition \ref{pro:linearity}, \ref{pro:symmetry} and \ref{pro:efficiency}.

\textbf{Interaction dummy axiom:} Below we prove that the optimal solution satisfies the interaction dummy axiom.
The constrained optimization problem can be written as follows:

\begin{equation*}
\small
\ex^{\text{F-Shap}}(\f,\ell) = \min_{\Expl \in \mathbb{R}^{d_\ell}} F_\ell(\f,\ex) = \min \sum_{S \subseteq [d], 1 \leq |S| \leq d-1} \mu_{|S|} \left(
\f(S) - \sum_{T \subseteq S, |T| \leq \ell} \Expl_T(\f, \ell)  \right)^2,
\end{equation*}
\begin{equation}
\label{eqn:constrained_ls_proof}
\text{ subject to } \Expl_{\text{\O}}(\f,\ell) = \f(\text{\O}) \text{   and   }  \sum_{T \subseteq [d], |T| \leq \ell} \Expl_{T}(\f,\ell) = \f([d]),
\end{equation}
where we use the notations:$\mu_{|S|} = \mu(S)$ and  $\bar{\mu}(S)
= \mubar{|S|} 
= \sum_{T \supseteq S, \mu(T) < \infty} \mu_{|T|} = \sum_{i: |S| \leq i \leq d, \mu_i < \infty}{d-|S| \choose i-|S|}\mu_{i}$ since the weighting function only depends on the size of input sets. Also, since multiplying a scalar to $\mu$ does not change the minimizer of Eqn.\eqref{eqn:weighted_regression}, without loss of generality, we let 
$$\mu(S) = \frac{(d-|S|-1)!(|S|-1)!}{(d-1)!} = B(|S|,d-|S|) \propto \frac{d-1}{\binom{d} {|S|}\,|S|\,(d-|S|)},
\text{ for all } S \subseteq [d] 
\text{ with } 1 \leq |S| \leq d-1,
$$
where $B(\cdot,\cdot)$ is a beta function.
%, without loss of generality, we assume that $\mu(S) = \frac{d-1}{\binom{d} {|S|}\,|S|\,(d-|S|)}$ for $S \subseteq [d]$ with $1 \leq |S| \leq d-1$.
Now, we prove the minimizer of Eqn.\eqref{eqn:con_weighted_ls_basis} satisfies interaction dummy axiom.  More generally, we prove that the constrained minimization problem with a dummy feature can be reduced to another problem with only $d-1$ features and the interaction terms containing the dummy feature is zero.
Formally, we have the following lemma:
\begin{lemma}
\label{lm:faith_shap_reduce}
Assume that $i^{\text{th}}$ feature of the set function $\f(\cdot)$ is a dummy feature such that $\f(S) = \f(S \cup i)$ for all $S \subseteq [d] \backslash \{i\}$.
Let $\f':2^{d-1} \mapsto \mathbb{R}$ with $\f'(S) = \f(S)$ for all $S \subseteq [d-1]$. Then we have 
\begin{equation}
\label{eqn:dummy_faith_solution}
\begin{cases}
\Expl_{S}^{\text{F-Shap}}(\f,\ell) = \Expl_{S}^{\text{F-Shap}}(\f',\ell), 
& \text{ for all }  \ \ S \subseteq [d] \backslash \{ i\}, 0 \leq |S| \leq \ell. \\
\Expl_{S \cup \{i\}}^{\text{F-Shap}}(\f,\ell) = 0, & \text{ for all }  \ \ S \subseteq [d] \backslash \{ i\}, 0 \leq |S| \leq \ell - 1. 
\end{cases}
\end{equation}
\end{lemma}

\begin{proof}
Without loss of generality, we assume that $d^{th}$ feature is a dummy feature, such that $\f(S \cup d) = \f(S)$ for all $S \subseteq [d-1]$.

Now, we solve the constrained minimization problem (Eqn.\eqref{eqn:constrained_ls_proof}) by Lagrange multipliers. 
\begin{equation}
\begin{cases}
\frac{\partial \ F_\ell(\f,\ex)}{\partial \Expl_S } = \lambda & \text{  for all  }
S \subseteq [d], 1 \leq |S| \leq \ell.  \\
\sum_{S \in \setlessell} \Expl_S(\f, \ell) = \f([d]). \\
\Expl_{\text{\O}}(\f, \ell) = \f(\emptyset).
\end{cases},
\end{equation}
We note that the partial derivative can be calculated as below:
$$
\frac{\partial \ F_\ell(\f,\ex)}{\partial \Expl_S } 
= -2\sum_{T \supseteq S, T \neq [d]} \mu(T) \left(\f(T) - \sum_{L \subseteq T, |L| \leq \ell} \ex_L(\f,\ell) 
\right)
= \lambda,
\text{  for all  }
S \subseteq [d], 1 \leq |S| \leq \ell.
$$
Now, for convenience, we denote 
$q(T) = \f(T) - \sum_{L \subseteq T, |L| \leq \ell} \ex^{\text{F-Shap}}_L(\f,\ell)$ for all $T \subseteq [d]$. Then we have
\begin{equation}
\label{eqn:lagrange2}
\begin{cases}
\sum_{T: S \subseteq T \subset [d]} \mu(T)q(T) = \frac{-\lambda}{2} & \text{  for all  }
S \subseteq [d], 1 \leq |S| \leq \ell.  \\
q([d]) = 0. \\
q(\text{\O}) = 0.
\end{cases}
\end{equation}
Similarly, the minimizer $\ex^{\text{F-Shap}}(\f',\ell)$ of $F_\ell(\f',\ex)$ satisfies 
\begin{equation}
\label{eqn:lagrange_for_f_prime}
\begin{cases}
\sum_{T: S \subseteq T \subset [d-1]} \mu'(T)q'(T) = \frac{-\lambda'}{2} & \text{  for all  }
S \subseteq [d-1], 1 \leq |S| \leq \ell.  \\
q'([d-1]) = 0.\\
q'(\text{\O}) = 0.
\end{cases}
\end{equation}
where $q:2^{d-1} \mapsto \mathbb{R}$ with $q'(T) = \f'(T) - \sum_{L \subseteq T, |L| \leq \ell} \ex_L^{\text{F-Shap}}(\f',\ell)$ for all $T \subseteq [d-1]$ and $\mu'(T) = B(|T|, d-1-|T|)$ for all $T \subseteq [d-1]$ with $1 \leq |T| \leq d-2$.

We prove that $\ex^{\text{F-Shap}}(\f,\ell)$ defined in Eqn.\eqref{eqn:dummy_faith_solution} satisfies the system of linear equations in Eqn.\eqref{eqn:lagrange2}.

First of all, by definitions of $\f'(\cdot)$ and $\ex^{\text{F-Shap}(\f,\ell)}$, we have 
$$
\ex_{\text{\O}}^{\text{F-Shap}}(\f,\ell)
= \ex_{\text{\O}}^{\text{F-Shap}}(\f,\ell) = \f'(\emptyset) = \f(\emptyset)
\Rightarrow q(\text{\O}) = 0,
$$
and 
$$
\sum_{S \in \setlessell} \Expl_S^{\text{F-Shap}}(\f, \ell)
= \sum_{S \subseteq [d-1], |S| \leq \ell} \ex_S^{\text{F-Shap}}(\f',\ell) 
=\f'([d-1]) = \f([d])
\Rightarrow q([d]) = 0.
$$

Before we prove that
$$
\sum_{T: S \subseteq T \subset [d]} \mu(T) q(T) = \frac{-\lambda}{2}  \text{  for all  }
S \subseteq [d], 1 \leq |S| \leq \ell,
$$
for some $\lambda \in \mathbb{R}$, we first derive some relations between weighting function $\mu(\cdot)$ and $\mu'(\cdot)$ and $q(\cdot)$ and $q'(\cdot)$.

Since we have $\ex^{\text{F-Shap}}_L(\f,\ell) = 0$ for all $L$ containing $\{d\}$ and $ \f(T) = \f(T \cup \{ d\})$ ( Eqn.\eqref{eqn:dummy_faith_solution}), for all $T \subseteq [d-1]$, we have 
\begin{equation}
\label{eqn:q_property1}
q(T \cup \{ d\}) 
= \f(T \cup \{ d\}) - \sum_{L \subseteq T \cup \{ d\}, |L| \leq \ell} \ex^{\text{F-Shap}}_L(\f,\ell) 
= \f(T) - \sum_{L \subseteq T, |L| \leq \ell} \ex^{\text{F-Shap}}_L(\f,\ell) 
= q(T),    
\end{equation}
and
\begin{equation}
\label{eqn:q_property2}
q'(T) 
= \f'(T) - \sum_{L \subseteq T, |L| \leq \ell} \ex^{\text{F-Shap}}_L(\f',\ell) 
= \f(T) - \sum_{L \subseteq T, |L| \leq \ell} \ex^{\text{F-Shap}}_L(\f,\ell) 
= q(T) = q(T \cup \{ d\}). 
\end{equation}


By using a property of the beta function, for positive integers $1 \leq i \leq d-2$,  we have
\begin{equation}
\label{eqn:mu_property}
\mu'_{i} = B(i,d-1-i) = B(i+1,d-1-i) + B(i,d-i) = \mu_{i+1} + \mu_{i},
\end{equation}

Also, for $2 \leq i \leq d-1$, we have 
\begin{align}
\mu_{i} = B(i,d-i)
& = \frac{(i-1)!(d-i-1)!}{(d-1)!}  \nonumber \\
& = \frac{(i-2)!(d-i-1)!}{(d-2)!} \cdot \frac{i-1}{d-1} \nonumber \\
& = B(i-1,d-i) \cdot \frac{i-1}{d-1} \nonumber \\
& = \frac{(i-1)\mu'_{i-1}}{d-1}.
\label{eqn:mu_property2}
\end{align}

(1) For all $S \subseteq [d-1]$ with $1 \leq |S| \leq \ell$, we have

\begin{align*}
\sum_{T: S \subseteq T \subset [d]} \mu(T) q(T) 
& =  \sum_{T: S \subseteq T \subseteq [d-1]} \mu(T) q(T)
+ \sum_{T: S \subseteq T \subset [d-1]} \mu(T \cup \{ d\}) q(T\cup \{ d\}) \\
& = \mu([d-1])q([d-1]) + \sum_{T: S \subseteq T \subset [d-1]} \left(\mu(T) +\mu(T \cup \{ d\}) \right) q(T) \ \ \text{( Using Eqn.\eqref{eqn:q_property1} )} \\
& =  \mu([d-1])q([d-1]) + \sum_{T: S \subseteq T \subset [d-1]} \mu'(T) q(T) \ \
\text{( Using Eqn.\eqref{eqn:mu_property} )} \\
& = \sum_{T: S \subseteq T \subset [d-1]} \mu'(T) q'(T) \ \ 
\text{(Using Eqn.\eqref{eqn:q_property2} and  $q([d-1]) = q'([d-1]) = 0$ )} \\
&  = \frac{-\lambda'}{2}  \ \ 
(\text{Eqn.\eqref{eqn:lagrange_for_f_prime}}).
\end{align*} 

(2) For all $S = \{d\}$, we have  
\begin{align*}
\sum_{T: S \subseteq T \subset [d]} \mu(T) q(T)
& = \sum_{T \subset [d-1]} \mu(T \cup \{d\} ) q(T \cup \{d\}) \\
& = \sum_{T \subset [d-1]}  \frac{|T|\mu'(T)}{d-1}  q'(T) \ \ 
\text{(Using Eqn.\eqref{eqn:mu_property2}, Eqn.\eqref{eqn:q_property2}, and $q(\text{\O}) = q(\{d\}) = 0$)} \\
& = \frac{1}{d-1}\sum_{i \in [d-1]} \sum_{T: \{i\} \subseteq T \subset [d-1]} \mu'(T) q'(T) \\
& = \frac{1}{d-1}\sum_{i \in [d-1]} -\frac{\lambda'}{2} \ \ 
(\text{Eqn.\eqref{eqn:lagrange_for_f_prime}})\\
& = -\frac{\lambda'}{2}.
\end{align*}

(3) For all $S \subseteq [d]$ containing $\{ d\}$ with $ 2 \leq |S| \leq \ell$, we have 
\begin{align*}
\sum_{T: S \subseteq T \subset [d]} \mu(T) q(T)
& = \sum_{T: (S\backslash \{d\}) \subseteq T \subset [d-1]} \mu(T \cup \{d\} ) q(T \cup \{d\}) \\
& = \sum_{T: (S\backslash \{d\}) \subseteq T \subset [d-1]}   \frac{|T|\mu'(T)}{d-1}  q'(T) \ \ 
\text{(Eqn.\eqref{eqn:mu_property2} and Eqn.\eqref{eqn:q_property2})} \\
& = \sum_{T: (S\backslash \{d\}) \subseteq T \subset [d-1]}   \frac{(|T|-|S|+1)\mu'(T)}{d-1}  q'(T) +
\sum_{T: (S\backslash \{d\}) \subseteq T \subset [d-1]}   \frac{(|S|-1 )\mu'(T)}{d-1}  q'(T)  \\
& = \sum_{i \in [d] \backslash S} \frac{1}{d-1}  \sum_{T: (S\backslash \{d\} \cup i) \subseteq T \subset [d-1]}   \mu'(T)  q'(T) +
\frac{(|S|-1)}{d-1} \cdot \sum_{T: S\backslash \{d\} \subseteq T \subset [d-1]} \mu'(T)  q'(T)  \\
& =  \sum_{i \in [d] \backslash S} \frac{-\lambda'}{2(d-1)} - \frac{|S|-1}{d-1} \cdot
\frac{\lambda'}{2}  \ \ 
(\text{Eqn.\eqref{eqn:lagrange_for_f_prime}}) \\
& = (d-|S|) \frac{-\lambda'}{2(d-1)} - \frac{|S|-1}{d-1} \cdot
\frac{\lambda'}{2} \\
& = \frac{-\lambda'}{2}.
\end{align*}
Therefore, combining (1), (2), and (3), we have 
$$
\sum_{T: S \subseteq T \subset [d]} \mu(T) q(T) = \frac{-\lambda'}{2}  \text{  for all  }
S \subseteq [d], 1 \leq |S| \leq \ell.
$$
That is, Eqn.\eqref{eqn:dummy_faith_solution} is the minimizer of Eqn.\eqref{eqn:constrained_ls_proof}. Consequently, the minimizer of Eqn.\eqref{eqn:constrained_ls_proof} satisfies interaction dummy axiom for all $1 \leq \ell \leq d$.
\end{proof}


\newpage

\subsubsection{Alternative proof of Sufficient Condition of Theorem \ref{thm:faith_shap}}
\label{sec:alternative_faithshap_sufficiency}

In the following, we present an alternative proof of sufficient condition of that under the weighting function defined in Eqn. \eqref{eqn:faithshap_weight}, the minimizers of Theorem \ref{thm:faith_shap}. This proof is similar to Theorem \ref{thm:thmdummysymm}. 

\textbf{Interaction linearity, symmetry, efficiency axiom:} The minimizers of Eqn.\eqref{eqn:constrained_weighted_regresion} satisfy interaction linearity, symmetry, and efficiency axioms by Proposition \ref{pro:linearity}, \ref{pro:symmetry} and \ref{pro:efficiency}.

\textbf{Interaction dummy axiom:} Below we prove that the optimal solution satisfies the interaction dummy axiom. 
The constrained optimization problem can be written as follows:

\begin{align*}
\small
\ex^{\text{F-Shap}}(\f_R,\ell) 
& = \min_{\Expl \in \mathbb{R}^{d_\ell}} F_R(\ex) \\
& = \min \sum_{S \supseteq R, S \subseteq [d]} \mu_{|S|} \left( \sum_{T \subseteq S, |T| \leq \ell} \Expl_T(\f_R, \ell) - 1 \right)^2 + \sum_{S \not\supseteq R, S \subseteq [d]} \mu_{|S|} \left( \sum_{T \subseteq S, |T| \leq \ell} \Expl_T(\f_R, \ell) \right)^2,
\end{align*}
\begin{equation}
\label{eqn:con_weighted_ls_basis}
\text{ subject to } \Expl_{\text{\O}}(\f,\ell) = \f(\text{\O}) \text{   and   }  \sum_{T \subseteq [d], |T| \leq \ell} \Expl_{T}(\f,\ell) = \f([d]), 
\end{equation}
where we use the notations:$\mu_{|S|} = \mu(S)$ and  $\bar{\mu}(S)
= \mubar{|S|} 
= \sum_{T \supseteq S, \mu(T) < \infty} \mu_{|T|} = \sum_{i: |S| \leq i \leq d, \mu_i < \infty}{d-|S| \choose i-|S|}\mu_{i}$ since the weighting function only depends on the size of input sets. Also, since multiplying a scalar to $\mu$ does not change the minimizer of Eqn.\eqref{eqn:weighted_regression}, without loss of generality,
, without loss of generality, we assume that $\mu(S) = \frac{d-1}{\binom{d} {|S|}\,|S|\,(d-|S|)}$ for $S \subseteq [d]$ with $1 \leq |S| \leq d-1$.


First, by Lemma \ref{lm:f_decomposable}, we only need to prove that the minimizers of all the basis functions $\f_R$ ( Definition \ref{def:basis_function} ) satisfy the interaction dummy axiom. That is, the minimizer $\ex^{\text{F-Shap}}_S(\f,\ell) = 0$ for all $S$ containing dummy features in $[d] \backslash R$, i.e.
$S \in \setlessell$ with $S \cap ([d] \backslash R) \neq \text{\O}$ .

Let $r = |R|$ denote the size of the set $R$. Now, we separate the problem into three cases: (1) $d \geq \ell \geq  r \geq 0$. (2) $d \geq \ell + r $ and $r > \ell$. (3) $\ell + r > d \geq r > \ell \geq 1$.

\paragraph{(1)  $d \geq \ell \geq  r \geq 0$:} In this case, the minimizer is trivial.

\begin{lemma}
\label{lm:solution_r_small_thm2}
If $\f_R$ is a basis function with $|R| = r \leq \ell \leq d$, the minimizer of Eqn.\eqref{eqn:con_weighted_ls_basis} is
\begin{equation}
\ex^{\text{F-Shap}}_T(\f_R, \ell)
= \begin{cases}
1 & \text{, if  } \ \  T = R. \\
0 & \text{, otherwise.}
\end{cases}
\end{equation}
\end{lemma}

\begin{proof}
If we plug in $\ex^{\text{F-Shap}}_T(\f_R, \ell)$ to Eqn.\eqref{eqn:con_weighted_ls_basis}, we get $F_R(\ex)= 0$. The solution also satisfies the constraints in Eqn. \eqref{eqn:con_weighted_ls_basis}:
\begin{equation}
\label{eqn:constrained_minimizer_r_small}
\Expl^{\text{F-Shap}}_{\text{\O}}(\f,\ell) = \f(\text{\O}) \ \  \text{   and   }  \sum_{T \subseteq [d], |T| \leq \ell} \Expl_{T}^{\text{F-Shap}}(\f,\ell) = 1 = \f([d]). 
\end{equation}
Since $F(\ex)$ is always non-negative, by Proposition \ref{pro:unique_minimizer}, it is the unique minimizer of Eqn.\eqref{eqn:con_weighted_ls_basis}.
\end{proof}
We note that the minimizer in Eqn.\eqref{eqn:constrained_minimizer_r_small} satisfies the interaction dummy axiom, i.e. $\ex_S(\f,\ell) = 0$ if $S \in \setlessell$ with $S \cap R \neq \text{\O}$.

\paragraph{(2) $d \geq \ell + r$ and $r > \ell$:} 
We solve the constrained optimization problem by using Lagrange multiplier. 

\begin{equation}
\label{eqn:lagrange}
\begin{cases}
\frac{\partial \ F(\ex)}{\partial \Expl_S } = \lambda & \text{  for all  }
S \subseteq [d], 1 \leq |S| \leq \ell.  \\
\sum_{S \in \setlessell} \Expl_S(\f_R, \ell) = 1. \\
\Expl_{\text{\O}}(\f_R, \ell) = 0.
\end{cases},
\end{equation}

where $\lambda \in \mathbb{R}$ is the Lagrange multiplier. Now we utilize the symmetry structure in the basis function $\f_R$. By proposition \ref{pro:unique_minimizer}, Eqn.\eqref{eqn:lagrange} has a unique minimizer $\ex^{\text{F-Shap}}(\f_R, \ell)$.

In the basis functions, there are only two kinds of input elements, which are elements in $R$ and not in $R$. Therefore, for $i^{th}$ order interactions terms $\Expl_{T}(\f_R,\ell)$ where $|T| = i$, there are at most $i+1$ distinct values, which has $j$ elements in $R$, $j=0,1,...i$. That is, by the interaction symmetry axiom, there are only $i+1$ different importance value for $i^{th}$ order interactions terms (since if $|T_1| = |T_2|$ and $|T_1 \cap R| = |T_2 \cap R|$ then $T_1$ and $T_2$ are symmetry and $\Expl_{T_1}(\f_R,\ell) = \Expl_{T_2}(\f_R,\ell)$), so there are $ 1 + 2 +... + (\ell + 1)= \frac{(\ell + 2)(\ell + 1)}{2}$ kinds of values in the optimal solution $\Expl(\f_R,\ell)$. Since we have known that $\Expl_{\text{\O}}(\f_R, \ell) = 0$, we then introduce a new notation system to represent the rest $\frac{(\ell + 2)(\ell + 1)}{2}-1$ values.

\begin{definition}
The minimizer
$ \bfb \in \mathbb{R}^{\frac{(\ell +1)(\ell + 2)}{2} - 1 } \text{ is indexed with  }
\bfb_{i,j} = \Expl_S(\f_R,\ell) \text{  with  } |S| = i \text{ and } |S \backslash R| = j,$
where $i, j$ are integers with $0 \leq j \leq i \leq \ell$ and $i+j > 0$.
\end{definition}

The term $\bfb_{i,j}$ means the importance score of an $i^{th}$ order interaction (of size $i$) term with $i-j$ elements lying in $R$ and $j$ element lying in $[d] \backslash R$. Now we can apply the new notation system to rewrite the system of linear equations (Eqn.\eqref{eqn:lagrange}). By plugging in the closed-form solution of partial derivatives with Lemma \ref{lm:bij_parital_derivative}, for all $0 \leq j \leq i \leq \ell, i+j > 0 $, we have 

\begin{equation}
\label{eqn:constrained_eqn1}
-\mubar{r+j}  
+  \sum_{p,q :0 \leq q \leq p \leq \ell, p+q > 0} \left( \sum_{\rho=0}^{i-j} \sum_{\sigma=0}^{j} { i-j \choose \rho} { r-(i-j) \choose p-q-\rho} { j \choose \sigma}{ d-r-j \choose q-\sigma} \mubar{i+p-\rho-\sigma} \bfb_{p,q} \right) = \frac{\lambda}{2}.
\end{equation}
and
\begin{equation}
\label{eqn:constrained_eqn2}
\sum_{p,q:0 \leq q \leq p \leq \ell, p+q > 0} { r \choose p-q }{ d-r \choose q } \bfb_{p,q} = 1.
\end{equation}
Moreover, we write them into the matrix form,
$\mathbf{M}
\begin{bmatrix} 
\lambda \\
\bfb \\ 
\end{bmatrix}= \mathbf{Y}$ defined below.

\begin{definition}
The coefficient matrix $\mathbf{M} \in \mathbb{R}^{\frac{(\ell +1)(\ell + 2)}{2} \times \frac{(\ell +1 ) (\ell + 2)}{2}}$, whose rows and columns are indexed with 2 iterators respectively. The value of each entry is 
$$
\mathbf{M}_{\{i,j\}, \{p,q\}} =
\begin{cases}
0 \ \  &  \text{ if } \ \ i=0, j=0, p=0 \text{ and } q = 0 .\\
-1/2 \ \  &  \text{ if } \ \ i+j > 0,  p=0 \text{ and } q = 0 .\\
{ r \choose p-q }{ d-r \choose q } \ \  &  \text{ if } \ \ i=0, j=0, p+q > 0 .\\
\sum_{\rho=0}^{i-j} \sum_{\sigma=0}^{j} { i-j \choose \rho } { r-(i-j) \choose p-q-\rho} { j \choose \sigma}{d-r-j \choose q-\sigma} \mubar{i+p-s-t} & \text{, otherwise}. \\
\end{cases}
$$
where $i,j,p,q$ satisfy the constraints: $ 0 \leq j \leq i \leq \ell$, and $ 0 \leq q \leq p \leq \ell$. 
\end{definition}

\begin{definition}
\label{def:Y_def_thm2}
$\mathbf{Y} \in \mathbb{R}^{\frac{(\ell + 1) (\ell+2)}{2}}$ is a column vector with each entry $$
\mathbf{Y}_{i,j} = 
\begin{cases}
1 & \text{ if } i = 0 \text{ and } j = 0 \\
\mubar{r+j} & \text{ if } 0 \leq j \leq i \leq \ell, i + j > 0 \\
\end{cases}
$$ 
\end{definition}
We note that the interaction dummy axiom holds for the basis function $\f_R$ if and only if $\bfb_{i,j} = 0$ for all $i,j > 0$  because $j > 0$ means this interaction term contains dummy features, which are lying in $[d] \backslash R$. 

Recall that Lemma \ref{lm:simplified_matrix} states that if we want to prove that some unknown variables are zero in a system of linear equations, we can prove that the rank of a simplified augmented matrix equals to the number of non-zero variables. To use Lemma  \ref{lm:simplified_matrix} to prove it, we now only consider columns corresponding to non-dummy elements (the column indexed with $p=q=0$), $\bfb_{1,0},..., \bfb_{\ell,0}$ and simplify the matrix $\mathbf{M}$ in the following way:

Put
$$
\mathbf{M'} \in \mathbb{R}^{\frac{(\ell+1)(\ell+2)}{2} \times (\ell+1)} \text{, whose columns correspond to } \lambda, \bfb_{1,0},..., \bfb_{\ell,0} \text{ of } \mathbf{M}  
$$
\begin{equation}
\label{eqn:m_definition_thm2}
\text{ with each entry } \mathbf{M'}_{\{i,j\},\{p, 0\} } = 
\begin{cases}
0 \ \  &  \text{ if } \ \ i=0, j=0 \text{ and } p = 0 \\
-1/2 \ \  &  \text{ if } \ \ i+j > 0, \text{ and } p = 0 \\
{ r \choose p } \ \  &  \text{ if } \ \ i=0, j=0 \text{ and } p > 0 \\
\sum_{\rho=0}^{i-j} { i-j \choose \rho} { r-(i-j) \choose p- \rho} \mubar{i+p-\rho}  & \text{, otherwise.} \\
\end{cases}
\end{equation}

The entry $\mathbf{M'}_{\{i,j\},\{p, 0\}}$ can be interpreted as the coefficient of $\bfb_{p,0}$ in the equation $\frac{\partial F(\ex)}{ \partial \bfb_{i,j}} = 0$.
Since we have already known that the system of linear equations, $\mathbf{M}b=\mathbf{Y}$, has a unique solution by Proposition \ref{pro:unique_minimizer}, if we can prove that the rank of the matrix $\mathbf{Q} = [\mathbf{M'}, \mathbf{Y}]$ equals to $\ell + 1$, we get that $\bfb_{i,j} = 0 $ for all $i \geq j > 0$ by Lemma \ref{lm:simplified_matrix}. It implies the interaction dummy axiom holds for the basis function $\f_R$. To calculate the rank of matrix $\mathbf{Q}$, we first define some notations.

\begin{definition}
\label{def:Pst_thm2}
Following Definition \ref{def:row_combination}, we define 
$$
\mathbf{P}_{s,t} = 
\begin{bmatrix}
\mathbf{z_s}  \\
\Re_{s+1,s}^{1}(\mathbf{Q}) \\
...\\
\Re_{s+t, s }^{t}(\mathbf{Q}) \\
\end{bmatrix}, 
\text{ and } 
\mathbf{P'}_{s,t} = 
\begin{bmatrix}
\mathbf{P}_{s,t} \\
\Re_{s+t-1, s }^{t-1}(\mathbf{Q}) - \Re_{s+t, s}^{t-1}(\mathbf{Q}) \\
\end{bmatrix}, 
$$
where 
$$
\mathbf{z_s} 
= \Re_{\max(1,s), \max(1,s)}^{0}(\mathbf{Q})
= \begin{cases}
\Re_{1, 1}^{0}(\mathbf{Q}) & \text{ , if } s = 0.\\
\Re_{s,s}^{0}(\mathbf{Q}) & \text{ , if } s > 0.\\
\end{cases}
$$
and 
$\mathbf{P}_{s,t} \in \mathbb{R}^{(t+1) \times (\ell + 2)}$ and $\mathbf{P'}_{s,t} \in \mathbb{R}^{(t+2) \times (\ell + 2)}$ for 
$0 \leq s \leq \ell-1 $ and $1 \leq t \leq \ell - s$.

\end{definition}

\begin{lemma}
\label{lm:Pst_value_thm2}
Following Definition \ref{def:Dpq} and \ref{def:Pst_thm2}, for any $s \geq 0$, let $s'=\max(1,s)$,
\begin{equation}
\label{eqn:def_pst_value_thm2}
\mathbf{P}^{'}_{s,t} =
\begin{bmatrix}
-\frac{1}{2}, & {r \choose 1 }D_0^{s'+1}, & ...&
{r \choose t-1 }D_0^{s'+t-1}, & {r \choose t }D_0^{s'+t}, &...  & { r \choose \ell  }D_0^{s'+\ell},  & D_0^{r+s'} \\
0, & {r-1 \choose 0 }D_{1}^{s+1}, & ...&
{r-1 \choose t-2 }D_{1}^{s+t-1}, & 
{r-1 \choose t-1 }D_{1}^{s+t}, & ... & { r-1 \choose \ell -1 } D_{1}^{s+\ell}, & D_{1}^{r+s} \\
0, &  0, & ...&  
{r-2 \choose t-3 }D_{2}^{s+t-1}, & 
{r-2 \choose t-2 }D_{2}^{s+t}, & ... & { r-2 \choose \ell-2 } D_{2}^{s+\ell}, & D_{2}^{r+s} \\
., & ., & ... &., &., & ... & .,& .  \\
0, & 0,& ...& {r-t+1 \choose 0 }  D_{t-1}^{s+t-1}, & 
{r-t+1 \choose 1 }  D_{t-1}^{s+t}, & ... & { r-t+1 \choose \ell-t+1 } D_{t-1}^{s+\ell}, & D_{t-1}^{r+s}  \\
0, &  0,& ...& 0 , & 
{r-t \choose 0 }  D_{t}^{s+t}, & ... 
 & { r-t \choose \ell-t } D_{t}^{s+\ell}, & D_{t}^{r+s}  \\
 0,& 0,& ...& {r-t+1 \choose 0} D_{t}^{s+t-1}, & 
[{r-t+1 \choose 1}- {r-t \choose 0 } ] D_{t}^{s+t}, &... & [{r-t+1 \choose \ell-t+1}- {r-t \choose \ell-t } ] D_{t}^{s+\ell}, & 0  \\
\end{bmatrix}.
\end{equation}

Formally, for all $1 \leq t' \leq t+1$ and $0 \leq p \leq \ell+1$, the $(p+1)^{th}$ element of  $(t'+1)^{\ th}$ row of $\mathbf{P}^{'}_{s,t} $ is 
\begin{equation}
\begin{cases}
-\frac{1}{2} & \text{ if } t' = 0 \text{ and } p=0 \\
{r \choose p}D_0^{s'+p} & \text{ if }  t' = 0 \text{ and } 1 \leq p \leq \ell \\
D_0^{r+s'} & \text{ if }  t' = 0 \text{ and } p = \ell + 1 \\
0 & \text{ if } 1 \leq t' \leq t \text{ and } p < t' \\
{r-t' \choose p-t'} D_{t'}^{s+p} 
& \text{ if } 1 \leq t' \leq t  \text{ and }  t' \leq p \leq \ell\\
D_{t'}^{r+s} & \text{ if } 1 \leq t' \leq t \text{ and } p = \ell+1 \\
0 & \text{ if }    t'=t+1 \text{ and } p < t-1  \\
{r-t+1 \choose 0} D_{t}^{s+t-1}  & \text{ if } t'=t+1 \text{ and } p = t-1\\
[{r-t+1 \choose p-t+1}- {r-t \choose p-t } ] D_{t}^{s+p} & \text{ if }    t'=t+1 \text{ and } t \leq  p \leq \ell  \\
0 & \text{ if }    t'=t+1 \text{ and } p =\ell + 1 \\
\end{cases}.
\end{equation}
\end{lemma}
\begin{proof}
First, we observe that the right-down $\mathbb{R}^{(\frac{(\ell+1)(\ell+2)}{2}-1) \times \ell} $ submatrix of $\mathbf{M'}$ is the same as in Eqn.\eqref{eqn:m_definition} in the proof of Theorem \ref{thm:thmdummysymm}\footnote{$D$ is a function of the cumulative weighting function to a real number. Although the value of cumulative function $\bar{\mu}(\cdot)$ in Theorem \ref{thm:thmdummysymm} and \ref{thm:faith_shap} is different, the coefficient of $D$ is the same.}. Therefore, the corresponding entries in the matrix $\mathbf{P}^{'}_{s,t}$ should also be the same as in Lemma \ref{lm:Pst_value} except for the first row and the first column of matrix $\mathbf{P}^{'}_{s,t}$.

Next, we calculate the first row of the matrix $\mathbf{P}^{'}_{s,t}$, which is the $(s',s')^{th}$ row of $\mathbf{M}'$. The first $\ell+1$ elements can be obtained with Eqn. \eqref{eqn:m_definition_thm2} and the last element of it can be obtained with Definition \ref{def:Y_def_thm2}.

Then, we calculate the first column of the matrix $\mathbf{P}^{'}_{s,t}$.

\begin{enumerate}
    \item If $1 \leq t' \leq t$ and $p=0$, the value of $1^{st}$ element of $(t'+1)^{th}$ row of $\mathbf{P'}_{s,t}$ is 
    $$
    \sum_{\sigma=0}^{\sigma=t'} {t' \choose \sigma} (-1)^{\sigma} (\frac{-1}{2})
    = \frac{-1}{2} (1-1)^{t'}
    = 0
    $$

    \item If $t'=t+1$ and $p=0$, the value of the first element of $(t'+1)^{th}$ row of $\mathbf{P'}_{s,t}$ is 
    \begin{align*}
    & \frac{-1}{2} \sum_{\sigma=0}^{t-1} {t-1 \choose \sigma} (-1)^{\sigma} 
    + \frac{-1}{2}  \sum_{\sigma=0}^{t-1} {t-1 \choose \sigma} (-1)^{\sigma} = 0  \\
    \end{align*}
\end{enumerate}

\end{proof}

\begin{lemma}
\label{lm:submatrix_rank_thm2}
Following Definition \ref{def:Pst_thm2}, the rank of matrices $\mathbf{P}_{s,t}$ and $\mathbf{P}^{'}_{s,t}$ are $t+1$ and therefore the vector $\Re_{s+t, s }^{t-1}(\mathbf{Q})$ lies in the span of $\{ \Re_{s',s'}^{0}(\mathbf{Q}),
\Re_{s+1,s}^{1}(\mathbf{Q}),
...,
\Re_{s+t, s }^{t}(\mathbf{Q}) \}$.
\end{lemma}
\begin{proof}
Before proving this lemma, we first introduce some properties of the value of $D^p_1$ (Definition \ref{def:Dpq}) if the weighting function is defined in Eqn. \eqref{eqn:faithshap_weight}.

\begin{claim}
\label{clm:dpq_value_thm2}
When the weighting function $\mu(\cdot)$ defined in Eqn. \eqref{eqn:faithshap_weight}, for all $p,q \in \{1,2,\ldots, d-1 \}$ with $1 \leq p+q \leq d$, we have
$$
D^p_q 
= \sum_{j=0}^q { q \choose j}(-1)^j \mubar{p+j} 
\propto \frac{d-1}{dq { p+q-1 \choose p-1 } }.
$$ 
\end{claim}

\begin{claim}
\label{clm:d_linear_relation_thm2}
When the weighting function $\mu(S)$ is defined in Eqn. \eqref{eqn:faithshap_weight}, for all $p,q \in \{0,1,2,...,d-1\}$ with $0 \leq p+q \leq d-1$, the ratios of $D^{p}_{q}$ and $D^{p}_{q+1}$ can be written as an affine function of $p$, which is equivalent to
$\frac{D^{p}_{q}}{D^{p}_{q+1}} = c^{(1)}_q p +  c^{(2)}_q $ for some constants $ c^{(1)}_q , c^{(2)}_q \in \mathbb{R}$ dependent on $q$.
\end{claim}

By Lemma \ref{lm:Pst_value_thm2}, we know value of each entry of $\mathbf{P}_{s,t}$ and $\mathbf{P'}_{s,t}$. The first $t+1$ columns of $\mathbf{P}_{s,t}$ is

\begin{equation}
\mathbf{P}_{s,t}^{(sub)} =
\begin{bmatrix}
-\frac{1}{2}, & {r \choose 1 }D_0^{s'+1}, & ...&
{r \choose t-1 }D_0^{s'+t-1}, & {r \choose t }D_0^{s'+t} \\
0, & {r-1 \choose 0 }D_{1}^{s+1}, & ...&
{r-1 \choose t-2 }D_{1}^{s+t-1}, & 
{r-1 \choose t-1 }D_{1}^{s+t} \\
0, & 0, & ...&  
{r-2 \choose t-3 }D_{2}^{s+t-1}, & 
{r-2 \choose t-2 }D_{2}^{s+t} \\
., & ., & ... &., &. \\
0, & 0,& ...& 0 , & 
{r-t \choose 0 }  D_{t}^{s+t}  \\
\end{bmatrix}.
\end{equation}

This is a upper triangular matrix and the values on the diagonal are nonzero  by Claim \ref{clm:dpq_value_thm2}. Therefore, the submatrix $\mathbf{P}_{s,t}^{(sub)}$ is full rank, so that $rank(\mathbf{P}_{s,t}^{(sub)}) = t+1$. It also implies that the rank of $\mathbf{P}_{s,t}$ is $t+1$ since the rank of $\mathbf{P}_{s,t}$ is always not smaller than the rank of column spaces of $\mathbf{P}_{s,t}^{1(sub)}$ and not larger then the number  of rows in $\mathbf{P}_{s,t}$, which are both $t+1$.

Next, we calculate the rank of the matrix $P'_{s,t}$. We first show that every $(t+2) \times (t+2)$ submatrix has rank $t+1$. The submatrix consists of the first $t$ columns, the $i^{th}$ column and the last column for all $t+1 \leq i \leq \ell$, which is as following:  

\begin{equation}
\mathbf{P}_{s,t}^{'(sub,i)} =
\begin{bmatrix}
-\frac{1}{2}, & {r \choose 1 }D_0^{s'+1}, & ...&
{r \choose t-1 }D_0^{s'+t-1}, & {r \choose i }D_0^{i+1}, & D_0^{r+s'} \\
0, & {r-1 \choose 0 }D_{1}^{s+1}, & ...& 
{r-1 \choose t-2 }D_{1}^{s+t-1}, & 
{r-1 \choose i-1 }D_{1}^{s+i}, & D_1^{r+s} \\
0, & 0, & ...&  
{r-2 \choose t-3 }D_{2}^{s+t-1}, & 
{r-2 \choose i-2 }D_{2}^{s+i}, & D_2^{r+s} \\
., & ., & ... &., &.,& . \\
0, & 0,& ...&  {r-t+1 \choose 0 }  D_{t-1}^{s+t-1}, & 
{r-t+1 \choose i-t+1 }  D_{t-1}^{s+i}, & D_{t-1}^{r+s}  \\
0, & 0,& ...& 0 , & 
{r-t \choose i-t }  D_{t}^{s+i}, & D_t^{r+s}  \\
0,& 0,& ...& {r-t+1 \choose 0} D_{t}^{s+t-1}, &
[{r-t+1 \choose i-t+1}- {r-t \choose i-t } ] D_{t}^{s+i},&  0  \\
\end{bmatrix}.
\end{equation}

The determinant of $\mathbf{P}_{s,t}^{'(sub,i)}$ is 
\begin{align*}
|\mathbf{P}_{s,t}^{(sub,i)}| 
& = 
-\frac{1}{2}
\prod_{j=1}^{t-2} {r-j \choose 0} D_{j}^{s+j} \times |P_{s,t}^{(3 \times 3,i)}|,
\end{align*}
where
$$
\mathbf{P}_{s,t}^{(3 \times 3,i)} 
= 
\begin{bmatrix}
 {r-t+1 \choose 0 }  D_{t-1}^{s+t-1}, & 
{r-t+1 \choose i-t+1 }  D_{t-1}^{s+i}, & D_{t-1}^{r+s}  \\
0 , & 
{r-t \choose i-t }  D_{t}^{s+i}, & D_{t}^{r+s}  \\
{r-t+1 \choose 0} D_{t}^{s+t-1}, &
[{r-t+1 \choose i-t+1}- {r-t \choose i-t } ] D_{t}^{s+i},&  0  \\
\end{bmatrix}
= \begin{bmatrix}
  D_{t-1}^{s+t-1}, & 
{r-t+1 \choose i-t+1 }  D_{t-1}^{s+i}, & D_{t-1}^{r+s}  \\
0 , & 
{r-t \choose i-t }  D_{t}^{s+i}, & D_{t}^{r+s}  \\
D_{t}^{s+t-1}, &
[{r-t+1 \choose i-t+1}- {r-t \choose i-t } ] D_{t}^{s+i},&  0  \\
\end{bmatrix}
$$
is the right bottom $3 \times 3$ submatrix of $\mathbf{P}_{s,t}^{(sub,i)}$.

Now we prove that the determinant of $P_{s,t}^{(3 \times 3,i)}$ is zero.
The determinant of $\mathbf{P}_{s,t}^{(3 \times 3,i)}$ is
\begin{align*}
|\mathbf{P}_{s,t}^{(3 \times 3,i)}| 
& = && - D_{t-1}^{s+t-1} D_{t}^{r+s}\left[{r-t+1 \choose i-t+1}- {r-t \choose i-t } \right] D_{t}^{s+i}\\
& && + D_{t}^{s+t-1} \left[  
{r-t+1 \choose i-t+1 }  D_{t-1}^{s+i}  D_{t}^{r+s} - D_{t-1}^{r+s} {r-t \choose i-t } D_{t}^{s+i}
\right] \ \ \ (\text{Expand with the first column}) \\ \\
& = && D_{t}^{s+t-1}D_{t}^{r+s}D_{t}^{s+i} \Bigg[
\left[-{r-t+1 \choose i-t+1}+{r-t \choose i-t } \right][c^{(1)}_{t-1}(s+t-1)+c^{(2)}_{t-1}] \\
& && + {r-t+1 \choose i-t+1 }[(c^{(1)}_{t-1}(s+i)+ c^{(2)}_{t-1}] -  {r-t \choose i-t }[c^{(1)}_{t-1}(r+s) + c^{(2)}_{t-1}]
\Bigg]
\ \ \ (\text{Lemma \ref{clm:d_linear_relation}}) \\
& = && D_{t}^{s+t-1}D_{t}^{r+s}D_{t}^{s+i}
\left[ {r-t+1 \choose i-t+1}(i-t+1) 
- {r-t \choose i-t }(r-t+1)
\right]c^{(1)}_{t-1} \\
& = && 0
\end{align*}
It implies that the submatrix $\mathbf{P}_{s,t}^{(sub,i)}$ is not full rank. 
Now if we take away the bottom row and the second last column of $\mathbf{P}_{s,t}^{(sub,i)}$, the submatrix becomes 
$$
\begin{bmatrix}
-\frac{1}{2}, & {r \choose 1 }D_0^{s'+1}, & ...&
{r \choose t-1 }D_0^{s'+t-1},  & D_0^{r+s'} \\
0, & {r-1 \choose 0 }D_{1}^{s+1}, & ...&
{r-1 \choose t-2 }D_{1}^{s+t-1}, & D_1^{r+s} \\
0, & 0, & ...&  
{r-2 \choose t-3 }D_{2}^{s+t-1},  & D_2^{r+s} \\
., & ., & ... &., & . \\
0, & 0,& ...&  {r-t+1 \choose 0 }  D_{t-1}^{s+t-1}, & 
 D_{t-1}^{r+s}  \\
0, & 0,& ...& 0 , 
& D_t^{r+s}  \\
\end{bmatrix}.
$$
This is again a full rank upper triangular matrix since its diagonal entries are all nonzero. Therefore, the second last ($(t+1)^{th}$) column of $\mathbf{P}_{s,t}^{'(sub,i)}$ lies in the span of the other $t+1$ columns. That is, the $i^{th}$ column of matrix $\mathbf{P}'_{s,t}$ can be expressed as the first $t$ columns and the last column of the matrix $P'_{s,t}$ for all $t+1 \leq i \leq \ell$.
Therefore, the rank of $\mathbf{P}'_{s,t}$ is $t+1$.

Finally, we note that matrices $\mathbf{P}_{s,t}$ and $\mathbf{P}'_{s,t}$ only differ in the last row, but their rank is the same. Consequently, the last row, $\Re_{s+t, s }^{t-1}$, lies in the span of the first $t+1$ rows, which are $\{ \Re_{0,0}^{0},
\Re_{s+1,s}^{1},
...,
\Re_{s+t, s }^{t} \}$.
\end{proof}


\begin{lemma}
\label{lm:overall_rank_thm2}
Given the results in Lemma \ref{lm:submatrix_rank_thm2}  and following Definition \ref{def:row_combination}, then 
$$
\calA = \{
\Re_{1,1}^{0}(\mathbf{Q}) ,
\Re_{1,0}^{1}(\mathbf{Q}),
...,
\Re_{\ell,0}^{\ell}(\mathbf{Q}) \}
$$
forms the basis of row space of matrix $\mathbf{Q}$ and therefore $rank(\mathbf{Q}) = \ell + 1$.
\end{lemma}
\begin{proof}

We prove a stronger version of this lemma: $\Re_{i,j}^k(\mathbf{Q})$ lies in the span of $\calA$ for all $0 \leq i \leq \ell $, $0 \leq k \leq i$, and $0 \leq j \leq i-k$. This results immediately imply that row $\mathbf{Q}_{\{i,j\}} = \Re_{i,j}^0$ in matrix $\mathbf{Q}$ also lies in the span of $\mathcal{A}$.

We prove it by induction on two indices, which are $i$ and $k$. 
\begin{enumerate}
    \item When $i=0$, $k$ and $j$ can only be zero. We prove that $\Re_{0,0}^{0}(\mathbf{Q}) = c\Re_{1,0}^{1}(\mathbf{Q})$ for some constant $c$. With Eqn. \eqref{eqn:m_definition_thm2} and  Lemma \ref{lm:Pst_value_thm2} (by applying $s=0$ to the second row of $\mathbf{P}'_{s,t}$), we can calculate the ratio of the $(p+1)^{th}$ element of $\Re_{1,0}^{1}(\mathbf{Q})$ and $\Re_{0,0}^{0}(\mathbf{Q})$. 
    \begin{enumerate}
        \item If $p=0$, the first element of both $\Re_{1,0}^{1}(\mathbf{Q})$ and $\Re_{0,0}^{0}(\mathbf{Q})$ are zero.
        \item If $0 < p \leq \ell$, we have 
        \begin{align*}
         \frac{1}{c} = \frac{{r-1 \choose p-1} D_1^{p} }{ {r \choose p} }  
         = D_1^{p} \frac{p}{r}  
         \propto \frac{d-1}{dp} \frac{p}{r} \ \ \ (\text{Claim \ref{clm:dpq_value_thm2}}) 
          = \frac{d-1}{dr}.
        \end{align*}
        \item If $p=\ell+1$, by Definition \ref{def:Y_def_thm2} , we have
        $$
        \frac{1}{c}
        = \frac{ D_1^{r} }{ 1 } 
        \propto \frac{d-1}{dr}\ \ \ (\text{Claim \ref{clm:dpq_value_thm2}}).
        $$
    \end{enumerate}
    
    Therefore, we have $\Re_{0,0}^0(\mathbf{Q}) \in \spann(\calA)$. 
    
    \item When $i=1$, $\Re_{1,1}^{0}(\mathbf{Q})$ and $\Re_{1,0}^{1}(\mathbf{Q})$ are all in the set $\calA$.
    
    \item When $i=i'$, suppose that $\Re_{i,j}^k(\mathbf{Q}) \in \spann(\calA)$ holds for $0 \leq i \leq i'$, $0 \leq k \leq i$ and $0 \leq j \leq i-k$.
    \item When $i=i'+1$, we prove $\Re_{i'+1,j}^k(\mathbf{Q})$  lies in the span of $\calA$ for all $0 \leq k \leq i'+1$, and $0 \leq j \leq i-k$ by using another induction on $k$. In this induction process, $k$ is taking value from $i'+1$ to $0$.

\begin{enumerate}
    \item When $k=i'+1$, by Lemma \ref{lm:submatrix_rank_thm2}, we know $\Re_{i'+1,i'+1}^{i'} \in \spann(\calA)$ by plugging in $s=0$ and $t=i'+1$. 
    
    \item Suppose $\Re_{i'+1, j}^{k'}(\mathbf{Q}) \in \spann(\calA)$ for $k=k'+1,.., i'+1$ and $0\leq j \leq i'+1 - k$ for some $0 \leq k' \leq i'$
    \item When $k=k'$,
    by Lemma \ref{lm:submatrix_rank}, we know 
    $$
    \Re_{i'+1,i'-k'}^{k'}(\mathbf{Q}) \in \spann(\Re_{i'-k',i'-k'}^{0}(\mathbf{Q}),...,\Re_{i',i'-k'}^{k'}(\mathbf{Q}),\Re_{i'+1,i'-k'}^{k'+1}(\mathbf{Q})) 
    $$ 
    by plugging in $s=i'-k'$ and $t=k'+1$. Since we have 
    $$
    \spann(\Re_{i'-k',i'-k'}^{0}(\mathbf{Q}),...,\Re_{i',i'-k'}^{k'}(\mathbf{Q})) \subseteq \spann(\calA)
    $$ 
    by induction hypothesis on $i$ and $\Re_{i'+1,i'-k'}^{k'+1}(\mathbf{Q}) \in \spann(\calA)$ by the induction hypothesis on $k$, we have 
    \begin{equation}
    \label{eqn:row_i_k_lie_A2}
    \Re_{i'+1,i'-k'}^{k'}(\mathbf{Q}) \in \spann(\Re_{i'-k',i'-k'}^{0}(\mathbf{Q}),...,\Re_{i',i'-k'}^{k'}(\mathbf{Q}),\Re_{i'+1,i'-k'}^{k'+1}(\mathbf{Q})) \subseteq \spann(\calA).
    \end{equation}

    
    Then we observe that 
    \begin{equation}
    \label{eqn:row_relation2}
    \Re_{i'+1,j}^k(\mathbf{Q}) = 
    \begin{cases}
    \Re_{i'+1,i'-k}^k(\mathbf{Q})  + \sum_{\rho=j}^{i'-k-1} \Re_{i'+1,\rho}^{k+1}(\mathbf{Q}) & \text{ if   } 0 \leq j < i'-k. \\
    \Re_{i'+1,i'-k}^k(\mathbf{Q}) & \text{ if   } j = i'-k \\
    \Re_{i'+1,i'-k}^k(\mathbf{Q}) - \Re_{i'+1,i'-k}^{k+1}(\mathbf{Q})  & \text{ if   } j = i'-k+1.\\
    \end{cases}    
    \end{equation}
    The Eqn.\eqref{eqn:row_relation} follows from 
    \begin{align*}
    \Re_{i'+1, \rho}^{k+1}(\mathbf{Q})
    & = \sum_{\sigma=0}^{k+1} {k+1 \choose \sigma} (-1)^{\sigma} \mathbf{Q}_{\{i'+1,\rho+\sigma \}} \\
    & = \sum_{\sigma=0}^{k} {k \choose \sigma} (-1)^{\sigma} \mathbf{Q}_{\{i'+1,\rho+\sigma \}}
    + \sum_{\sigma=1}^{k+1} {k \choose \sigma-1} (-1)^{\sigma} \mathbf{Q}_{\{i'+1,\rho+\sigma \}} \\
    & = \sum_{\sigma=0}^{k} {k \choose \sigma} (-1)^{\sigma} \mathbf{Q}_{\{i'+1,\rho+\sigma \}}
    - \sum_{\sigma=0}^{k} {k \choose \sigma} (-1)^{\sigma} \mathbf{Q}_{\{i'+1,\rho+\sigma +1\}} \\
    & = \Re_{i'+1, \rho}^{k}(\mathbf{Q}) - \Re_{i'+1, \rho+1}^{k}(\mathbf{Q}),
    \end{align*}
    Then Eqn. \eqref{eqn:row_relation2} can be attained by summing over the above equation from $\rho =j$ to $\rho=i'-k-1$.
    
    By Eqn. \eqref{eqn:row_relation2} $\Re_{i'+1,j}^{k'}(\mathbf{Q})$ can be expressed as the combination of some terms in the form of $\Re_{i'+1,\rho}^{k'+1}(\mathbf{Q})$ and $\Re_{i'+1,i'-k' }^{k'}(\mathbf{Q})$. Both terms lie in the span of $A$ by the induction hypothesis on $k$ and Eqn. \eqref{eqn:row_i_k_lie_A2}.
    
    Therefore, we can conclude that $\Re_{i'+1,j}^{k'}(\mathbf{Q})$ also lies in the span of $\calA$ for all $0 \leq j \leq i'+1-k'$. It implies that it also holds when $k=k'$ and we establish the induction step on $k$.
\end{enumerate}
After completing mathematical induction proof on $k$, we know that $\Re_{i'+1,j}^k(\mathbf{Q})$ lies in the span of $\calA$ for all $0 \leq k \leq i'+1$ and $0 \leq j \leq i'+1-k$. Consequently, we also finish the induction step on $i$ (when $i= i'+1$).

\end{enumerate}

Finally, we can deduce that $\Re_{i,j}^k(\mathbf{Q})$ lies in the span of $\calA$ for any $0 \leq i \leq \ell $, $0 \leq j \leq i$ and $0 \leq k \leq i-j$. Then we know that  every row $\mathbf{Q}_{\{i,j\}} = \Re_{i,j}^0(\mathbf{Q})$ in matrix $\mathbf{Q}$ also lies in the span of $\mathcal{A}$, which in turn implies $rank(\mathbf{Q}) = \ell +1$.


\end{proof}



\paragraph{(3) $ r + \ell > d \geq \ell + r$ and $r > \ell$:} Now, we generalize the results in the second case to the last case. We recall that $\bfb_{i,j}$ denotes the interaction indices with $j$ elements in $R$ and $j$ elements in $[d] \backslash R$ (Definition \ref{def:bij}). However, 
when $r + \ell > d$, there are some $\bfb_{i,j}$ that do not exist since there are not enough elements outside $R$.
For example, $\bfb_{\ell,\ell}$ does not exist since there are only $d-r < \ell$ elements outside $R$. 

In this case, we can still compute the matrix of linear equations,  $\mathbf{Q'} = [ \mathbf{M'}, \mathbf{Y}]$, but some rows do not exist. Particularly, all rows corresponding to $\bfb_{i,j}$ with $d-r < j \leq i$ do not exist.
Nevertheless, removing rows do not
increases the rank of the matrix $\mathbf{Q}$. Therefore, by Lemma \ref{lm:overall_rank_thm2}, the rank of $\text{rank}(\mathbf{Q'}) \leq \text{rank}(\mathbf{Q}) = \ell + 1 $. Also, we note that the columns in the coefficient matrix $\mathbf{M}$ are linearly independent (since it has a unique solution by Proposition \ref{pro:unique_minimizer}). This implies that the columns in the reduced coefficient matrix $\mathbf{M'}$ are also linearly independent (since $\mathbf{M'}$ is a submatrix of $\mathbf{M}$). Therefore, the rank of the reduced coefficient matrix $\mathbf{M'}$ equals to the number of columns in $\mathbf{M'}$, which is $\ell+1$. 

Overall, we have $ \ell + 1 \geq \text{rank}(\mathbf{Q'}) \geq \text{rank}(\mathbf{M'}) = \ell +1 $. That is, $\text{rank}(\mathbf{Q'}) = \ell +1$, which in turn implies that $\bfb_{i,j} = 0 $ for all $i \geq j > 0$ by Lemma \ref{lm:simplified_matrix}. Therefore, the corresponding Faith-Interaction indices satisfy the interaction dummy axiom when $ r + \ell > d \geq \ell + r$ and $r > \ell$.


Therefore, by summarizing (1)-(3),
we conclude that the interaction dummy axiom holds for all basis function $\f_R$. This result can be generalized to any function $\f(\cdot)$ by applying Lemma \ref{lm:f_decomposable}.


In conclusion, 
the Faith-Interaction indices with respect to the weighting function defined in Eqn.\eqref{eqn:thmdummysymm} satisfy the interaction linearity, symmetry and dummy axioms for all set functions $\f(\cdot):2^d \mapsto \mathbb{R}$ and all maximum interaction order $1 \leq \ell \leq d$.


\newpage



\subsubsection{Closed-form Solution of Faith-Shap}
\label{sec:closed_form_solution_faith_shap}

In this section, we solve the constrained weighted linear regression problem defined in Eqn.\eqref{eqn:constrained_weighted_regresion} with the weighting function defined in Eqn.\eqref{eqn:faithshap_weight}. We start with solving Faith-Shap indices for basis functions (Lemma \ref{lm:faithshap_for_basis_function}) and then extend the results to general set functions (Lemma \ref{lm:faithshap_for_general_functions}). Lastly, we provide another expression for the highest order terms of Faithful Shapley Interaction indices, i.e. $\ex_S(\f,\ell)$ for $|S| = \ell$, in terms of discrete derivatives (Lemma \ref{lm:faithshap_highest_order}).


First of all, we solve the closed-form solution when the set function $\f(\cdot)$ is a basis function.

\begin{lemma}
\label{lm:faithshap_for_basis_function}
(Faith-Shap for basis functions)
Consider the basis function $\f_R$ defined as 
$ \f_R(S) = 1$ if $S \supseteq R$, otherwise $0$, where $R \subseteq [d]$. Let $\ell$ be the maximum interaction order. Let $\Expl^{\text{F-Shap}}(\f_R,\ell)$ be the solution of the constrained weighted linear regression problem defined in Eqn.\eqref{eqn:constrained_weighted_regresion} with the weighting function defined in Eqn.\eqref{eqn:faithshap_weight}. Then, for all $S \subseteq [d]$ with $|S| \leq \ell$,
\begin{equation}
\label{eqn:solution_basis_function}
\Expl^{\text{F-Shap}}_S(\f_R,\ell)= 
\begin{cases}
(-1)^{\ell - |S| }\frac{|S|}{\ell + |S|} {\ell \choose |S| } \frac{ {|R| - 1 \choose \ell }}{ { |R| + \ell -1 \choose \ell + |S|}} 
& \text{, if } S \subseteq R, |S| \geq 1, \text{ and } |R| > \ell. \\
0 & \text{, if } S \not \subseteq R \text{ and } |R| > \ell. \\
0 & \text{, if } S = \text{\O} \text{ and } |R| > \ell . \\
1 & \text{, if } S = R \text{ and } |R| \leq \ell. \\
0 & \text{, if } S \neq R \text{ and } |R| \leq \ell. \\
\end{cases}
\end{equation}
\end{lemma}
\begin{proof}

For clarity, we let $r = |R|$ and $s = |S|$.
We first deal with the cases when $|R| = r \leq \ell$. By Lemma \ref{lm:solution_r_small_thm2}, the minimizer of Eqn.\eqref{eqn:con_weighted_ls_basis} is 
$$
\ex^{\text{F-Shap}}_T(\f_R, \ell)
= \begin{cases}
1 & \text{, if  } \ \  T = R. \\
0 & \text{, otherwise.}
\end{cases}
$$


Next, we consider the case when $r > \ell \geq 1$ and $d > \ell + r$ . If $S = \text{\O}$, by the constraints, we must have $\Expl^{\text{F-Shap}}_{\text{\O}}(\f,\ell) = \f(\text{\O}) = 0$. If $S \not \subseteq R$, since elements outside $R$ are dummy features, we have $\Expl^{\text{F-Shap}}_S(\f,\ell) = 0$ by the dummy axiom. Also, by symmetric axiom, for all $S \subseteq R$, $\Expl^{\text{F-Shap}}_S(\f,\ell)$ only depends on the size of the set $S$. Therefore, there are only $\ell$ kinds of different values, which are $\Expl^{\text{F-Shap}}_S(\f,\ell)$ for $S \subseteq R$ with $|S| = 1,\cdots,\ell$. For convenience, we use $\Expl^{\text{F-Shap}}_{i}(\f,\ell)$ to deonte $\Expl^{\text{F-Shap}}_{S}(\f,\ell)$ with $|S| = i$ and $S \subseteq R$. 

We solve the problem via Lagrange multiplier. Following the same simplification process in Section \ref{sec:alternative_faithshap_sufficiency}, we get the matrix $\mathbf{P}_{0,\ell}$, which is the matrix in Eqn.\eqref{eqn:def_pst_value_thm2} in Lemma \ref{lm:Pst_value_thm2} and Definition \ref{def:Pst_thm2}. $\mathbf{P}_{0,\ell} \in \mathbb{R}^{(\ell+1) \times (\ell+2)}$ can be expressed as follows.
\begin{equation}
\mathbf{P}_{0,\ell} =
\left(
\begin{array}{@{}rrrrrr|c@{}}
-\frac{1}{2}, & {r \choose 1 }D_0^{2}, & ...&
{r \choose \ell-2 }D_0^{\ell-1}, & {r \choose \ell-1 }D_0^{\ell}, & { r \choose \ell  }D_0^{\ell+1},  & D_0^{r+1} \\
0, & {r-1 \choose 0 }D_{1}^{1}, & ...&
{r-1 \choose \ell-3 }D_{1}^{\ell-2}, & 
{r-1 \choose \ell-2 }D_{1}^{\ell-1}, &  { r-1 \choose \ell -1 } D_{1}^{\ell}, & D_{1}^{r} \\
0, &  0, & ...&  
{r-2 \choose \ell-4 }D_{2}^{\ell-2}, & 
{r-2 \choose \ell-3 }D_{2}^{\ell-1}, &  { r-2 \choose \ell-2 } D_{2}^{\ell}, & D_{2}^{r} \\
., & ., & ... &., &., &  .,& .  \\
0, & 0,& ...& 0, & 
{ r-\ell+1 \choose 0 } D_{\ell-1}^{\ell-1} & { r-\ell+1 \choose 1 } D_{\ell-1}^{\ell}, & D_{\ell-1}^{r}  \\
0, &  0,& ...& 0 , & 
0, & { r-\ell \choose 0 } D_{\ell}^{\ell}, & D_{\ell}^{r}  \\
\end{array} \right)
\end{equation}

Formally, for $0 \leq i \leq \ell $ and $0 \leq j \leq \ell + 1$, the value of the element in $(i+1)^{th}$ row and $(j+1)^{th}$ column is 
\begin{equation}
\begin{cases}
-\frac{1}{2} & \text{ if } i = 0 \text{ and } j=0. \\
{r \choose j}D_0^{j+1} & \text{ if }  i = 0 \text{ and } 1 \leq j \leq \ell. \\
D_0^{r+1} & \text{ if }  i = 0 \text{ and } j = \ell + 1. \\
0 & \text{ if } 1 \leq i \leq \ell \text{ and } j < i. \\
{r-i \choose j-i} D_{i}^{j} 
& \text{ if } 1 \leq i \leq \ell  \text{ and }  i \leq j \leq \ell.\\
D_{i}^{r} & \text{ if } 1 \leq i \leq \ell \text{ and } j = \ell+1 .\\
\end{cases}.
\end{equation}

From Definition \ref{def:Pst_thm2}, this matrix is the augmented matrix that is obtained form applying Gaussian elimination process to the original matrix for solving a system of linear equations. Row $i+1$ in $\mathbf{P}_{0,\ell}$ corresponds to $\Expl^*_{S}(\f,\ell)$ with $|S| = i$ and $S \subseteq R$ ( except that the first row maps to Lagrange multiplier $\lambda$). That is, 
\begin{equation}
\label{eqn:def_p0ell}
\underbrace{\left(
\begin{array}{@{}rrrrrr}
-\frac{1}{2}, & {r \choose 1 }D_0^{2}, & ...&
{r \choose \ell-2 }D_0^{\ell-1}, & {r \choose \ell-1 }D_0^{\ell}, & { r \choose \ell  }D_0^{\ell+1}\\
0, & {r-1 \choose 0 }D_{1}^{1}, & ...&
{r-1 \choose \ell-3 }D_{1}^{\ell-2}, & 
{r-1 \choose \ell-2 }D_{1}^{\ell-1}, &  { r-1 \choose \ell -1 } D_{1}^{\ell} \\
0, &  0, & ...&  
{r-2 \choose \ell-4 }D_{2}^{\ell-2}, & 
{r-2 \choose \ell-3 }D_{2}^{\ell-1}, &  { r-2 \choose \ell-2 } D_{2}^{\ell}\\
., & ., & ... &., &., &  . \\
0, & 0,& ...& 0, & 
{ r-\ell+1 \choose 0 } D_{\ell-1}^{\ell-1} & { r-\ell+1 \choose 1 } D_{\ell-1}^{\ell} \\
0, &  0,& ...& 0 , & 
0, & { r-\ell \choose 0 } D_{\ell}^{\ell} \\
\end{array} \right)}_{\text{ upper triangular matrix}}
\left( 
\begin{array}{@{}c}
\lambda \\
\Expl^{\text{F-Shap}}_{1}(\f_R,\ell)  \\
\Expl^{\text{F-Shap}}_{2}(\f_R,\ell)  \\
. \\
\Expl^{\text{F-Shap}}_{\ell-1}(\f_R,\ell) \\
\Expl^{\text{F-Shap}}_{\ell}(\f_R,\ell)  \\
\end{array}
\right)
= 
\left( 
\begin{array}{@{}c}
D_{0}^{r+1}\\
D_{1}^{r} \\
D_{2}^{r}  \\
. \\
D_{\ell-1}^{r}  \\
D_{\ell}^{r}  \\
\end{array}
\right),
\end{equation}
where $\Expl^{\text{F-Shap}}_{i}(\f,\ell) = \Expl^{\text{F-Shap}}_{S}(\f,\ell)$ with $|S| = i$ and $S \subseteq R$.
Now, we can verify the solution 
$$
D^p_q 
\propto \frac{d-1}{dq { p+q-1 \choose p-1 } } \propto \frac{(p-1)!(q-1)!}{(p+q-1)!}. 
$$

we can solve $\Expl^{\text{F-Shap}}(\f,\ell)$ with the above matrix equation. 
Claim \ref{clm:dpq_value_thm2} gives us the value of $D_{q}^{p}$, for all $p,q \in \{1,2,\ldots, d-1 \}$, we have 
\begin{equation}
\label{eqn:def_Dpq_closed_form}
D^p_q 
\propto \frac{d-1}{dq { p+q-1 \choose p-1 } } \propto \frac{(p-1)!(q-1)!}{(p+q-1)!}.  
\end{equation}

We begin by the following claim.

\begin{claim}
\label{clm:closed_form_basis_function}
For $ 1 \leq i \leq \ell < r$, 
$$
\sum_{j=0}^{\ell - i} 
{ r- i \choose j} \frac{D_{i}^{j+i}}{D^{r}_{i}} 
\frac{(r-1)!(\ell + j+i -1)!}{(r+\ell-1)!(j+i-1)!} { r - j-i - 1 \choose \ell - i-j} (-1)^{\ell - i - j} 
= 1.
$$
\end{claim}

Now, by plugging in 
$$\ex_i^{\text{F-Shap}}(\f_R,\ell) = (-1)^{\ell - i }\frac{i}{\ell + i} {\ell \choose i } \frac{ {r - 1 \choose \ell }}{ { r + \ell -1 \choose \ell + i}}
$$ 
to the $(i+1)^{th}$ row of matrix Eqn.\eqref{eqn:def_p0ell}, we have
\begin{align*}
& \sum_{j=0}^{\ell-i} {r-i \choose j} D^{j+i}_i \ex_{i+j}^{\text{F-Shap}}(\f_R,\ell) \\
& = \sum_{j=0}^{\ell-i} {r-i \choose j} D^{j+i}_i (-1)^{\ell - i -j}\frac{i}{\ell + i+j} {\ell \choose i+j } \frac{ {r- 1 \choose \ell }}{ { r + \ell -1 \choose \ell + i+j}}
\\
& = \sum_{j=0}^{\ell-i} {r-i \choose j} D^{j+i}_i \frac{(r-1)!(\ell + j+i -1)!}{(r+\ell-1)!(j+i-1)!} { r - j-i - 1 \choose \ell - i-j} (-1)^{\ell - i - j} 
\\
& = D^{r}_i \ \ \ (\text{By Claim \ref{clm:closed_form_basis_function}}).
\end{align*}
Therefore, the solution in Eqn.\eqref{eqn:solution_basis_function} satisfies the system of linear equations.

Finally, we deal with the case when $\ell +r > d \geq r > \ell \geq 1$. We define a new set function $\f_R':2^{d+\ell} \mapsto \mathbb{R}$ with $\f'_R(S) =
\f(S \cap [d])$ for all $S \subseteq [d + \ell]$. Then we can easily see that $\f'_R(\cdot)$ is also a basis function and 
features $d+1,\cdots, d+ \ell$ are dummy nods, which have no effect to the set function. Then by Lemma \ref{lm:faith_shap_reduce}, we have $\ex_S^{\text{F-Shap}}(\f_R,\ell) = \ex_S^{\text{F-Shap}}(\f'_R,\ell)$ for all $S \subseteq [d]$ with $|S| \leq \ell$. That is, the values of these interaction terms are the same but $\f'_R(\cdot)$ has more features. We can apply the previous results since $d' = d+ \ell > \ell + r$. We note that Eqn.\eqref{eqn:solution_basis_function} does not depend on the number of features $d$, so Eqn.\eqref{eqn:solution_basis_function} is the minimizer in this case.

\end{proof}

\begin{lemma}
\label{lm:faithshap_for_general_functions}
(Faith-Shap for general set functions)
For any set function $\f:2^d \mapsto \mathbb{R}$,
the Faith-Shap interaction indices have the following form:
\begin{equation*}
\ex^{\text{F-Shap}}_S(\f,\ell) =
a(S) + (-1)^{\ell - |S| }\frac{|S|}{\ell + |S|} {\ell \choose |S| } \sum_{T \supset S, |T| > \ell} \frac{ {|T| - 1 \choose \ell }}{ { |T| + \ell -1 \choose \ell + |S|}} a(T), \;\; \forall S \in \mathcal{S}_\ell,
\end{equation*}
where $a(S)$ is the Möbius transform of $\f$.
\end{lemma}

By Lemma 3 in \citet{shapley1953value}, any set function $\f: 2^d \rightarrow \mathbb{R}$ can be written into a linear combination of basis functions:
$$
\f(S) = \sum_{R \subseteq [d]} a(R)\f_R(S).
$$
Using the linearity axiom, we can get extend the closed-form minimizers for basis functions in Lemma \ref{lm:faithshap_for_basis_function} to general functions as follows:
\begin{align*}
\Expl^{\text{F-Shap}}(\f,\ell) 
& = \sum_{R \subseteq [d]} a(R)\Expl^{\text{F-Shap}}(\f_R,\ell).
\end{align*}
Then we could obtain 
$\ex_S^{\text{F-Shap}}$ by using the above equation. For any $S \in \setlessell$.
\begin{align*}
& \ex^{\text{F-Shap}}_S(\f,\ell) \\
& = \sum_{R \subseteq [d]} a(R)\Expl^{\text{F-Shap}}_S(\f_R,\ell) \\
& = a(S)\Expl^{\text{F-Shap}}_S(\f_S,\ell) 
+ \sum_{R: S \not \subseteq R, R \subseteq [d] } a(R)\Expl^{\text{F-Shap}}_S(\f_R,\ell) 
 \\
& + \sum_{R: S \subset R, |R| \leq \ell, R \subseteq [d] } a(R)\Expl^{\text{F-Shap}}_S(\f_R,\ell) 
+ \sum_{R: S \subset R, |R| > \ell, R \subseteq [d] } a(R)\Expl^{\text{F-Shap}}_S(\f_R,\ell) 
\\
& = a(S) + 0 + 0 +  (-1)^{\ell - |S| }\frac{|S|}{\ell + |S|} {\ell \choose |S| } \sum_{R: S \subset R \subseteq [d], |R| > \ell} \frac{ {|R| - 1 \choose \ell }}{ { |R| + \ell -1 \choose \ell + |S|}} a(R)
\ \ \ \text{(Lemma \ref{lm:faithshap_for_basis_function}) } \\
& = a(S) + (-1)^{\ell - |S| }\frac{|S|}{\ell + |S|} {\ell \choose |S| } \sum_{T \supset S, |T| > \ell} \frac{ {|T| - 1 \choose \ell }}{ { |T| + \ell -1 \choose \ell + |S|}} a(T).
\end{align*}

\begin{lemma}
\label{lm:faithshap_highest_order}
(Faith-Shap in the form of discrete derivatives)
The highest order term of Faithful Shapley Interaction indices have the following form:
\footnote{We have tried to solve expressions for general orders in terms of discrete derivatives. However, even for the second-highest term  $|S| = \ell -1$, there is no clear expressions. Specifically, for $|S| = \ell -1$, we have
$$
\Expl^{\text{F-Shap}}_S(\f,\ell) = 
\frac{(2\ell-3)!}{(\ell- 2)!(\ell-1)!}\sum_{T \subseteq [d] \backslash S}\frac{(|T|+\ell-2)!(d-|T|-1)!}{(d-1+l)!}(\ell^2 -\ell d+ 2 \ell |T| - 2\ell - |T| +1)\Delta_S f(T) \text{   for   } |S| = \ell-1.
$$}
$$
\Expl_S^{\text{F-Shap}}(\f,\ell) = \frac{(2\ell -1)!}{((\ell-1)!)^2 } 
\sum_{T \subseteq [d] \backslash S}\frac{(\ell+|T|-1)!(d-|T|-1)!}{(d+\ell-1)!}   \Delta_S(\f(T))
\ \ \text{ for all } S \in \setlessell 
\text{ with } |S| = \ell.
$$
\end{lemma}

Using the formula for basis functions in 
Lemma \ref{lm:faithshap_for_basis_function}, for any $S \subseteq [d]$ with $|S| = \ell$, we get 
\begin{align*}
& \Expl^{\text{F-Shap}}_S(\f,\ell)  = \sum_{R \subseteq [d], R \supseteq S} a(R)\Expl^{\text{F-Shap}}_S(\f_R,\ell) \\
& = \sum_{ W \subseteq [d]  \backslash S} a(W \cup S)\Expl_S^{\text{F-Shap}}(\f_{W \cup S},\ell)  \ \ \ 
\text{ where } W = R \backslash S \text{ and } \Expl^{\text{F-Shap}}_S(\f_R,\ell) = 0 \text{ for all } S \not \subseteq R. \\
& =  a(S) + 
\sum_{ \substack{W \subseteq [d] \backslash S \\ |W| > \ell - |S|}} a(W \cup S) (-1)^{\ell - |S| }  \frac{(|W \cup S|-1)!(\ell + |S| -1)! (|W|-1)!}{(|W \cup S| -\ell-1)! (|W \cup S| +\ell-1)! (|S|-1)!(\ell-|S|)!} \\
& =  \Delta_S(\f(\text{\O})) + 
\underbrace{\sum_{ \substack{W \subseteq [d] \backslash S \\ |W| > \ell - |S|}} a(W \cup S) (-1)^{\ell - |S| }  \frac{(|W \cup S|-1)!(\ell + |S| -1)! (|W|-1)!}{(|W \cup S| -\ell-1)! (|W \cup S| +\ell-1)! (|S|-1)!(\ell-|S|)!}}_{(i)}.
\end{align*}
The second last equality is obtained by applying Lemma \ref{lm:faithshap_for_basis_function} and the last equality is due to Claim \ref{clm:mobius_to_discrete_derivaitive} below.

\begin{claim}
\label{clm:mobius_to_discrete_derivaitive}
(\citet{sundararajan2020shapley} ,Lemma 2) Möbius coefficients and discrete derivatives are related by following relation:
$$
a(T \cup S) = \sum_{W \subseteq T} (-1)^{|T| - |W|} \Delta_S (\f(W))
$$
for $S$ and $T$ such that $S \cap T = \text{\O}$.
\end{claim}

Now, we analyze (i).
{\small
\begin{align}
(i) & = \frac{(-1)^{\ell - |S| }(\ell + |S| -1)!}{(|S|-1)! (\ell-|S|)! } 
\sum_{\substack{W \subseteq [d] \backslash S \\ |W| > \ell - |S|}} a(W \cup S)   \frac{(|W \cup S|-1)! (|W|-1)!}{(|W \cup S| -\ell-1)! (|W \cup S| +\ell-1)! } \nonumber \\
& =  \frac{(-1)^{\ell - |S| }(\ell + |S| -1)!}{(|S|-1)! (\ell-|S|)! } 
\sum_{\substack{W \subseteq [d] \backslash S \\ |W| > \ell - |S|}}
\sum_{ U \subseteq W} (-1)^{|U|-|W|} \Delta_S(\f(U))
\frac{(|W \cup S|-1)! (|W|-1)!}{(|W \cup S| -\ell-1)! (|W \cup S| +\ell-1)! } \nonumber \\
& \ \ \ \ \ \ \ \text{ (Using Claim \ref{clm:mobius_to_discrete_derivaitive}) }
\nonumber \\
& = \frac{(-1)^{\ell - |S| }(\ell + |S| -1)!}{(|S|-1)! (\ell-|S|)! } 
\sum_{U \subseteq [d] \backslash S} \Delta_S(\f(U))
\sum_{ \substack{ W \supseteq U, W \subseteq [d]\backslash S \\ |W| > \ell - |S|}} (-1)^{|U|-|W|}
\frac{(|W \cup S|-1)! (|W|-1)!}{(|W \cup S| -\ell-1)! (|W \cup S| +\ell-1)! }.
\label{eqn:expression_(i)_closed_form}
\end{align}}
Now, we analyze the inner sum. For clarity, we let $w = |W|$, $s = |S|$ and $u = |U|$. We also use the properties of beta functions: $B(m,n) = \frac{(m-1)!(n-1)!}{(m+n-1)!} = \int_{0}^1 x^{m-1}(1-x)^{n-1} dx$ for any $m,n \subseteq \mathbb{N}$.

\begin{align*}
& \sum_{ W \supseteq U, W \subseteq [d]\backslash S, |W| > \ell - |S|} (-1)^{|U|-|W|} 
\frac{(|W \cup S|-1)! (|W|-1)!}{(|W \cup S| -\ell-1)! (|W \cup S| +\ell-1)! } \\
& = \sum_{w = \max(u,\ell-s+1)}^{d-s} { d-s-u\choose w-u } (-1)^{u-w}
\frac{(w+s-1)! (w-1)!}{(w + s -\ell-1)! (w + s +\ell-1)! } \\
& = \frac{1}{(\ell-1)!}\sum_{w = \max(u,\ell-s+1)}^{d-s} { d-s-u\choose w-u } (-1)^{u-w}
\frac{(\ell-1)!(w+s-1)!}{ (w + s +\ell-1)! } \prod_{i=1}^{\ell-s}(w-i) \\
& = \frac{1}{(\ell-1)!}\sum_{w = \max(u,\ell-s+1)}^{d-s} { d-s-u\choose w-u } (-1)^{u-w}B(w+s,\ell) \prod_{i=1}^{\ell-s}(w-i) \\
& \ \ \ \text{(Definition of Beta function)}
 \\
& = \frac{1}{(\ell-1)!}\sum_{w = \max(u,\ell-s+1)}^{d-s} { d-s-u\choose w-u } (-1)^{u-w} \left(\prod_{i=1}^{\ell-s}(w-i) \right) \int_{0}^1 x^{w+s-1}(1-x)^{\ell-1} dx \\
& \ \ \ \text{(Property of Beta function)}
 \\
& = \frac{1}{(\ell-1)!}  \int_{0}^1 x^{s-1} (1-x)^{\ell-1} \sum_{w = \max(u,\ell-s+1)}^{d-s} { d-s-u\choose w-u } (-1)^{u-w} \left(\prod_{i=1}^{\ell-s}(w-i) \right) x^{w} dx  \\
& \ \ \ \text{(Exchange of integration)}
 \\
& = \frac{1}{(\ell-1)!}  \int_{0}^1 x^{\ell-1} (1-x)^{\ell-1} \sum_{w = \max(u,1)}^{d-\ell} { d-\ell-u\choose w-u } (-1)^{u-w} x^{w} dx  
\ \ \ (\text{Using } s = \ell).\\
\end{align*}

\paragraph{(1)} For the case when $u \geq 1$, we have 
\begin{align*}
& \frac{1}{(\ell-1)!}  \int_{0}^1 x^{\ell-1} (1-x)^{\ell-1} \sum_{w = \max(u,1)}^{d-\ell} { d-\ell-u\choose w-u } (-1)^{u-w} x^{w} dx  \\
& = \frac{1}{(\ell-1)!}  \int_{0}^1 x^{\ell-1+u} (1-x)^{\ell-1} \sum_{w'=0}^{d-\ell-u} { d-\ell-u\choose w' } (-1)^{w'} x^{w'} dx  
\ \ \ (\text{let } w' = w-u)\\
& = \frac{1}{(\ell-1)!}  \int_{0}^1 x^{\ell-1+u} (1-x)^{\ell-1} (1-x)^{d-\ell-u} dx   \\
& = \frac{1}{(\ell-1)!}  \int_{0}^1 x^{\ell-1+u} (1-x)^{d-u-1} dx   \\
& = \frac{ B(\ell+u, d-u)}{(\ell-1)!}  \\
& = \frac{(\ell+u-1)!(d-u-1)!}{(d+\ell-1)!(\ell-1)!}.  \\
\end{align*}

\paragraph{(2)} For the case when $u =0$, we have 
\begin{align*}
& \frac{1}{(\ell-1)!}  \int_{0}^1 x^{\ell-1} (1-x)^{\ell-1} \sum_{w = \max(u,1)}^{d-\ell-u} { d-\ell-u\choose w-u } (-1)^{u-w} x^{w} dx  \\
& = \frac{1}{(\ell-1)!}  \int_{0}^1 x^{\ell-1} (1-x)^{\ell-1} \sum_{w=1}^{d-\ell} { d-\ell \choose w } (-1)^{w} x^{w} dx  \\
& = \frac{1}{(\ell-1)!}  \int_{0}^1 x^{\ell-1} (1-x)^{\ell-1} \sum_{w=0}^{d-\ell} { d-\ell \choose w } (-1)^{w} x^{w} dx  - \frac{1}{(\ell-1)!}  \int_{0}^1 x^{\ell-1} (1-x)^{\ell-1} dx  \\
& = \frac{1}{(\ell-1)!}  \int_{0}^1 x^{\ell-1} (1-x)^{\ell-1} (1-x)^{d-\ell} dx  - \frac{ B(\ell,\ell)}{(\ell-1)!}  \\
& = \frac{1}{(\ell-1)!}  \int_{0}^1 x^{\ell-1} (1-x)^{d-1} dx   - \frac{ B(\ell,\ell)}{(\ell-1)!} \\
& = \frac{ B(\ell, d)}{(\ell-1)!}  - \frac{B(\ell,\ell)}{(\ell-1)!} \\
& = \frac{(\ell+u-1)!(d-u-1)!}{(d+\ell-1)!(\ell-1)!} - \frac{(\ell-1)!}{(2\ell-1)!}. \\
\end{align*}

Now, combining the two cases and plugg into Eqn.\eqref{eqn:expression_(i)_closed_form}, we have 
{\small
\begin{align*}
(i) & = \frac{(-1)^{\ell - |S| }(\ell + |S| -1)!}{(|S|-1)! (\ell-|S|)! } 
\sum_{U \subseteq [d] \backslash S} \Delta_S(\f(U))
\sum_{ \substack{ W \supseteq U, W \subseteq [d]\backslash S \\ |W| > \ell - |S|}} (-1)^{|U|-|W|}
\frac{(|W \cup S|-1)! (|W|-1)!}{(|W \cup S| -\ell-1)! (|W \cup S| +\ell-1)! }  \\
& = \frac{(2\ell -1)!}{(\ell-1)! } 
\sum_{U \subseteq [d] \backslash S} \Delta_S(\f(U))
\sum_{ \substack{ W \supseteq U, W \subseteq [d]\backslash S \\ |W| > \ell - |S|}} (-1)^{|U|-|W|}
\frac{(|W \cup S|-1)! (|W|-1)!}{(|W \cup S| -\ell-1)! (|W \cup S| +\ell-1)! } \\
& \ \ \ (\text{using } s = |S| = \ell)\\
& = \frac{(2\ell -1)!}{((\ell-1)!)^2 } 
\sum_{U \subseteq [d] \backslash S}\frac{(\ell+u-1)!(d-u-1)!}{(d+\ell-1)!}   \Delta_S(\f(U)) - \Delta_S(\f(\text{\O})).
\end{align*}}
Therefore, by substituting $U$ with $T$, we get the desired result:
$$
\Expl_S^{\text{F-Shap}}(\f,\ell) = \frac{(2\ell -1)!}{((\ell-1)!)^2 } 
\sum_{T \subseteq [d] \backslash S}\frac{(\ell+|T|-1)!(d-|T|-1)!}{(d+\ell-1)!}   \Delta_S(\f(T)).
$$

\newpage


\subsubsection{Proof of Necessary Condition of Theorem \ref{thm:faith_shap}}
\label{sec:faithshap_necessity}


Now we prove the necessary condition of Theorem \ref{thm:faith_shap}. That is, Faith-Interaction indices $\Expl$ 
satisfy linearity, symmetry, efficiency and dummy axioms only if the weighting function $\mu$ has the form in Eqn.\eqref{eqn:faithshap_weight}.

From Proposition \ref{pro:symmetry}, the Faithful-Interaction indices satisfy the interaction symmetry axiom if and only if $\mu(S)$ only depends on the size of the input set $|S|$. Therefore, the weighting function must be symmetric.
Also, by Proposition \ref{pro:efficiency}, Faithful-Interaction indices satisfy the interaction efficiency axiom if and only if $\mu(\text{\O}) = \mu([d]) = \infty$. Therefore, the weighting function must be permutation-invariant and has infinity measure on the empty set and the full set.

Then, the following lemma show that the weighting function must be in the form of Eqn.\eqref{eqn:faithshap_weight} if the corresponding Faith-Interaction indices additionally satisfy dummy axiom.

\begin{lemma}
\label{lm:necessity_dummy_shapley}
Faith-Interaction indices $\Expl$ with a  weighting function, which is permutation-invariant and has $\mu(\text{\O}) = \mu([d]) = \infty$, 
satisfy the interaction dummy axiom only if the weighting function $\mu$ has the following form: 
$$
\mu(S) \propto
\frac{d-1}{\binom{d} {|S|}\,|S|\,(d-|S|)}
\text{   for all   } S \subseteq [d]
\text{   with   } 1 \leq |S| \leq d-1, 
\ \ \text{ and } \ \ 
\mu(\text{\O}) = \mu([d]) = \infty
$$
\end{lemma}

\begin{proof}

We now solve the case when the function $\f = \f_R$ is a basis function for some $R \subseteq [d]$. Recall that the definition of basis functions is :
$$
\f_R(S) = \begin{cases}
1, & \text{if}\ S \supseteq R \\
0, & \text{otherwise}. \\
\end{cases}
$$ 
Since the weighting function $\mu(\cdot)$ if finite and only depends on the size of the input set, we use the definitions in Section \ref{sec:extra_notations}: $\mu_{|S|} = \mu(S)$ and  $\mubar{|S|} = \sum_{T \supseteq S} \mu(T) = \sum_{i=|S|}^d { d-|S| \choose i-|S|} \mu_i$ for all $S \subseteq [d]$. Since  Faithful-Interaction indices should hold for all maximum interaction orders $1 \leq \ell \leq d$, we restrict the maximum interaction order to $\ell=1$. We now use the following results from \citet{ding2008formulas}.


\begin{proposition}
(\citet{ding2008formulas}, Theorem 16) When the maximum interaction order $\ell = 1$ (no interaction terms) and the set function $\f = \f_R$ is a basis function for some $R \subseteq [d]$ with $|R| = r$, and the weighting function $\mu(S)$ is permutation-invariant and has $\mu(\text{\O}) = \mu([d]) = \infty$, the minimizer of Eqn.\eqref{eqn:constrained_weighted_regresion}, $\Expl(\f_R, \ell) \in \mathbb{R}^{d+1}$, has the following form:
\begin{equation}
\label{eqn:ding_thm16}
\Expl_S(\f_R, \ell) = 
\begin{cases}
0 & \text{, if $S = \phi$.} \\
\frac{d-r}{d} \cdot  \frac{\mubar{r}- \mubar{r+1}}{\mubar{1} - \mubar{2}}   + \frac{1}{d}
& \text{, if $S = \{ i\}$ for $ i \in R$.} \\
\frac{-r}{d} \cdot \frac{\mubar{r}- \mubar{r+1}}{\mubar{1} - \mubar{2}}  + \frac{1}{d} & \text{, if $S = \{ i\}$ for $ i \notin R$.} \\
\end{cases}
\end{equation}
Note that when $R = [d]$, we let $\mubar{d+1} = 0$ for clarity.
\end{proposition}
Since the optimal solution $\Expl(\f_R,\ell)$ satisfies the symmetry, dummy and efficiency axiom, we should have 
\begin{equation}
\label{eqn:shapley_for_basis_function}
\Expl_{\{i\}}(\f_R, \ell) =  
\begin{cases}
\frac{1}{r} & \text{, if } i \in R. \\
0 & \text{, otherwise.}
\end{cases}
\ \ \text{, and } \ \ 
\Expl^*_{\text{\O}}(\f_R, \ell) =  0.    
\end{equation}

By comparing Eqn.\eqref{eqn:ding_thm16} and Eqn.\eqref{eqn:shapley_for_basis_function}, we obtain
$$
 \frac{\mubar{r}- \mubar{r+1}}{\mubar{1} - \mubar{2}} = \frac{1}{r} 
\ \ \ \text{ for }  1 \leq r \leq d-1.
$$
By letting $\mubar{1} - \mubar{2} = k$ and  plugging in the definition of $\mubar{r}$, i.e. $\mubar{r} = \sum_{i=r}^d { d-r \choose i-r} \mu_i$, we get 
$$
 \sum_{i=r}^{d-1} { d-1-r \choose i-r} \mu_i = \frac{k}{r} 
\ \ \ \text{ for }  1 \leq r \leq d-1.
$$
There are $d-1$ unknown parameters, $\mu_1,\cdots,\mu_{d-1}$, and $d-1$ equations. Hence, the solution is uniquely determined (in terms of $k$).
By solving the equation from $r=d-1$ to $r=1$, we obtain this unique solution:
$$
\mu_{|S|} = \mu(S) \propto
\frac{d-1}{\binom{d} {|S|}\,|S|\,(d-|S|)}
\text{   for all   } S \subseteq [d]
\text{   with   } 1 \leq |S| \leq d-1.
$$

\end{proof}

Now, by Lemma \ref{lm:necessity_dummy_shapley}, we conclude that the necessary condition of Theorem \ref{thm:faith_shap} holds. 

\newpage

\section{Proof of Claims}
\label{sec:proofs_claims}
In this sections, we give the omitted proof of claims that are used in the our proof in Appendix \ref{sec:proofs_propositions} and \ref{sec:proofs_theorems}.

\subsection{Proof of Claim \ref{clm:p_q_relation}}
\begin{proof}
For any $S \subseteq [d]$,
\begin{align*}
\sum_{T \supseteq S} (-1)^{|T| - |S|}p(T)
& = \sum_{T \supseteq S} (-1)^{|T| - |S|} \sum_{L \supseteq T} q(L) \\
& = \sum_{L \supseteq S} q(L)  \sum_{T: S \subseteq T \subseteq L} (-1)^{|T| - |S|} \\
& = \sum_{L \supseteq S} q(L)  \sum_{t=0}^{|L| - |S|} {|L| - |S| \choose t} (-1)^{t} \\
& = \sum_{L \supseteq S} q(L)  (1-1)^{|L|-|S|} \\
& = q(S) \\
\end{align*}
\end{proof}

\subsection{Proof of Claim \ref{clm:all_zero}}
\begin{proof}
Suppose that there exists a $\ex(\f,\ell) \in \mathbb{R}^{2^d-1}$ satisfying $p(L) = 0$ for all $L \subseteq [d]$.

By Claim \ref{clm:p_q_relation}, we have 
$q(S) = \sum_{T \supseteq S} (-1)^{|T| - |S|}p(T) = 0$ for all $S \subseteq [d]$. That is,
\begin{equation*}
0 = q(S) = \begin{cases}
\mu'(S) \left(1 - \sum_{T \subseteq S, |T| \leq d-1} \Expl_T(\f, \ell) \right)  & \text{ , if $S = [d]$} \\
\mu'(S) \left(\sum_{T \subseteq S, |T| \leq d-1} \Expl_T(\f, \ell) \right) & \text{, otherwise.} \\
\end{cases}
\end{equation*}
By the definition of $\mu'(\cdot)$, we have $\mu'(S) > 0$ for all $S \subseteq [d]$. We have 
\begin{align*}
& \sum_{T \subseteq S, |T| \leq d-1} \Expl_T(\f, \ell) =1 & \text{ , if $S = [d]$.} \\
& \sum_{T \subseteq S, |T| \leq d-1} \Expl_T(\f, \ell)  = 0 & \text{ , if $S \subset [d].$} 
\end{align*}
If we plug in $S = \phi$, we get $\Expl_{\phi}(\f,\ell) = 0$. Then we plug in $T = \{ i\}$ for some $1 \leq i \leq d$, we get $\Expl_{\phi}(\f,\ell) + \Expl_{\{i\}}(\f,\ell) = 0$, which implies $\Expl_{\{i\}}(\f,\ell) = 0$. 

Similarly, we obtain $\Expl_{T}(\f,\ell) = 0$ for all  $T \in \setlessell$ by simple induction. However, this $\Expl(\f,\ell)$ fails to satisfy the first equality:
$$
1 - \sum_{T \subseteq S, |T| \leq d-1} \Expl_T(\f, \ell)  = 1 \neq 0,
$$ 
which is a contradiction. Therefore, there is no $\ex(\f,\ell) \in \mathbb{R}^{2^d-1}$ satisfying $p(L) = 0$ for all $L \subseteq [d]$.

\end{proof}

\subsection{Proof of Claim \ref{clm:mubar_mu_relation}}
\begin{proof}
\begin{align*}
\sum_{T \supseteq S} (-1)^{|T| - |S|} \bar{\mu}(T) 
& = \sum_{T \supseteq S} (-1)^{|T| - |S|} \sum_{L \supseteq T} \mu(L)    \\
& = \sum_{L,T: L \supseteq T \supseteq S}  (-1)^{|T| - |S|} \mu(L) \\
& = \sum_{L: L \supseteq S} \mu(L) \sum_{T:  L \supseteq T \supseteq S} (-1)^{|T| - |S|}  \\
& = \sum_{L: L \supseteq S} \mu(L) \sum_{i=|S|}^{|L|} { |L| - |S| \choose i - |S|}(-1)^{i- |S|}  \\
& = \sum_{L: L \supseteq S} \mu(L) (1-1)^{|L| - |S|}  \\
& = \mu(S)\\
\end{align*}

\end{proof}


\subsection{Proof of Claim \ref{clm:mubar_closeform}}

\begin{proof}
Let $\prodd_t = \prod_{j=0}^{t-1} \frac{a(a-b) + j(b-a^2)}{a -b + j(b-a^2)}$. By definition, we have

\begin{align*}
\mubar{t} 
& = \sum_{k=t}^{d} {d-t \choose k-t } \mu_k \\
& = \sum_{k=t}^{d} {d-t \choose k-t } 
\sum_{i=k}^{d} {d-k \choose i-k}(-1)^{i-k} \prod_{j=0}^{j=i-1} \frac{a(a-b) + j(b-a^2)}{a-b + j(b-a^2)} \\
& = \sum_{k=t}^{d} {d-t \choose k-t } 
\sum_{i=k}^{d} {d-k \choose i-k}(-1)^{i-k} \prodd_i   \\
& = \sum_{k=t}^{d} \sum_{i=k}^{d} \prodd_i {d-t \choose k-t }  {d-k \choose i-k}(-1)^{i-k} \\
& = \sum_{i=t}^{d} \prodd_i  \sum_{k=t}^{i} (-1)^{i-k}{d-t \choose k-t }  {d-k \choose i-k} \\
& = \sum_{i=t}^{d} \prodd_i  \sum_{k=t}^{i} (-1)^{i-k} \frac{(d-t)!(d-k)!}{(k-t)!(d-k)!(i-k)!(d-i)!} \\
& = \sum_{i=t}^{d} \prodd_i \frac{(d-t)!}{(d-i)!} \sum_{k=t}^{i}(-1)^{i-k}  \frac{1}{(k-t)!(i-k)!} \\
& = \sum_{i=t}^{d} \prodd_i \frac{(d-t)!}{(d-i)!(i-t)!} \sum_{k=t}^{i} (-1)^{i-k} \frac{(i-t)!}{(k-t)!(i-k)!} \\
& = \sum_{i=t}^{d} \prodd_i {d-t \choose i-t} \sum_{k=t}^{i}(-1)^{i-k} {i-t \choose i-k} \\
& = \prodd_t  + \sum_{i=t+1}^{d} \prodd_i(-1)^{i-k} {d-t \choose i-t} (1 - 1)^{i-t} \\
& = \prodd_t \\
\end{align*}
Therefore, we have $\mubar{t} = \prodd_t =  \prod_{j=0}^{t-1} \frac{a(a-b) + j(b-a^2)}{a -b + j(b-a^2)}$ for all $1 \leq t \leq d$. Also, when $t=0$, since we assume that $\sum_{S \subseteq [d]} \mu(S) = 1$, we have $\mu_0 = 1$.

\end{proof}

\subsection{Proof of Claim \ref{clm:d_ri_positive}}

\begin{proof}
We prove $D^{p}_q > 0$ for all $p,q \in \{0,1,2,...,d\}$ with $0 \leq p+q \leq d$ by induction. 

(i) First, for all $p$ with $0 \leq p \leq d$, we have 
\begin{align*}
D^{p}_{d-p}
& = \sum_{j=0}^{d-p}{d-p \choose j} (-1)^{j}\mubar{p+j} 
\ \ \ \text{ (Definition \ref{def:Dpq}) } \\
& = \sum_{T: S \subseteq T \subseteq [d] }{d - |S| \choose |T| - |S|} (-1)^{|T|-|S|}\bar{\mu}(T) 
\ \ \ \text{ , for some } S \text{ with } |S| = p \\
& = \mu(S) \ \ \ (\text{Claim }  \ref{clm:mubar_mu_relation} ) > 0.
\end{align*}
(ii) Also, we have $D^p_0 = \mubar{p} = \sum_{j=0}^{d-p} {d-p \choose j } \mu_{j+p} > 0$.

Then, for all $p,q \in \{0,1,2,...,d-1\}$ with $0 \leq p+q \leq d$, we have

\begin{align*}
D^{p}_{q}
& = \sum_{j=0}^{q}{q \choose j} (-1)^{j}\mubar{p+j} 
\ \ \ \text{ (Definition \ref{def:Dpq}) } \\
& = \mubar{p} + \mubar{p+q} (-1)^{p+q} + \sum_{j=1}^{q-1} \left({q-1 \choose j} + {q-1 \choose j-1} \right) (-1)^{j}\mubar{p+j} 
\ \ \ \text{ (Pascal's rule) } \\
& =  \mubar{p} + \mubar{p+q}(-1)^{p+q} + \sum_{j=1}^{q-1} \left( {q-1 \choose j}  (-1)^{j}\mubar{p+j} + {q-1 \choose j-1}  (-1)^{j}\mubar{p+j} \right) \\
& =  \mubar{p} + \mubar{p+q} (-1)^{p+q} + \sum_{j=1}^{q-1}  {q-1 \choose j}  (-1)^{j}\mubar{p+j} + \sum_{j=1}^{q-1}{q-1 \choose j-1}  (-1)^{j}\mubar{p+j}  \\
& = \sum_{j=0}^{q-1}  {q-1 \choose j}  (-1)^{j}\mubar{p+j} - \sum_{j=0}^{q-1}{q-1 \choose j}  (-1)^{j}\mubar{p+1+j} \\
& = D^{p}_{q-1} - D^{p+1}_{q}.
\end{align*}
Therefore, we have $D^{p}_{q} + D^{p+1}_{q} =  D^{p}_{q-1}$ (iii). Now, we use this formula to prove $D^{p}_{q}$ is positive by using induction. 

\begin{itemize}
    \item When $p=d$, we have $D^p_0 > 0$ by (ii).
    \item Assume that when $p = i$, $D^p_q > 0$ for all $0 \leq  q \leq d-p$. 
    \item When $p = i-1$, we now prove that $D^p_q > 0$ for all $0 \leq  q \leq d-p$. By (i) and (ii),
    we have $D^p_0 > 0 $ and $D^{p}_{d-p} > 0$. Then by (iii), we have $D^{p}_{d-p} + D^{p+1}_{d-p} =  D^{p}_{d-p-1}$, since we have already had $D^{p}_{d-p} > 0$ and $ D^{p+1}_{d-p} > 0$ by induction hypothesis, we have $D^{p}_{d-p-1} > 0$. Then by calling (iii) recursively from $q= d-p$ to $q=1$, we conclude that $D^p_q > 0$ for all $0 \leq  q \leq d-p$, which also conclude the induction proof.
\end{itemize}


\end{proof}



\subsection{Proof of Claim \ref{clm:row_operation}}
\begin{proof}
First of all, we develop the following equality.

\begin{claim}
\label{clm:I_value}
For any integers $\ell,r, t' p', \rho$ with constraints $1 \leq \ell < r $, $0 \leq t' \leq \ell$, $ 0 \leq p' \leq \ell$ and $0 \leq \rho \leq t'$, we have
\begin{equation}
\sum_{\sigma=0}^{t'-\rho} {t' \choose \sigma} (-1)^{\sigma} {t'-\sigma \choose \rho} { r-t'+\sigma \choose p'- \rho} = \begin{cases}
0 & \text{ if } p' < t' \\
(-1)^{t'-\rho}{r-t' \choose p' - t' } {t' \choose \rho} & \text{ if }  t' \leq p' \leq \ell \\
\end{cases}
\end{equation}
\end{claim}
The proof is delayed to Section \ref{sec:proof_claim_I_value}
By using the definition of $M'$ in Eqn.\eqref{eqn:m_definition} , we have 
\begin{align*}
\sum_{\sigma=0}^{t'} {t' \choose \sigma} (-1)^{\sigma} M'_{\{s'+t', s'+\sigma \},\{p',0\}} 
& = 
\sum_{\sigma=0}^{t'} {t' \choose \sigma} (-1)^{\sigma} \sum_{\rho=0}^{t'-\sigma} {t'-\sigma \choose \rho} { r-t'+\sigma \choose p'- \rho} \mubar{s'+t'+p'-\rho}  \\
& = 
\sum_{\sigma=0}^{t'}
\sum_{\rho=0}^{t'-\sigma} {t' \choose \sigma} (-1)^{\sigma}  {t'-\sigma \choose \rho} { r-t'+\sigma \choose p'- \rho} \mubar{s'+t'+p'-\rho} 
 \\
& = 
\sum_{\rho=0}^{t'}  \sum_{\sigma=0}^{t'-\rho} {t' \choose \sigma} (-1)^{\sigma} {t'-\sigma \choose \rho} { r-t'+\sigma \choose p'- \rho} \mubar{s'+t'+p'-\rho} 
 \\ 
& = 
\sum_{\rho=0}^{t'}  \mubar{s'+t'+p'-\rho}  \sum_{\sigma=0}^{t'-\rho} {t' \choose \sigma} (-1)^{\sigma} {t'-\sigma \choose \rho} { r-t'+\sigma \choose p'- \rho} 
\\ 
\end{align*}

Then, by plugging in the results of Claim. \ref{clm:I_value}, we have 
\begin{align*}
\sum_{\sigma=0}^{t'} {t' \choose \sigma} (-1)^{\sigma} M'_{\{s'+t', s'+\sigma \},\{p',0\}} 
& = 
\sum_{\rho=0}^{t'}  \mubar{s'+t'+p'-\rho}  \sum_{\sigma=0}^{t'-\rho} {t' \choose \sigma} (-1)^{\sigma} {t'-\sigma \choose \rho} { r-t'+\sigma \choose p'- \rho}  \\
& = \begin{cases}
0 & \text{ if } p' < t' \\
{r-t' \choose p'-t'} \sum_{\rho=0}^{t'}  (-1)^{t'-\rho} {t' \choose \rho} \mubar{s'+t'+p'-\rho} 
  & \text{ if }  t' \leq p' \leq \ell \\
\end{cases} \\
& = \begin{cases}
0 & \text{ if } p' < t' \\
{r-t' \choose p'-t'} D_{t'}^{s'+p'}
  & \text{ if }  t' \leq p' \leq \ell  \text{   ( Definition \ref{def:Dpq})}\\
\end{cases}
\end{align*}


\end{proof}

\subsection{Proof of Claim \ref{clm:row_decomp}}


\begin{proof}
By Definition \ref{def:row_combination} and Pascal's rule, we have
\begin{align*}
\Re_{s+t,s}^{t} 
& = \sum_{\sigma=0}^{t} {t \choose \sigma} (-1)^{\sigma} Q_{\{s+t,s+\sigma \}} \\
& = \sum_{\sigma=0}^{t} [{t-1 \choose \sigma-1} + {t-1 \choose \sigma}](-1)^{\sigma} Q_{\{s+t,s+\sigma \}} \\
& = \sum_{\sigma=1}^{t} {t-1 \choose \sigma-1} (-1)^{\sigma} Q_{\{s+t,s+\sigma \}} 
+  \sum_{\sigma=0}^{t-1} {t-1 \choose \sigma}(-1)^{\sigma} Q_{\{s+t,s+\sigma \}}  \\
& = -\sum_{\sigma=0}^{t-1} {t-1 \choose \sigma} (-1)^{\sigma} Q_{\{s+t,s+\sigma+1 \}} +  \sum_{\sigma=0}^{t-1} {t-1 \choose \sigma} (-1)^{\sigma} Q_{\{s+t,s+\sigma \}} \\
& = -\Re_{s+t,s+1}^{t-1} +\Re_{s+t,s}^{t-1}.   \\
\end{align*}
By rearanging, we have $\Re_{s+t,s}^{t-1} = \Re_{s+t,s}^{t} +  \Re_{s+t,s+1}^{t-1}$.

\end{proof}


\subsection{Proof of Claim \ref{clm:d_linear_relation}}
\label{sec:clm_d_linear_relation}
\begin{proof}
We prove a stronger version of the claim:
$$ \frac{D^{p}_{q}}{D^{p}_{q+1}} = c^{(1)}_q p +  c^{(2)}_q \text{ and } \frac{D^{p+1}_{q}}{D^{p}_{q+1}} =  c^{(1)}_q  p +  c^{(3)}_q $$ 
for some constants $ c^{(1)}_q , c^{(2)}_q,  c^{(3)}_q \in \mathbb{R}$ dependent on $q$. We prove it by induction.
\begin{enumerate}
    \item For $q = 0$, 
    \begin{equation}
    \label{eqn:AB0}
    \frac{D^p_0}{D^p_1} 
    = \frac{\mubar{p}}{ \mubar{p}-\mubar{p+1}}
    = \frac{1}{1-\mubar{p+1}/\mubar{p}} 
    = \frac{1}{1- \frac{a(a-b) + p(b-a^2)}{a -b + t(b-a^2)}}
    = \frac{a-b + p(b-a^2) }{(1-a)(a-b)} 
    = c^{(1)}_0 p + c^{(2)}_0
    \end{equation}
    \begin{equation}
    \label{eqn:AC0}
    \frac{D^{p+1}_0}{D^p_1} 
    = \frac{\mubar{p+1}}{ \mubar{p}-\mubar{p+1}}
    = \frac{1}{\mubar{p}/\mubar{p+1}-1} 
    = \frac{1}{\frac{a-b + p(b-a^2)}{a(a-b) + p(b-a^2)} - 1}
    = \frac{a(a-b) + p(b-a^2) }{(1-a)(a-b)} 
    = c^{(1)}_0 p + c^{(3)}_0 
    \end{equation}

    \item When $q = k$, suppose we have 
    $$\frac{D^{p}_{k}}{D^{p}_{k+1}} = c^{(1)}_k p + c^{(2)}_k, \text{ and } \frac{D^{p+1}_{k}}{D^{p}_{k+1}} = c^{(1)}_k p + c^{(3)}_q$$ for some constants $c^{(1)}_k, c^{(2)}_k, c^{(3)}_k \in \mathbb{R}$.


    \item When $q = k+1$, by the assumption in step 2, we have 
    $$ \frac{D^{p+1}_{k+1}} {D^p_{k+1}}
    = \frac{D^{p+1}_{k}/  D^{t}_{k+1}} {D^{p+1}_{k}/D^{p+1}_{k+1}}
    = \frac{c^{(1)}_k p + c^{(3)}_k}{c^{(1)}_k p + c^{(1)}_k + c^{(2)}_k}.
    $$
    Then, 
    
    \begin{align}
    \label{eqn:a_k_relation}
     \frac{D^p_{k+1}}{D^p_{k+2}} 
    & = \frac{D^p_{k+1}}{D^p_{k+1} - D^{p+1}_{k+1}} 
    =  \frac{1}{1 - D^{p+1}_{k+1}/ D^p_{k+1}}
    = \frac{c^{(1)}_k p + c^{(1)}_k + c^{(2)}_k}{c^{(1)}_kt + c^{(1)}_k + c^{(2)}_k - c^{(1)}_k t - c^{(3)}_k} \nonumber \\
    & = \frac{c^{(1)}_k p}{c^{(1)}_k + c^{(2)}_k - c^{(3)}_k} + \frac{c^{(1)}_k + c^{(2)}_k}{c^{(1)}_k + c^{(2)}_k - c^{(3)}_k}  
    \end{align}

    Also, 
    \begin{equation}
    \label{eqn:c_k_relation}
    \small
    \frac{D^{p+1}_{k+1}}{D^p_{k+2}} 
    = \frac{D^{p+1}_{k+1}}{D^p_{k+1} - D^{p+1}_{k+1}}
    = \frac{1}{D^p_{k+1} /D^{p+1}_{k+1} - 1}
    = \frac{c^{(1)}_k p + c^{(3)}_k}{c^{(1)}_k + c^{(2)}_k - c^{(3)}_k}
    = \frac{c^{(1)}_k p }{c^{(1)}_k + c^{(2)}_k - c^{(3)}_k} + \frac{c^{(3)}_k}{c^{(1)}_k + c^{(2)}_k - c^{(3)}_k}
    \end{equation}
    The first equality in equations \eqref{eqn:a_k_relation} and \eqref{eqn:c_k_relation} is due to 
    \begin{align}
    D^{p}_{k+2} 
    & = \sum_{i=0}^{k+2} {k+2 \choose i }(-1)^i \mubar{p+i}  
    \nonumber \\
    & =  \mubar{p} + \sum_{i=1}^{k+2} ( {k+1 \choose i-1} + {k+1 \choose i})(-1)^i \mubar{p+i} 
     \nonumber\\
    & = \sum_{i=0}^{k+1} {k \choose i }(-1)^i \mubar{p+i} - \sum_{i=0}^{k+1} {k+1 \choose i }(-1)^i \mubar{p+i+1}
    \nonumber \\
    & =  D^{p}_{k+1} - D^{p+1}_{k+1} \nonumber \\
    \label{eqn:D_recursive_relation}
    \end{align}
    
    Therefore, by Eqn. \eqref{eqn:a_k_relation}, \eqref{eqn:c_k_relation}, we can get 
    \begin{equation}
    \label{eqn:abc_k_relation}
    c^{(1)}_{k+1} = \frac{c^{(1)}_k}{c^{(1)}_k + c^{(2)}_k - c^{(3)}_k},
    \ \ c^{(2)}_{k+1} = \frac{c^{(1)}_k + c^{(2)}_k}{c^{(1)}_k + c^{(2)}_k - c^{(3)}_k},
    \ \ c^{(3)}_{k+1}=  \frac{c^{(3)}_k}{c^{(1)}_k + c^{(2)}_k - c^{(3)}_k}
    \end{equation}
    So we can conclude that these two ratio have affine relationship with $p$.

\end{enumerate}

\end{proof}



\subsection{Proof of Claim \ref{clm:dpq_value_thm2}}
We first prove that $D^p_1 = \mubar{p} - \mubar{p+1} \propto \frac{d-1}{pd}$ for $1 \leq p \leq d-1$.

\begin{align*}
\mubar{p}
& = \sum_{i=0}^{d-p-1} { d-p \choose i } \mu_{i+p} \ \ \ ( \text{ Definition } \ref{def:cumulative_weighting})  \\
& \propto 
\sum_{i=0}^{d-p-1} { d-p \choose i } \frac{d-1}{{d \choose i+p}(i+p)(d-i-p) } \ \ \ ( \mu_d=0)\\
& =
(d-1)\sum_{i=0}^{d-p-1}  \frac{ (d-p)!(i+p-1)!(d-i-p-1)!}{i!(d-p-i)!d!  } \\
& = 
\frac{(d-1)(d-p)!}{d!} \sum_{i=0}^{d-p-1}  \frac{(i+p-1)!}{i!(d-p-i)} \\
& = 
\frac{(d-1)(d-p)!}{d!} \sum_{i=0}^{d-p-1}  \frac{\prod_{j=1}^{p-1}(i+j) }{d-p-i} \\
\end{align*}
Then, we have 
\begin{align*}
D^p_1 
& = \mubar{p} - \mubar{p+1} \\
& \propto 
\frac{(d-1)(d-p)!}{d!} \sum_{i=0}^{d-p-1}  \frac{\prod_{j=1}^{p-1}(i+j) }{d-p-i}
- \frac{(d-1)(d-p-1)!}{d!} \sum_{i=0}^{d-p-2}  \frac{\prod_{j=1}^{p}(i+j) }{d-p-i-1}
\\
& =
\frac{(d-1)(d-p-1)!}{d!}
\left[
(p-1)! +
\sum_{i=0}^{d-p-2}  \left[ \frac{(d-p)\prod_{j=1}^{p-1}(i+j+1) }{d-p-i-1} 
- \frac{\prod_{j=1}^{p}(i+j) }{d-p-i-1}
\right]\right] \\
& =
\frac{(d-1)(d-p-1)!}{d!}
\left[
(p-1)! +
\sum_{i=0}^{d-p-2} \frac{\prod_{j=1}^{p-1}(i+j+1)}{d-p-i-1} \left[ d-p-i-1
\right]\right] \\
& =
\frac{(d-1)(d-p-1)!(p-1)!}{d!}
\left[
1 +
\sum_{i=0}^{d-p-2} \ \  \frac{\prod_{j=1}^{p-1}(i+j+1)}{(p-1)!}
\right] \\
& =
\frac{(d-1)(d-p-1)!(p-1)!}{d!}
\sum_{i=p-1}^{d-2}  
{ i \choose p-1 }\\
& = 
\frac{(d-1)(d-p-1)!(p-1)! {d-1 \choose p }}{d!} \ \ \ (*)\\
& = 
\frac{(d-1)(d-p-1)!(p-1)!(d-1)!}{d!p!(d-p-1)!} \\
& = 
\frac{d-1}{dp} \\
\end{align*}

where $(*)$ follows from using Pascal's rule for multiple times:
\begin{align*}
{d-1 \choose p} 
& = {d-2 \choose p-1} + {d-2 \choose p}   \\
& = {d-2 \choose p-1} + {d-3 \choose p-1} +  {d-3 \choose p} \\
& = {d-2 \choose p-1} + {d-3 \choose p-1} + \cdots +  {p \choose p-1} + {p \choose p} \\
& = \sum_{i=p-1}^{d-2} {i \choose p-1} \\
\end{align*}

Then we prove the following equation by induction on $q$. We have proved the basic case when $q=1$. Let assume that it holds for $q-1$, such that for all $0 \leq p \leq d-q$, 
\begin{align*}
D^p_{q-1}
= \sum_{j=0}^{q-1} 
{ q-1 \choose j}(-1)^j \mubar{p+j}
\propto 
\frac{d-1}{d(q-1) { p+q-2 \choose p-1 } }.
\end{align*}

Then, we have
\begin{align*}
D^p_{q}
& = D^p_{q-1} - D^{p+1}_{q-1} 
\ \ \ \ \ (\text{Eqn. \eqref{eqn:D_recursive_relation}}) \\
& \propto 
\frac{d-1}{d} \times \frac{1}{(q-1) { p+q-2 \choose p-1 } } - \frac{1}{(q-1) { p+q-1 \choose p } } \\
& = 
\frac{d-1}{d} \times
\frac{1}{(q-1) { p+q-2 \choose p-1 } }
\left( 1 - \frac{p}{ p+q-1 } \right)\\
& = 
\frac{d-1}{d} \times
\frac{1}{{ p+q-2 \choose p-1 }( p+q-1) } \\
& = 
\frac{d-1}{d} \times
\frac{(p-1)!(q-1)!}{(p+q-1)! } \\
& = 
\frac{d-1}{dq {p+q-1 \choose p-1}} \\
\end{align*}
Therefore, we complete the induction proof. 


\subsection{Proof of Claim \ref{clm:d_linear_relation_thm2}}
\begin{proof}
By Claim \ref{clm:dpq_value_thm2}, we have
\begin{align*}
\frac{D^{p}_{q}}{D^{p}_{q+1}}  
& = \frac{\frac{1}{q { p+q-1 \choose p-1 } }}{\frac{1}{(q+1) { p+q \choose p-1 } }} 
= \frac{q+1}{q} \times \frac{p+q}{q+1}
= \frac{p}{q} + 1 \\
\end{align*}
The constants are $ c^{(1)}_q = \frac{1}{q}  \text{  and  } c^{(2)}_q  = 1$.

\end{proof}

\subsection{Proof of Claim \ref{clm:closed_form_basis_function}}

First of all, by Claim \ref{clm:dpq_value_thm2}, we plug in $D^p_q 
= \frac{d-1}{dq { p+q-1 \choose p-1 } }$ to the equation.

\begin{proof}

\begin{align}
& \sum_{j=0}^{\ell - i} 
{ r- i \choose j} \frac{D_{i}^{j+i}}{D^{r}_{i}} 
\frac{(r-1)!(\ell + i+j -1)!}{(r+\ell-1)!(j+i-1)!} { r - j-i - 1 \choose \ell - i-j} (-1)^{\ell - i - j}  \nonumber\\
& = \frac{(r+i-1)!(r-i)!}{(r+\ell-1)!(r-\ell-1)!}\sum_{j=0}^{\ell - i} 
\frac{(\ell + i+ j -1)!}{(r-i-j)j!(j+2i-1)!(\ell-i-j)!}(-1)^{\ell - i - j}   \nonumber\\
& = 
\frac{(r+i-1)!(r-i)!}{(r+\ell-1)!(r-\ell-1)!}\sum_{j=0}^{\ell - i} 
\frac{(\ell-i)!(-1)^{\ell-i-j}}{(r-i-j)j!(\ell-i-j)!}\cdot 
\frac{(\ell + i+j -1)!}{(j+2i-1)!(\ell-i)!}  \nonumber\\
& = 
\frac{(r+i-1)!(r-i)!}{(r+\ell-1)!(r-\ell-1)!}
\underbrace{\sum_{j=0}^{\ell - i} 
 \frac{(-1)^{\ell-i-j}{\ell -i \choose \ell -i - j}}{r-i-j} \cdot
{\ell+i+j-1 \choose \ell-i} }_{(i)}
\label{eqn:(i)_substitute}
\end{align}
Now we use generating function to prove the above equation equals 1. 

First, we look at the coefficients of the generating function $p_1(x) = \int x^{r-\ell-1}(1-x)^{\ell-i} dx$. 
By using the fact that the 
coefficient of $x^{r-i-n-1}$ in the polynomial $x^{r-\ell-1}(1-x)^{\ell-i} $ is
$(-1)^{\ell-i-n}{\ell -i \choose \ell-i-n}$ for some $0 \leq n \leq \ell-i$, we have 
$$
p_1(x) = \int x^{r-\ell-1}(1-x)^{\ell-i} dx = \sum_{n=0}^{\ell-i} \frac{(-1)^{\ell-i-n}{\ell-i \choose \ell-i-n}}{r-i-n} x^{r-i-n},
$$
where we set the constant term in the integration is zero.

Secondly, we consider another polynomial \footnote{Generally, for any non-negative integer $k$ and non-zero real value $a$, we have $\sum_{n=0}^{\infty}a^n {n+k \choose k} x^n = \frac{1}{(1-ax)^{k+1}}$.} 
$$p_2(x) =\frac{1}{(1-x)^{\ell-i+1}}
= \sum_{m=0}^{\infty}{ m + \ell -i \choose \ell-i}x^m.$$ 

Finally, we deal with the coefficient of $x^{r+i-1}$ term of the polynomial $p_1(x)p_2(x)$. By combining the above two equalities, this coefficient is 
\begin{align*}
& \sum_{n=0}^{\ell-i} \left( \frac{(-1)^{\ell-i-n}{\ell-i \choose \ell-i-n}}{r-i-n} x^{r-i-n}
 \cdot {(2i+n-1)+\ell-i \choose \ell-i }x^{2i+n-1} \right) \\
& = x^{r+i-1} \underbrace{\sum_{n=0}^{\ell-i} \frac{(-1)^{\ell-i-n}{\ell-i \choose \ell-i-n}}{r-i-n}
\cdot {\ell+i+n-1 \choose \ell-i } }_{(ii)}. 
\end{align*}

Now, if we compare (i) and (ii), we can see that their values are the same. Therefore, (i) is actually the coefficient of $x^{r+i-1}$ term of the polynomial $p_1(x)p_2(x)$.

We now analyze the polynomial $p_1(x) = \int x^{r-\ell-1}(1-x)^{\ell-i} dx$.
\begin{claim}
\label{clm:int_closed_form}
Assume that the constant term in the polynomial $p_1(x) = \int x^{r-\ell-1}(1-x)^{\ell-i} dx$ is zero so that $p_1(0)=0$. Then we have 
$$
p_1(x) = \int x^{r-\ell-1}(1-x)^{\ell-i} dx 
= (1-x)^{\ell-i+1}p(x) + \frac{(r-\ell-1)! }{\prod_{k=0}^{r-\ell-1} (\ell-i+k+1)},
$$
where $p(x)$ is a polynomial with degree at most $\leq r-\ell-1$.
\end{claim}

We delay the proof to Section \ref{sec:proof_int_closed_form}. Now, we are able to calculate the polynomial $p_1(x)p_2(x)$:
\begin{align*}
p_1(x)p_2(x) 
& = \frac{\int x^{r-\ell-1}(1-x)^{\ell-i} dx }{(1-x)^{\ell-i+1}} \\
& = p(x) + \frac{(r-\ell-1)! }{\prod_{k=0}^{r-\ell-1} (\ell-i+k+1)} \cdot \frac{1}{{(1-x)^{\ell-i+1}}}
\ \  \text{(Claim \ref{clm:int_closed_form})} \\
& =  p(x) + \frac{(r-\ell-1)! }{\prod_{k=0}^{r-\ell-1} (\ell-i+k+1)}  \sum_{m=0}^{\infty}{ m + \ell -i \choose \ell-i}x^m. \\
\end{align*}
We note that $p(x)$ is a polynomial with degree $\leq r-\ell-1$. Recall that our goal is to calculate the coefficient of $x^{r+i-1}$ term of the polynomial $p_1(x)p_2(x)$, so $p(x)$ has nothing to do with it. Therefore, we have 
\begin{align*}
(i) & = \frac{(r-\ell-1)! }{\prod_{k=0}^{r-\ell-1} (\ell-i+k+1)} { (r+i-1) + \ell -i \choose \ell-i} \\
& = \frac{(r-\ell-1)!(\ell-i)! }{(r-i)!} { r+\ell-1 \choose \ell-i} \\
& = \frac{(r-\ell-1)!(r+\ell-1)! }{(r-i)!(r+i-1)!}. \\
\end{align*}

By substituting the value of (i) to Eqn.\eqref{eqn:(i)_substitute}, we get
$$
\sum_{j=0}^{\ell - i} 
{ r- i \choose j} \frac{D_{i}^{j+i}}{D^{r}_{i}} 
\frac{(r-1)!(\ell + j+i -1)!}{(r+\ell-1)!(j+i-1)!} { r - j-i - 1 \choose \ell - i-j} (-1)^{\ell - i - j} 
= 1.
$$

\end{proof}



\subsection{Proof of Claim \ref{clm:I_value}}
\label{sec:proof_claim_I_value}
\begin{proof}
Before we prove Claim \ref{clm:I_value}, we first derive the following equality.
\begin{claim}
\label{clm:rho_poly}
For any $x',\sigma \in \mathbb{R}$ and $y' \in \mathbb{N} + \{0\}$, we have
$$ 
\prod_{j=0}^{y'} (x'+\sigma-j) =
C_0 +
\sum_{j=0}^{y'} C_{j+1} \sigma(\sigma-1)...(\sigma-j) 
\text{ with } 
C_i = \frac{1}{i!}\prod_{j=0}^{i-1} (y'+1-j) \prod_{k=0}^{y'-i}(x'-k)
$$
\end{claim}

\begin{proof}
Let
$$
g(\sigma) = \prod_{j=0}^{y'} (x'+\sigma-j)  
$$
We note that $g(\sigma)$ is a $(y'+1)^{\text{th}}$-polynomial in terms of $\sigma$. Since $\{\sigma(\sigma-1)...(\sigma-j)  \}_{j=0}^{y'}\cup \{ 1\}$ is a basis for this polynomial, $g(\sigma)$ can be expressed as $C_{(0)}(x') +
\sum_{j=0}^{y'} C_{(j+1)}(x') \sigma(\sigma-1)...(\sigma-j) $ with some functions $C_{(0)}(x'),...,C_{(y'+1)}(x')$ of $x'$. Now we proof that 

$$
C_{(i)}(x') =  \frac{1}{i!}\prod_{j=0}^{i-1} (y'+1-j) \prod_{k=0}^{y'-i}(x'-k) = C_i
$$
by induction.
At each induction step, we prove that 
$ C_i = C_{(i)}(x') = \frac{1}{i!}( \sum_{j=0}^{i} (-1)^{i-j}{ i \choose j }g(j) )
=  \frac{1}{i!}\prod_{j=0}^{i-1} (y'+1-j) \prod_{k=0}^{y'-i}(x'+i+k)$.
\begin{enumerate}
    \item When $i=0$, by plugging in $\sigma = 0$ in $g(\sigma)$, we have
    $$
    C_{(0)}(x')  = g(0) 
    = \prod_{j=0}^{y'} (x'-j)
    = \prod_{k=0}^{y'} (x'-k) 
    = C_0.
    $$ 
    
    \item When $i=0,1,...,i'$ for some $i'>0$, assume that we have 
    $$
    C_{i}
    = C_{(i)}(x')
    = \frac{1}{i!} \left( \sum_{j=0}^{i} (-1)^{i-j}{ i \choose j }g(j) \right)
    = \frac{1}{i!}\prod_{j=0}^{i-1} (y'+1-j) \prod_{k=0}^{y'-i}(x'-k).
    $$
    
    \item When $i=i'+1$, by plugging in $\sigma = i'+1$, we have
    $$
    g(i'+1) = \prod_{j=0}^{y'} (x'+i'+1-j) 
    = C_{(0)}(x') + \sum_{j=0}^{i'} C_{(j+1)}(x') (i'+1)(i')...(i'+1-j) 
    $$
    Now we can express $C_{(i'+1)}(x')$ as $C_{(0)}(x'),..., C_{(i')}(x')$ and $g(i'+1)$. First, we proof $C_{(i'+1)}(x') =  \frac{1}{(i'+1)!}\sum_{k=0}^{i'+1} 
    { i'+1 \choose k}
     (-1)^{i'+1-k}  g(k) $.
    \begin{align*}
    & C_{(i'+1)}(x') \\
    & = \frac{1}{(i'+1)!}\left(g(i'+1) - C_{(0)}(x') - \sum_{j=0}^{i'-1}  (i'+1)(i')...(i'+1-j) C_{(j+1)}(x')\right) \\
    & = \frac{1}{(i'+1)!}\left(g(i'+1) - g(0) - \sum_{j=0}^{i'-1}(i'+1)(i')...(i'+1-j)  \frac{1}{(j+1)!} \left[ \sum_{k=0}^{j+1} (-1)^{j+1-k}{ j+1 \choose k }g(k) \right] \right) \\
    & = \frac{1}{(i'+1)!}\left(g(i'+1) - g(0) - \sum_{j=0}^{i'-1}
    { i'+1 \choose j+1 }
    \left[ \sum_{k=0}^{j+1} (-1)^{j+1-k}{ j+1 \choose k }g(k) \right] \right) \\
    & = \frac{1}{(i'+1)!}\left(g(i'+1)  - \sum_{j=0}^{i'}
    { i'+1 \choose j }
    \left[ \sum_{k=0}^{j} (-1)^{j-k}{ j \choose k }g(k) \right] \right) \\
    & = \frac{1}{(i'+1)!}\left(g(i'+1)  - \sum_{k=0}^{i'}  \sum_{j=k}^{i'}
    { i'+1 \choose j }
    (-1)^{j-k}{ j \choose k }g(k)  \right) \\
    & = \frac{1}{(i'+1)!}\left(g(i'+1)  - \sum_{k=0}^{i'}  g(k) \sum_{j=k}^{i'} 
    \frac{(-1)^{j-k}(i'+1)!j!}{j!(i'+1-j)!k!(j-k)!}\right) \\
    & = \frac{1}{(i'+1)!}\left(g(i'+1)  - \sum_{k=0}^{i'}  g(k)
    \frac{(i'+1)!}{k!(i'-k+1)!}
    \sum_{j=0}^{i'-k} 
    \frac{(-1)^{j}(i'-k+1)!}{(i'-j+k+1)!(j)!}\right) \\
    & = \frac{1}{(i'+1)!}\left(g(i'+1)  - \sum_{k=0}^{i'}  g(k)
    { i'+1 \choose k}
    ( (-1)^{i'-k} + \sum_{j=0}^{i'-k+1} 
    \frac{(-1)^{j}(i'-k+1)!}{(i'-j+k+1)!(j)!} )\right) \\
    & = \frac{1}{(i'+1)!}\left(g(i'+1)  - \sum_{k=0}^{i'}  g(k)
    { i'+1 \choose k}
    ( (-1)^{i'-k} + (1-1)^{i'-k+1} )\right) \\
     & = \frac{1}{(i'+1)!}\sum_{k=0}^{i'+1}  g(k)
    { i'+1 \choose k}
     (-1)^{i'+1-k} \\
    \end{align*}
    Secondly, we prove that $C_{(i'+1)}(x')
    =  \frac{1}{(i'+1)!}\prod_{j=0}^{i'} (y'+1-j) \prod_{k=0}^{y'-i}(x'+i'+1+k) 
    = C_{i'+1}$.
    
    \begin{align*}
    C_{(i'+1)}(x')
    & = \frac{1}{(i'+1)!}( \sum_{j=0}^{i'+1} (-1)^{i'+1-j}{ i'+1 \choose j }g(j) ) \\
    & = \frac{1}{(i'+1)!}
    \left(  \sum_{j=0}^{i'} (-1)^{i'-j}{ i' \choose j } g(j+1)-\sum_{j=0}^{i'} (-1)^{i'-j}{ i' \choose j }g(j) \right) 
    \ \ \ (\text{Pascal's rule} )\\
    & = \frac{1}{(i'+1)!}
    \left(  \sum_{j=0}^{i'} (-1)^{i'-j}{ i' \choose j } g(j+1)
    -\sum_{j=0}^{i'} (-1)^{i'-j}{ i' \choose j }g(j) \right) \\
    & = \frac{1}{(i'+1)!}
    (i'!C_{(i')}(x'+1) - i'!C_{(i')}(x') ) \\
    & =  \frac{1}{(i'+1)!}(\prod_{j=0}^{i'-1} (y'+1-j) \prod_{k=0}^{y'-i'}(x'+1-k) - \prod_{j=0}^{i'-1} (y'+1-j) \prod_{k=0}^{y'-i'}(x'-k) ) \\
    & =  \frac{\prod_{j=0}^{i'-1} (y'+1-j) \prod_{k=0}^{y'-i'-1}(x'-k)}{(i'+1)!}( (x'+1) -  (x'-y'+i') ) \\
    & =  \frac{\prod_{j=0}^{i'} (y'+1-j) \prod_{k=0}^{y'-i'-1}(x'-k)}{(i'+1)!}\\
    & = C_{i'+1} \\
    \end{align*}
\end{enumerate}
Then we complete the induction proof of Claim \ref{clm:rho_poly}.
\end{proof}

Now we come back to the proof of Claim \ref{clm:I_value}.

Since we may have $r-t'+\sigma < t'=\rho$, we expand ${ r-t'+\sigma \choose p'- \rho}$ with ${ r-t'+\sigma \choose p'- \rho} = \frac{ \prod_{j=0}^{p'-\rho-1} (r-t'+\sigma-j)}{(p'-\rho)!}$ to avoid the denominator being zero.
\begin{align*}
& \sum_{\sigma=0}^{t'-\rho} {t' \choose \sigma} (-1)^{\sigma} {t'-\sigma \choose \rho} { r-t'+\sigma \choose p'- \rho} \\
& = \sum_{\sigma=0}^{t'-\rho} 
\frac{(-1)^{\sigma}t'!(t'-\sigma)!}
{\sigma!(t'-\sigma)!\rho!(t'-\sigma-\rho)!} 
\frac{ \prod_{j=0}^{p'-\rho-1} (r-t'+\sigma-j)}{(p'-\rho)!}
\\
& = \frac{t'!}{\rho!(p'-\rho)!}
\sum_{\sigma=0}^{t'-\rho} 
\frac{(-1)^{\sigma} \prod_{j=0}^{p'-\rho-1} (r-t'+\sigma-j)}
{\sigma!(t'-\sigma-\rho)!}
\\
& = \frac{t'!}{\rho!(p'-\rho)!}
\sum_{\sigma=0}^{t'-\rho} 
\frac{(-1)^{\sigma} (C_0 + \sum_{j=0}^{p'-\rho-1} C_{j+1}
\sigma(\sigma-1)...(\sigma-j) ) } 
{\sigma!(t'-\sigma-\rho)!} \\
& (\text{By plugging in $x'=r-t'$ and $y'=p-\rho -1$ in Claim.\ref{clm:rho_poly}.})
\\
& = 
\underbrace{\frac{ t'!}{\rho!(p'-\rho)!} 
\left[C_0 \sum_{\sigma=0}^{t'-\rho} 
\frac{(-1)^{\sigma} }
{\sigma!(t'-\sigma-\rho)!}  + \sum_{j=0}^{p'-\rho-1} C_{j+1} 
\sum_{\sigma=0}^{t'-\rho} 
\frac{(-1)^{\sigma} \sigma(\sigma-1)...(\sigma-j) }
{\sigma!(t'-\sigma-\rho)!} \right]}_{(I)}.
\\
\end{align*}

Then we separate $(I)$ into two cases. 
First, when $\sigma \leq j'$, we have $\sigma(\sigma-1)...(\sigma-j)= 0$. Therefore, we have 
\begin{align*}
(I) & = \frac{ t'!}{\rho!(p'-\rho)!} 
\left[C_0 \sum_{\sigma=0}^{t'-\rho} 
\frac{(-1)^{\sigma} }
{\sigma!(t'-\sigma-\rho)!}  + \sum_{j=0}^{t'-\rho-1} C_{j+1} 
\sum_{\sigma=j+1}^{t'-\rho} 
\frac{(-1)^{\sigma} }
{(\sigma-j-1)!(t'-\sigma-\rho)!} \right] 
\\
& = \frac{t'!}{\rho!(p'-\rho)!}
\sum_{j=0}^{t'-\rho}  C_j \sum_{\sigma=j}^{t'-\rho} 
\frac{(-1)^{\sigma} }
{(\sigma-j)!(t'-\sigma-\rho)!} 
\\
& = \frac{t'!}{\rho!(t'-\rho)!}
\sum_{j=0}^{t'-\rho} C_j (t'-\rho -j)! \sum_{\sigma=j}^{t'-\rho} 
(-1)^{\sigma} {t'-\rho -j \choose t'-\rho-\sigma}
\\
& = \frac{t'!}{\rho!(t'-\rho)!}
\sum_{j=0}^{t'-\rho}  C_j (t'-\rho -j)! (1-1)^{t'-\rho-j} (-1)^j
\\
& =
\frac{t'!C_{t'-\rho}}{\rho!(p'-\rho)!} (-1)^{t'-\rho} \\
& =
\frac{t'!}{\rho!(p'-\rho)!}
\frac{(p'-\rho)!(r-t')!}{(t'-\rho)!(p'-t')!(r-p')!} (-1)^{t'-\rho} \\
& (\text{By plugging in $x'=r-t'$ and $y'=p-\rho -1$ in Claim.\ref{clm:rho_poly}.}) \\
& =
{r-t' \choose p' - t' }{t' \choose \rho} (-1)^{t'-\rho} \\
\end{align*}

Secondly, if $p' < t'$, 
\begin{align*}
(I)& = \frac{ t'!}{\rho!(p'-\rho)!} 
\left[\frac{ C_0(-1)^{\sigma} }{\sigma!(t'-\sigma-\rho)!}\sum_{\sigma=0}^{t'-\rho} 
\frac{(-1)^{\sigma} }
{\sigma!(t'-\sigma-\rho)!}  + \sum_{j=0}^{t'-\rho-1} C_{j+1} 
\sum_{\sigma=0}^{t'-\rho} 
\frac{(-1)^{\sigma} }
{(\sigma-j-1)!(t'-\sigma-\rho)!} \right] 
\\
& = \frac{t'!}{\rho!(p'-\rho)!}
\sum_{j=0}^{t'-\rho}  C_j \sum_{\sigma=j}^{t'-\rho} 
\frac{(-1)^{\sigma} }
{(\sigma-j)!(t'-\sigma-\rho)!} \ \ \ ( \sigma \leq j \Rightarrow \sigma(\sigma-1)...(\sigma-j)= 0)
\\
& = \frac{t'!}{\rho!(t'-\rho)!}
\sum_{j=0}^{p'-\rho} C_j (t'-\rho -j)! \sum_{\sigma=j}^{t'-\rho} 
(-1)^{\sigma} {t'-\rho -j \choose t'-\rho-\sigma}
\\
& = \frac{t'!}{\rho!(t'-\rho)!}
\sum_{j=0}^{p'-\rho}  C_j (t'-\rho -j)! (1-1)^{t'-\rho-j}
\\
& =0
\end{align*}
\end{proof}

\subsection{Proof of Claim \ref{clm:int_closed_form}}
\label{sec:proof_int_closed_form}

\begin{proof}
We prove a more general form: for any $a,b \in \mathbb{N} + \{0\}$, we have 
\begin{equation}
\label{eqn:int_closed_form}
g_{a,b}(x) = \int x^{a}(1-x)^{b} dx 
= 
(1-x)^{b+1}p_{a,b}(x) + \frac{a! }{\prod_{k=0}^{a} (b+k+1)},
\end{equation}
where $g_{a,b}(x),p_{a,b}(x)$ are polynomials depended on $a,b$ with $g_{a,b}(0)=0$ . 

Now we prove Eqn.\eqref{eqn:int_closed_form} by induction on $a$. For $a=0$, we have 
$$
\int (1-x)^{b} dx  = \frac{-(1-x)^{b+1}}{b+1} + \frac{1}{b+1}.
$$
Assume that Eqn.\eqref{eqn:int_closed_form} holds for $a=n$. 
Then, for $a,b \in \mathbb{N}$, using integration by parts, we have 
\begin{align*}
& \int x^{n+1}(1-x)^{b} dx \\
& = \frac{-1}{b+1}\int x^{n+1} d (1-x)^{b+1} \\
& = \frac{-1}{b+1}x^{n+1}(1-x)^{b+1} + \frac{1}{b+1} \int (1-x)^{b+1} d x^{n+1}  \\
& =  \frac{-1}{b+1}x^{n+1}(1-x)^{b+1} + \frac{n+1}{b+1} \int x^{n}(1-x)^{b+1} dx.
\end{align*}
We note that the first term is divisible by $(1-x)^{b+1}$, while the second term can be obtained by induction hypothesis. Therefore, we have 
\begin{align*}
g_{n+1,b}(x)
& = \int x^{n+1}(1-x)^{b} dx \\
& = (1-x)^{b+1}p_{n+1,b}(x) + \frac{n+1}{b+1}\frac{n! }{\prod_{k=0}^{n} (b+k+2)}   \\
& = (1-x)^{b+1}p_{n+1,b}(x) + \frac{(n+1)! }{\prod_{k=0}^{n+1} (b+k+1)}.
\end{align*}
By plugging in $a=r-\ell-1$ and $b=\ell-1$, we have the desired results. Also, since the degree of $p_1(x) = \int x^{r-\ell-1}(1-x)^{\ell-i} dx$ is at most $r-i$, $p(x)$ should have degree less or equal to $r-\ell-1$.

\end{proof}



